A Survey on Trajectory Data Management, Analytics, and Learning

Recent advances in sensor and mobile devices have enabled an unprecedented increase in the availability and collection of urban trajectory data, thus increasing the demand for more efficient ways to manage and analyze the data being produced. In this survey, we comprehensively review recent research trends in trajectory data management, ranging from trajectory pre-processing, storage, common trajectory analytic tools, such as querying spatial-only and spatial-textual trajectory data, and trajectory clustering. We also explore four closely related analytical tasks commonly used with trajectory data in interactive or real-time processing. Deep trajectory learning is also reviewed for the first time. Finally, we outline the essential qualities that a trajectory data management system should possess in order to maximize flexibility.

==> 1-Survey-trajectory 2/NewCommands.tex <==
\let\labelindent\relax
\usepackage{enumitem}
\renewcommand{\cite}{\citep}

\newcommand{\ms}[1]{\textrm{\textcolor{cyan}{Mark says: #1}}}
\newcommand{\shane}[1]{\textrm{\textcolor{orange}{Shane says: #1}}}
\newcommand{\myparagraph}[1]{\vspace{0.6\baselineskip}\noindent{\textbf{#1.}}~}
\newcommand{\var}[1]{\mbox{\emph{#1}}}
\newcommand{\svar}[1]{\mbox{\scriptsize\emph{#1}}}
\newcommand{\tvar}[1]{\mbox{\tiny\emph{#1}}}
\newcommand{\avar}[1]{\mbox{#1}}
\newcommand{\asvar}[1]{\mbox{\scriptsize{#1}}}
\newcommand{\atvar}[1]{\mbox{\tiny{#1}}}
\def\D{\hphantom{1}}
\def\C{\hphantom{1,}}
\newcommand{\mycaption}[1]{\caption{\normalfont{#1}}}



\newtheorem{example}{Example}
\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{conjecture1}{Conjecture}
\newtheorem{assumption}{Assumption}
\newtheorem{criteria}{Criteria}
\newtheorem{property}{Property}
\newtheorem{observation}{Observation}


\newcommand{\bao}[1]{{\color{blue} #1}}
\newcommand{\sheng}[1]{{\color{blue} #1}}
\newcommand{\newcontent}[1]{{\color{black} #1}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\numb}[1]{\num[group-separator={,}]{#1}}

\newcommand{\pats}{{\footnotesize\textsf{PATS}}\xspace}
\newcommand{\twota}{{\small$\mathsf{2TA}$}\xspace}
\newcommand{\ila}{{\small$\mathsf{ILA}$}\xspace}
\newcommand{\ilagap}{{\small$\mathsf{ILA}$-$\mathsf{GAP}$}\xspace}
\newcommand{\tkstt}{{\small\textbf{T$k$STT}}\xspace}
\newcommand{\canlist}{L_{\svar{it}}}
\newcommand{\ite}{it}

%\textbf for algorithm
%\textsf for distance 
%\texttt for dataset
%\mathbf for index
%\mathsf for algorithm
%\textsc for library or reference methods


%\usetikzlibrary{tikzmark}
%\usepackage[group-separator={,}]{siunitx}
\def\D{\hphantom{1}}
\def\C{\hphantom{1,}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\traclus}{{\small{\textsf{TRACLUS}}}\xspace}
\newcommand{\ebd}{{\footnotesize{\textsf{EBD}}}\xspace}
\newcommand{\eh}{\var{EH}}
\newcommand{\lh}{\var{LH}}
\newcommand{\alh}{\var{ALH}}
\newcommand{\kpath}{{\small{\textbf{$k$-paths}}}\xspace}
\newcommand{\kmeans}{{\small{\textbf{$k$-means}}}\xspace}
\newcommand{\indices}{{\small{$\mathbf{PIG}$}}\xspace}
\newcommand{\cpep}{{\small{$\mathsf{CPEP}$}}\xspace}
\newcommand{\lb}{lb}% the lower bound distance of each trajectory
\newcommand{\up}{ub}%
\newcommand{\centroid}{\mu}% the i-th medoid
\newcommand{\cluster}{C}% the set of trajectory 
\newcommand{\inverted}{II}% the inverted index of edge
\newcommand{\fre}{TF}% the frequency of edge in cluster
\newcommand{\edgefre}{ef}%ef_
\newcommand{\his}{H}% the histogram of edge in cluster H(i,e))
\newcommand{\assign}{a}% shows the assignment idx of a trajectory during the processing, in the end it will be the nc_1(j)
\newcommand{\neighborcenter}{nc}%n_3(i), 3rd nearest neighbor, dist(j, nc_1(j)) uses the id instead of T
%i is the idx of trajectory, T_i is the trajectory
%j is the idx of cluster
%e is the idx of edge
%a(i) is the assignment center id of i-th trajectory, j=a(i), which will be change.
%all the bounds are got from last iteration and used for current iteration.



\renewcommand{\labelitemii}{$\bullet$}
%\usepackage[authoryear,round,longnamesfirst]{natbib}
%\usepackage[numbers,sort]{natbib}

%\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
%\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{black}{#1}}
%\SetCommentSty{mycommfont}

\def\D{\hphantom{1}}
\def\C{\hphantom{1,}}
%\newcommand{\mycaption}[1]{\caption{\normalfont{#1}}}
\SetKwComment{Comment}{$\triangleright$\ }{}

\newcommand{\query}{{\small\textbf{MASK}}\xspace}
\newcommand{\tksk}{{\small\textbf{T$k$SK}}\xspace}
\newcommand{\ann}{{\small\textbf{ANN}}\xspace}
\newcommand{\kbct}{{\small\textbf{$k$BCT}}\xspace}
\newcommand{\atnn}{{\small\textbf{ATNN}}\xspace}
\newcommand{\mask}{{\small\textbf{MASK}}\xspace}
\newcommand{\baseline}{\textbf{2TA}}
\newcommand{\methodone}{\textbf{H2TA}}
\newcommand{\compare}{\textbf{BF}}
\newcommand{\ourindex}{{\small$\mathbf{TGP}$}}
\newcommand{\ouralgorithm}{{\small$\mathsf{ETAIL}$}\xspace}
\newcommand{\cachealgorithm}{{\small$\mathsf{RETAIL}$}\xspace}



\newcommand{\rknnt}{{\small\textbf{R${k}$NNT}}}
\newcommand{\knn}{{\small\textbf{${k}$NN}}\xspace}
\newcommand{\trknnt}{{\small\textbf{TR${k}$NNT}}}
\newcommand{\konn}{\textbf{${k}$ONN}}
\newcommand{\ctra}[1]{$C_{tra}[#1]$}%candidate set
\newcommand{\tc}[1]{$tc[#1]$}%trajectory code
\newcommand{\rl}[1]{$RL[#1]$}%ranking list of trajectory
\newcommand{\slice}{\textbf{SIR}}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\newcommand{\Sim}[2]{$Sim\left(#1,#2\right)$}%Similarity between two trajectories.
\newcommand{\ub}[2]{$UB(#1,#2)$}%upper bound of similarity bewtween two trajectories
\newcommand{\gs}[1]{$G_#1$}%group set of a trajectory 
\newcommand{\cg}[2]{$G_{#1}[#2]$}%group of one code 
\newcommand{\qgs}[1]{$QG_#1$}% quad group set
\newcommand{\cqg}[2]{$QG_#1[#2]$}% quad group of one code
\newcommand{\mqgs}[1]{$MQG_#1$}%merged quad gorup set
\newcommand{\cmqg}[2]{$MQG_#1[#2]$}%Merged quad group
\newcommand{\treeindex}[1]{{\em TCQ#1-tree}}
\newcommand{\rknn}{{\small\textbf{R${k}$NN}}\xspace}
\newcommand{\route}{\mathcal{R}}%route trajectory
\newcommand{\tran}{{T}}%transitions
\newcommand{\rs}{\mathcal{D}_{\route}}%route set
\newcommand{\ts}{\mathcal{D}_{\tran}}%transitions set
\newcommand{\tdist}[2]{\var{dist}(#1,#2)}%distance between route and transitions
\newcommand{\pdist}[2]{\var{distance}(#1,#2)}%distance between points
\newcommand{\hs}[2]{H_{#1:#2}} %half space
\newcommand{\sfill}{\mathcal{S}_{\svar{filter}}}
\newcommand{\scnd}{\mathcal{S}_{\svar{cnd}}}
\newcommand{\fr}{{\small$\mathbf{RR}$-$\mathbf{tree}$}\xspace}
\newcommand{\sr}{{\small$\mathbf{TR}$-$\mathbf{tree}$}\xspace}
\newcommand{\Gr}{{G}}
\newcommand{\br}{\mathcal{\var{BR}}}
\newcommand{\rknntm}{\mathcal{\var{RM}(\Gr)}}%RkNNT matric
\newcommand{\dm}{\mathcal{\var{DM}(\Gr)}}%Distance matric
\newcommand{\orgin}{v_s}
\newcommand{\destination}{v_e}
\newcommand{\rknntweight}[1]{\omega(#1)}
\newcommand{\maxrknnt}{{\small\textbf{MaxR${k}$NNT}}}
\newcommand{\minrknnt}{{\small\textbf{MinR${k}$NNT}}}
\newcommand{\traveldistance}[1]{\epsilon(#1)}
\newcommand{\planroute}{\mathcal{R}}%the planned route
\newcommand{\currentroute}{R^*}% the current route 
\newcommand{\candidatestop}{S^*}%the candidate stops
\newcommand{\srefine}{\mathcal{S}_{\svar{refine}}}
\newcommand{\tovisit}[1]{\var{toVisit}(#1)}
\newcommand{\connectivity}[2]{\mathcal{C}(#1,#2)}
\newcommand{\queue}{\mathcal{Q}}
\newcommand{\graph}{{G}}
\newcommand{\sresult}{\mathcal{S}_{\svar{result}}}
\newcommand{\sroute}{\mathcal{S}_{\svar{filterroute}}}
\newcommand{\mr}[2]{\mathcal{M}_\omega[#1][#2]}
\newcommand{\md}[2]{\mathcal{M}_\epsilon[#1][#2]}
\newcommand{\compareone}{\mathsf{FilterRefine}}
\newcommand{\comparetwo}{\mathsf{Voronoi}}
\newcommand{\comparethree}{\mathsf{DivideConquer}}
\newcommand{\maxcompareone}{\mathsf{Bruteforce}}
\newcommand{\maxcomparetwo}{\mathsf{Pre}}
\newcommand{\maxcomparethree}{\textbf{PreCPS}}
\newcommand{\rp}{r}
\newcommand{\tp}{p}
\newcommand{\crs}[1]{\mathcal{C}(#1)}
\newcommand{\scomment}[1]{\iffalse#1\fi}
\newcommand{\plist}{{\small\mathbf{PList}}}
\newcommand{\nlist}{{\small\mathbf{NList}}}
\newcommand{\revione}[1]{{\color{black}#1}}
\newcommand{\revitwo}[1]{{\color{black}#1}}
\newcommand{\revithree}[1]{{\color{black}#1}}

%\renewcommand{\cite}{\citep}
\newcommand{\todo}[1]{\textrm{\textcolor{blue}{To Do: #1}}}

\renewcommand{\labelitemii}{$\bullet$}
\newcommand{\MMTraj}{\overline{T}}
\newcommand{\mnth}[1]{\ensuremath{\mathnormal{#1}\cdot}th}
\def\D{\hphantom{1}}
\def\C{\hphantom{1,}}


\SetKwComment{Comment}{$\triangleright$\ }{}
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
%self-defined command
\newcommand{\tr}{{T}\xspace}
\newcommand{\segts}{\overline{T}\xspace}
\newcommand{\verts}{\ddot{T}\xspace}
\newcommand{\ds}{\mathcal{D}_T\xspace}

%name of query


\newcommand{\tss}{{\small{\textbf{TSS}}}\xspace}
\newcommand{\bts}{{\small{\textbf{BTS}}}\xspace}
\newcommand{\torch}{{\small{\textbf{Torch}}}\xspace}

\newcommand{\lors}{{\footnotesize{\textsf{LORS}}}\xspace}
\newcommand{\lcss}{{\footnotesize{\textsf{LCSS}}}\xspace}
\newcommand{\dtw}{{\footnotesize{\textsf{DTW}}}\xspace}
\newcommand{\erp}{{\footnotesize{\textsf{ERP}}}\xspace}
\newcommand{\edr}{{\footnotesize{\textsf{EDR}}}\xspace}

\newcommand{\levi}{{\small{$\mathbf{LEVI}$}}\xspace}
\newcommand{\vii}{{\small{$\mathbf{VerII}$}}\xspace}
\newcommand{\eii}{{\small{$\mathbf{EdgII}$}}\xspace}
\newcommand{\vgi}{{\small{$\mathbf{VGI}$}}\xspace}

\newcommand{\nb}{{--}\xspace}
\newcommand{\nc}{{--}\xspace}

\newcommand{\traid}{\var{traID}\xspace}
\newcommand{\edgid}{\var{edgID}\xspace}
\newcommand{\verid}{\var{verID}\xspace}



==> 1-Survey-trajectory 2/ack.tex <==
\section{Acknowledgments}

Identification of funding sources and other support, and thanks to
individuals and groups that assisted in the research and the
preparation of the work should be included in an acknowledgment
section, which is placed just before the reference section in your
document.

This section has a special environment:
\begin{verbatim}
  \begin{acks}
  ...
  \end{acks}
\end{verbatim}
so that the information contained therein can be more easily collected
during the article metadata extraction phase, and to ensure
consistency in the spelling of the section heading.

Authors should not prepare this section as a numbered or unnumbered {\verb|\section|}; please use the ``{\verb|acks|}'' environment.

==> 1-Survey-trajectory 2/advanced.tex <==
%\vspace{-0.5em}
\section{trajectory-boosted applications in urban planning}
\label{sec:application}

%Many city governments now use real-time analytics to manage aspects
%of how a city functions and is regulated \cite{Kitchin2014}.
Large-scale trajectory data is primarily collected in urban areas,
making it a valuable tool for applications in real-time smart
cities and timely decision making.
We will focus on four categories of applications which can benefit from trajectory data.
Table~\ref{tab:applications} provides a summary of representative
work in each of these broad areas.
To intuitively illustrate the connections between each of these, we also
provide several examples in Fig.~12.
Other examples can be found in the Appendix of \cite{Wang2020}.

\input{tableApplications}

\iffalse
\begin{figure}
	\centering
	\subfigure[Road traffic monitoring with range queries on the Porto collection \cite{Wang2019} ]{\label{fig:a}\includegraphics[width=0.32\textwidth]{graph/traffic-monitoring.png}}\hspace{3em}
	\textbf{\subfigure[Transit network planning with commuter trajectory data to cater to new travel demands \cite{Wang2018c}]{\label{fig:b}\includegraphics[width=0.4\textwidth]{graph/bus-route.pdf}}}\\ %\vspace{-1em}
	\subfigure[Trajectory-based queries for travel planning and interest discovery for a tourist visiting Los Angeles~\cite{Wang2018a}]{\label{fig:c}\includegraphics[width=0.58\textwidth]{graph/trip-planning.pdf}}\hspace{3em}
	\subfigure[Site selection of billboards to maximize commuter views~\cite{Zhang2019a}]{\label{fig:d}\includegraphics[width=0.29\textwidth]{graph/billboard.pdf}}
	%\vspace{-1em}
	\caption{Examples of four urban applications for trajectory data.}
	%\vspace{-2em}
	\label{fig:four-apply}
\end{figure}
\fi

\vspace{-1em}

\subsection{Applications in Road Traffic}
Cities and government agencies are often a valuable source of
trajectory data.
There has been an increased emphasis on collecting data from traffic
signals and other related sensors for internal auditing purposes, and
regulatory requirements often require the data collected to be made
publicly available since it was gathered using tax income.
Such data can be used for traffic monitoring \cite{Wang2019}, anomaly
detection \cite{Wang2018f}, and traffic jam and flow analysis
{\cite{Wang2013f}}.

%Liu2017c,Chen2015,Wang2013f,Wang2019,Fan2016,Wang2018f,

\myparagraph{An Overview}
%\shane{I don't fully understand the goal of this paragraph or the
%"commonality" label. It seems kind of redundant.}
Fig.~\ref{fig:pipeline-road} shows the pipeline of three
representative trajectory analytical tasks for road traffic.
As a common operator, mapping trajectories onto road networks not
only cleans the data, but also enables traffic jam and flow analysis
in real time.
%\shane{Arguably this might come first in this section to connect the work
%that is being covered and provide context.}
%Critical performance improvements in similarity search and clustering
%operations on mapped trajectory data can be achieved when mapping
%trajectory to a series of road segments.


\subsubsection{Traffic Monitoring}
{Since trajectories record the trace of vehicles in the road,
many visualization systems \cite{Chen2015} were 
developed to observe and monitor past or real-time traffic trends and movement patterns
based on trajectory data. Users can interactively explore the traffic condition in a specific area or road, and further control the traffic if necessary.}
As visualizing an entire city-wide trajectory dataset on a single screen can
be unreadable, selecting an area and identifying the trajectories
covered is a useful application of a range query, which was described
in Section~\ref{sec:spatialonly}.
In addition to a range query, a wide variety of {\em trajectory
search} queries
\cite{Chen2005a,Krogh2016,SanduPopa2011,DeAlmeida2005,Koide2015,Roh2011}
have been proposed over the years to support various applications.
To monitor all vehicles that use \textit{a Main Street}, a
\textit{{path query}} \cite{Krogh2016} can be issued.
Further, a \textit{{strict path query}} identifies
every vehicle that traverses all of \textit{a Main Street}.
\citet{Wang2019} integrated all the above queries into a real-time
traffic monitoring system, where user can interactively conduct
queries and get results in real time.

\iffalse
These three kinds of queries are 
\textbf{\textit{basic trajectory search queries}}.
Given a trajectory, a \textit{{top-k trajectory similarity
		search query}} returns the $k$ highest ranked trajectories based on a
similarity metric~{\cite{Xie2017a}}, which can be used to
investigate driving habits \cite{Chen2010a}, cluster trajectories to
discover popular routes~{\cite{Won2009}}, or search over all of the
trajectories which have a pre-specified trajectory as a $k$ nearest
neighbors -- a task used in transportation route
planning~{\cite{Wang2018c}}.


\shane{I think all of the above text is taken verbatim from a
published paper. If so, it needs to be reworded or it could
get flagged as plagiarism, albeit self.}
\fi



\input{traffic-method}

\subsubsection{Traffic Jam and Flow Analytics}
\iffalse
\shane{While better, I still think this subsection is really high
level. No real information on the algorithms or indexes is provided.
I still haven't seen a single piece of pseudocode that captures
an important concept.}
\fi

Live traffic monitoring enables analysts to track usage of
specific roads or areas in real time, and can be used to identify
traffic jams in order to notify commuters through digital traffic
signs or GPS applications.
%For example, Google Maps provides a view of traffic with red areas
%indicating poor traffic conditions.
%The main challenge in real-time traffic jam detection is how to
%dynamically apply map-matching efficiently and precisely.
%\citet{Hashemi2014} recently surveyed real-time map matching in
%detail, and we do not explore this important problem
%further here, but there still are many interesting work \cite{Rappos2018} proposed recently.
%\shane{Have there been new advances? Is it worth
%at least summarizing the most important lessons learned in that
%work for completeness?}
After mapping trajectory data to a road network, {\citet{Wang2013f}}
visually inspected traffic data and verified problem areas based
on speed limit information of the streets under consideration.
%\shane{This was entirely manual or semi-automated?}

Instead of inspecting individual road segments to identify
traffic jams, traffic flow analysis does not rely on domain-specific
features such as speed limits.
The goal is to discover important movement patterns of drivers such
as repeatedly using a common route composed of several different road
segments.
Several recent papers have proposed concept definitions that capture
essential properties of traffic flow analysis based on trajectories.
\citet{Gudmundsson2006} defined the concept of a \textit{flock},
which is a common sub-trajectory covered by a set of trajectories
with at least $k$ circles with the same-radius.
% \shane{Can't visualize this.}
\citet{Jeung2008} extended the concept of a \textit{convoy}, where
the circles can have various radii.
%\shane{Same. Seems
%like a generalization of the above but not enough information to really
%understand why these concepts matter or what they do.}
\citet{Li2010c} proposed the concept of a \textit{swarm} to solve the
problem that a sub-trajectory has to be a continuous set of points in
the corresponding trajectory.
%non-consecutive.
%\shane{non-consecutive commented out as it is not clear what it means here.}
%\citet{Tang2012} defined a similar concept called a \textit{trajectory
%companion} for streaming environments, which is essentially the online
%identification of similar trajectories. \shane{How do they differ?}
%\citet{Yadamjav2019} defined a problem of finding recurrent pattern
%of co-moving objects from streaming trajectories.
%\shane{Not a concept and really just another bullet point you need to
%expand. The problem a paper proposes is not interesting without an
%understanding of the solution.}
%All of the above work locates a set of objects which persist for at
%least $k$ (possibly non-consecutive) timestamps.
Rather than a single sub-trajectory, \citet{Zheng2014a} proposed the
concept of \textit{gathering}, which returns multiple
sub-trajectories.
To further avoid specifying multiple hyper-parameters, e.g., the
number of circles, {\kpath} trajectory clustering will return $k$
most representative trajectories (real paths on road network)
\cite{Wangaclustering}, which can be used in the traffic flow
analysis.

%maybe solution

%\shane{Nope. The stuff below this isn't appropriate. It isn't objective.
%Parameters are not evil. If none of the above is related to road networks
%why include them at all. Isn't road networks the scope?}
%However, none of them are based on the road network, and they also
%need several parameters and are not applicable.
%Instead, a \kpath trajectory clustering will return $k$ most
%representative trajectories (real paths on road network)
%\cite{Wangaclustering}, which can be used in the traffic flow
%analysis without specifying hyperparameters.

\subsubsection{Anomaly Trajectory Detection}
Anomaly or outlier trajectories in a dataset can be defined as
a trajectory that falls outside of a predefined confidence
interval w.r.t. the entire collection distribution.
It has be applied in applications such as identifying criminal
behavior in a population~\cite{Shen2015} and taxi driver fraud
detection~\cite{Wang2018f}.
A combination of similarity and clustering can be used to
solve this problem.
Computing similarity between trajectories can be used to identify
trajectories that are the most dissimilar in a dataset, and
clustering can be used to aggregate common trends that might not be
easily identifiable otherwise.
For example, given an incoming trajectory $T$ between a source $s$
and a destination $d$, anomaly detection was defined by
\citet{Chen2012a} as: 1) the anomaly score of $T$ based
on the proportion of existing trajectories in $D$ passing through $s$
and $d$ and covering $T$ completely; 2) a predefined threshold
$\theta$ to determine if $T$ is anomalous or not.
The similarity measures are based on two types of information:
1) sub-trajectories~\cite{Lee2008a}; 2) entire
trajectories~\cite{Chen2012a,Wang2018f}.
\citet{Lee2008a} detected outliers using line segments, i.e.,
a trajectory was partitioned into a set of line segments, and then,
outlying line segments were used to find trajectory outliers.
\citet{Wang2018f} utilized an edit-based similarity measure to detect
anomalies in a hierarchical cluster arrangement.
%\shane{More.
%Now mixing ML and non-ML too. It is not clear how this optimization
%worked. That would be the secret sauce.}



\subsection{Applications in Green Transport}
Public transportation networks such as subways, bus routes, and gas
stations provide more choices for green commuting.
Trajectory data is commonly applied in green transport (also known as ``sustainable transport''
\cite{Schiller2017}) applications to optimize network design, conduct
personalized and adaptive navigation, and carpooling.
Note that this survey focuses on algorithms and complexity,
and we also refer the interested readers to a review which covers this problem in detail
\cite{Markovic2019} for a more comprehensive view from the
perspective of road transportation agencies.

\myparagraph{An Overview} 
%\shane{Still a weird transition name and you didn't really think
%about it.
%I think these are actually overviews and should come before each of
%the detailed breakdowns in my opinion.}
Based on these examples, we observe that a critical task in road networks is
trip planning or finding common routes in a graph for a passenger or
a driver, as shown in Fig.~\ref{fig:pipeline-transport}.
Complex route planning problems typically maximize a capacity or
minimize a travel time.
When viewed this way, many of the problems encountered are NP-hard,
reducible to the traveling salesmen problem, and solved using a
greedy algorithm.

%\shane{Is this what all of the above actually did?}



\input{transport-pipe}

\subsubsection{Transit Network Planning}
By mining taxi data, \citet{Chen2014a} approximated night
time bus route planning by first clustering all points in taxi
trajectories to determine ``hot spots'' that could be bus stops, and
then created bus routes based on the connectivity between two stops.
{\citet{Toole2015162} used census records and mobile phone location
information to estimate demand in transit routes.
Historical traffic data~\cite{6878453}, smart cards~\cite{Zhang2017},
sensors~\cite{Lv2014}, and cellular data~\cite{Pinelli2016} can
provide more comprehensive demand data and be used to further improve
data-driven transit network design.
\citet{Pinelli2016} derived frequent patterns of movement from
trajectories by computing distance and the flow gain, then merge them
to generate a network for the whole city.
A common shortcoming of these methods is that they are building a new
network, and are not applicable for most cities which already have
bus networks.
Based on human mobility patterns extracted from taxi data and smart
card data, \citet{Liu2016} proposed a localized transportation choice
model, which predicted travel demand for different bus routes by
taking into account both existing bus network and taxi routes.
%\shane{No insight into why any of these problems were hard or how
%they were solved.}

\subsubsection{Adaptive Navigation}
Travel distance-based shortest path search between a source and
destination is widely used in navigation services.
It can be applied adaptively using historical trajectory data from
drivers.
With precise map matching techniques, discovering trajectory paths
in data can enrich models for a road network, e.g., dynamic time
cost of each road~\cite{Dai2016}, driver preferences
\cite{Guo2018a}. %\shane{Not sure what time cost in various hours
%means.}
Using a dynamic travel time cost for each road segment, travel time
estimation \cite{Dai2016} and fastest path search \cite{Wang2019c}
is more realistic, capturing various traffic conditions, and
potentially leading to alternative shortest paths when all aspects
are considered.
\citet{Guo2018a} proposed learning to route with sparse trajectory
sets, by constructing a region graph of transfer routing preferences.
In the graph, the nodes are equal-size grids, and the edges represent
two grids crossed by more than a fixed number of trajectories.
%\shane{Not clear what they did with this.}
Discovering preferences from trajectories can also be used
to support personalized route recommendation for green vehicle
routing~\cite{bektacs2016green}. 
\citet{Dai2015} developed techniques to support efficient
trajectory subset selection for following using 
driver preferences (travel distance, travel time, and consumed fuel)
and the source, destination, and departure time specified by the
driver. %\shane{Learned? How? More.}
\citet{Delling2016} proposed a framework to generate personalized
driving directions from trajectories, where the path preferences 
were composed of several features, such as avoiding tolls, U-turns,
and highway versus surface streets.
%Preferences were represented as a vector and unsupervised learning
%was applied.
%\shane{More. Is this clustering? If not have you diverged from the
%original scope?}

\subsubsection{Carpooling}
There are two common approaches to ridesharing problems which rely
heavily on trajectory data.
The first one is grouping passengers and drivers based on their
historical trajectory data.
The underlying goal is to keep all seats in all vehicles occupied,
and is essentially a type of bin packing problem.
For example, \citet{Hsieh2017} devised a carpooling system to match
passengers and drivers based on their travel trajectories, and the
similarity measure was defined as the sum of the distance from the
pickup and drop off points to the nearest point to a driver
trajectory.
The other approach is to detect frequent routes using only rider
trajectories.
\citet{He2014} proposed a carpooling system that generates an
efficient route for dynamic ridesharing by mining the frequent
routes taken by participating riders.
\citet{Hong2017} performed rider matching by clustering trajectories,
and generated a simulation model of ridesharing behaviors to
illustrate the potential impact.
%\citet{Cruz2018} proposed an innovative approach to generate clusters
%of users that share similar trajectories and profile for carpooling
%purposes.
Similar to other road traffic applications, similarity computations
are performed between passenger and driver trajectories, clustering
is then used to detect the frequent routes shared by multiple
passengers in the trajectory-driven carpooling.
%\shane{No insight. As written, there is no obvious difference between
%the last two.}




\subsection{Applications in Tourism Planning}
The tourism market is an enormously valuable commodity in many
countries.
For example, this market in Britain is expected to be worth more than 
£257 billion by 2025, and represents 11\% of the total GDP of the
UK.\footnote{\url{https://www.visitbritain.org/visitor-economy-facts}}
%So it should come as little surprise that research targeted to improve
%this valuable commodity is plentiful.
From a consumer perspective, historical trip data can also improve
overall satisfaction, and provide tools to discover more personalized
opportunities that align with individual preferences.


\subsubsection{Customizing Tours}
Searching for similar trips related to a set of given points with
keywords \cite{Wang2017,Zheng2013c,Zheng2015}, or a range
\cite{HanWZZL15} can enable more effective zero knowledge querying
capabilities, as we described in Section~\ref{sec:spatialtextual}.
In addition to spatial proximity and text relevance, other factors
can be considered, such as photos \cite{Lu2010a}.
\citet{Lu2010a} leveraged existing travel clues recovered
from 20 million geo-tagged photos to suggest customized travel route
plans according to user preferences.
\citet{Wei2013} developed a
framework to retrieve the top-$k$ trajectories that pass through
popular regions.
%\citet{Yan2014} considered the importance of location when defining
%the similarity measure. \shane{and???}
%Given a set of targets, obstacles, and trajectories, the $k$ Aggregate
%Maximum Visibility Trajectory query \cite{Tripto2019} finds the
%top-$k$ trajectories that provide the best view of the targets.
%\shane{This is related to trip planning how?}
%\subsubsection{Customizing Tours}
Rather deriving search results using only existing trips, generating
new trip plans without keywords or locations is also
possible. % \shane{How did they do it.}
%Another approach taken was casting the problem to that of road
%network navigation~\cite{Dai2015}. \shane{How did it help specifically?}
\citet{Chen2011a} discovered popular routes from spatial-only
trajectories by constructing a transfer network from trajectory data
in two steps.
First, hot areas are detected as nodes in the network; then edges are
added based on connectivity properties in the entire trajectory
collection.
Then, a network flow algorithm was proposed to discover the most
popular route from the transfer network.
%\shane{Why is this good? Efficiency? Scalability? More.}
%\citet{Luo2013} generated frequent paths by
%integrating temporal information. \shane{More}
%\citet{Liang2018b} studied top-$k$ route search over a Foursquare
%check-in dataset, and integrated diversification directly into
%the similarity computation. \shane{How? More.} 
\citet{Wang2018b} developed an interactive trip planning system
called TISP, which enabled interesting attractions to be
discovered, and used to dynamically modify recommendations using
click-based feedback from POIs displayed on the map.

\input{toursim-pipe}

\subsubsection{User Interest Discovery}
\iffalse
\shane{Still needs more details on the actual algorithms and indexes
being used. Be specific. You are still bullet pointing problem after
problem with very little insight into why the {\em solutions} were
novel. I am skeptical CSurv will find the depth sufficient.}
\fi
When a trajectory is enriched with text, it is possible to discover
more useful patterns by leveraging semantic information as well as
human interaction.
Interest discovery is a valuable tool to improve the effectiveness of
recommendations for restaurants, attractions, or public event to
tourists.
The three most common categories of interests discovery using
trajectory data for tourism are: 1) point of interest (POI)
\cite{Giannotti2007}; 2) region of interest (ROI)
\cite{Uddin2011,Jarv2018}; and 3) interactive discovery
\cite{Brilhante2015a,Wang2018a}.
\citet{Palma2008} discovered interesting locations from trajectories
using a spatiotemporal clustering method, based on the speed of
single trajectories. % \ shane{More detail.}
\citet{Uddin2011} presented a generalized ROI definition for
trajectories which is parameter independent, and an efficient index
over the segments by speed was proposed to find the ROIs without
scanning the whole dataset.
%\shane{What index what is the role of data independent
%parameters here? Not clear.}
%\citet{Jarv2018} extended this idea to Hierarchical ROIs to enable
%semantic annotation, 
\citet{Brilhante2015a} utilized Wikipedia content, trajectories over
georeferenced Flickr photos, and human feedback to discover a
``budget-constrained sightseeing tour'' using a tourist's preferences
and available time.
\citet{Wang2018a} proposed a unified index, composed of inverted
index and grid index, to find POIs, including attractions, hotels,
and restaurants, to achieve fast performance for real-time response.
%\citet{Oliveira2018} solved the orienteering problem with hotel
%selection in several cities, taking advantage of the tourist
%trajectories extracted from location-based services.
%\shane{How? More.}

%{Friggstad2018} define a new trip planning algorithm by maximizing the benefit of the worst day rather than maximizing the sum of benefits of all days. 

\subsubsection{Semantic Pattern Mining}%add this to be part of tourism

Generally, semantic pattern mining aims to mine the frequent movement
with descriptive text information, which is more comprehensive than a
spatial-only route.
\citet{Zhang2014a} discovered fine-grained sequential patterns which
satisfy spatial compactness, semantic consistency and temporal
continuity simultaneously from semantic trajectories.
The algorithm first groups all the places by category and retrieves a
set of coarse patterns from the database, then splits a coarse
pattern in a top-down manner.
Instead of two steps in \cite{Zhang2014a}, \citet{Kim2015b} presented
a latent topic-based clustering algorithm to discover semantic
patterns in the trajectories of geo-tagged text messages.
However, the above method can only work over trajectories with texts.
%\citet{Chen2016c} extract the semantic attributes from raw
%spatial-only trajectories and convert the trajectories into
%semantic trajectory sequences.
%The semantic attributes are generated from a set of semantic tags by
%the geographic API, check-in data, or tweets.
%Instead of mining semantic pattern in the entire spatial area,
\citet{Choi2017} studied a regional semantic trajectory pattern
mining problem, aiming at identifying all the regional sequential
patterns in semantic trajectories.
%\citet{Cai2018} proposed an itinerary recommender system with semantic trajectory pattern mining from geo-tagged photos by discovering sequential points-of-interest with temporal information from other users’ visiting sequences and preferences.
Semantic pattern mining was not covered in previous
surveys~\cite{Parent2013a, Zheng2015}.
Trajectory pattern mining was grouped into four categories 
by \citet{Zheng2015}: 1) co-movement pattern which has been described
in the traffic flow analytics, e.g., the convoy, flock, group,
gathering; 2) trajectory clustering (check
Section~\ref{sec:clustering}); 3) sequential patterns which indicate
a certain number of moving objects traveling a common sequence of
locations in a similar time interval; 4) periodical patterns which
indicate periodic behaviors for future movement prediction.
%We will not
%\citet{Wan2018} designed a probabilistic generative model with latent variables to characterize the semantic mobility of vehicles. Based on the model, SMOPAT labels each location in a trajectory with a visit purpose by using a polynomial-time dynamic programming algorithm.

\iffalse
\myparagraph{Insights}
%\shane{Very little useful information in this paragraph really.
%Drop it entirely IMO.}
In tourism applications, keywords are pervasive in the trajectory
data, but trajectory data is often sparse, and map matching is not
necessary.
%Trip search is similar to searching spatial-only trajectories, but
%often text plays a more significant role.
Human interaction is also essential for effective tourism planning,
as lack of personalization often leads to undesirable results.
\fi
\begin{table}
	\centering
	\caption{Recent work on trajectory-driven site selection.}
	\vspace{-1em}
	\scalebox{0.75}{
	\begin{tabular}{ccccccccc}
		\toprule	\addlinespace[0pt]\rowcolor{gray!30}\rowcolor{gray!30}
		& \textbf{Work} & \textbf{Constraint} & \cellcolor{gray!30} \textbf{\makecell{Extra Input Data\\besides Trajectory}}& \textbf{\makecell{Road\\ Network}} & \textbf{\makecell{The Objective \\Function}} & \textbf{\makecell{The Reduced \\NP Problem}} & \textbf{\makecell{ Accelerating \\Strategies~~~~}} & \textbf{Guarantee} \\ \addlinespace[0pt]\midrule
	\multirow{7}{*}{\hspace{-4em}$\left. {\ref{sec:charging}}\begin{array}{l}
		\\
		\\
		\\ \\ \\ \\ \\ 
		\end{array}\right\lbrace{}$} 	& \cite{Li2015c} & $k$ stations & \makecell{existing stations,\\\#charging points} & \cmark & \makecell{travel time,\\waiting time} & \makecell{ integer\\ programming} & LP-rounding & N/A \\
		 &\cite{Han2016} & $k$ stations & \makecell{+\\battery\\ performance} & \cmark & \makecell{+\\installing cost,\\charging cost,\\ waiting time} & - & \makecell{evolution \\algorithm} & - \\
		 &\cite{Liu2017d} & \makecell{for the \\whole city} & \makecell{ petroleum\\ stations, POIs,\\ real-estate} & \cmark & \makecell{revenue, \\queueing time} & \makecell{bilevel \\optimization} & \makecell{ alternating \\framework} & \makecell{ local\\ minima} \\ \midrule
		\multirow{12}{*}{\hspace{-4em}$\left.\ref{sec:billboard}\begin{array}{l}
		\\
		\\
		\\ \\ \\ \\ \\ \\ \\ \\ \\ \\ \\
		\end{array}\right\lbrace{}$} 	& \cite{Guo2017} & $k$ billboards & \makecell{bus \\advertisement, \\bus station \\audiences} & \xmark & influence & set-cover & \makecell{index,\\expansion,\\upper bound} & $1-1/e $ \\
		& \cite{Liu2017c} & \makecell{budget or\\ $k$ location} & \makecell{traffic volume,\\ speed} & \xmark & \makecell{coverage\\ value} & \makecell{ maximum\\ coverage} & \makecell{ inverted\\ index,\\greedy\\ heuristic} & $1-1/e $ \\
	&	\cite{Zhang2018c} & budget & \makecell{billboards' \\price} & \xmark & \makecell{one-time \\ impression } & \makecell{set cover\\ problem} & bound & $1-1/e $ \\
	&	\cite{Zhang2019a} & budget & \makecell{billboards' \\price} & \xmark & \makecell{ logistic \\influence} & \makecell{ biclique\\ detection} & \makecell{branch-\\and-bound} & $\frac{\theta}{2}(1-1/e)$ \\
	&	\cite{Wang2019a} & $k$ & \makecell{advertisement\\ topics,\\ traffic conditions,\\ mobility transition} & \cmark & \makecell{influence \\spread} & \makecell{weighted\\ maximum\\
		coverage} & \makecell{divide-\\and-conquer} & N/A \\ \midrule
	\multirow{7}{*}{\hspace{-4em}$\left.\ref{sec:facility}\begin{array}{l}
	\\
	\\
	\\ \\ \\ \\ \\ 
	\end{array}\right\lbrace{}$} 	&	 \cite{Bao2017a} & \makecell{ budget,\\construction \\cost,\\utilization} & \makecell{ bike\\ trajectories} & \cmark & \makecell{ beneficial \\score} & \makecell{ 0-1 knapsack\\ problem} & \makecell{ greedy \\network \\expansion,\\inverted \\index } & N/A \\
	&	\cite{Wang2018c} & \makecell{travel \\distance} & \makecell{ node\\ capacity } & \cmark & \makecell{ route \\capacity } & \makecell{constrained \\shortest\\ path search } & \makecell{divide-\\and-conquer} & exact \\
	&	 \cite{Li2018d} & \makecell{ source, \\destination } & \makecell{ parking \\edges } & \cmark & \makecell{on-road\\ travel time } & \makecell{ shortest \\path search} & \makecell{incremental \\expansion } & exact \\ \midrule
		\multirow{3}{*}{\hspace{-4em}$\left.\ref{sec:general}\begin{array}{l}
		\\
		\\
		\\ \\ \\ \\
		\end{array}\right\lbrace{}$} &	\cite{Wang2016g} & \makecell{$k=1$ } & \makecell{probability \\threshold } & \xmark & \makecell{cumulative\\ influence\\ probability } & - & \makecell{filter-\\and-validate} & exact \\
	&	 \cite{Li2016g} & $k$ & - & \cmark & \makecell{\#covered \\unique \\trajectories} & max-$k$-cover & \makecell{group \\pruning} & $1-1/e $ \\
	&	\cite{Mitra2017} & $k$ & \makecell{Existing\\facilities} & \cmark & \makecell{User \\inconvenience} & k-center & best-first & $1-1/e $ \\ 
%	&	 \cite{Ali2019} & $k$ & bus routes & \xmark & service value & \makecell{maximum\\ coverage} & \makecell{divide-\\and-conquer} & \makecell{no proved \\ratio} \\
	 \bottomrule
	\end{tabular}}
	\label{tab:site-select}
	\vspace{-1.5em}
\end{table}

\subsection{Applications in Site Selection}
As a core decision-making tool, trajectory-driven site selection has
been a crucial factor in increasing business profit and public
service quality.
%Compared with point-based site selection methods such as
%the \textit{reverse $k$ nearest neighbor query}~\cite{Tao2004}, a 
%trajectory allow more informative decisions.
Using collected trajectory data to estimate the influence of
selected sites for drivers or passengers can be applied to
problems such as charging
station placement~\cite{Li2015c}, billboard placement~\cite{Guo2017}, 
%bike station redeployment~\cite{Zhang2016f}, 
and facility route design~\cite{Wang2018c}.
%Specific constraints can also be applied, such as the total number of
%available stations or total budget costs.

\begin{definition}\textbf{(Constrained Site Selection)}
Given a set of trajectories $D$, a set of facilities $F$, a
constraint value $C$, and an influence model ($IM$), the aim of
constrained site selection is to find a subset $S \subset F$ to that
satisfies an objective function: $O = \argmax_{cost(S)<C} IM(S, D)$.
\end{definition}

Different objective functions can be defined based on the exact
scenario.
In Table}~\ref{tab:site-select}, we compare recent work in this area
in terms of constraints, input data, map matchability, objective
function, NP-hardness reduction, acceleration strategies, and
approximation guarantees.


\input{site-pipe}

\myparagraph{An Overview} Fig.~\ref{fig:pipeline-site}
illustrates common connections between various site selection problems.
Site selection definitions can change based on a specific problem
scenario and may cover a singe dataset or multiple datasets.
The general problem is NP-Hard by reduction to the set cover problem,
and even approximate solutions tend to scale poorly.
Bounded or greedy algorithms can be used to accelerate the processing
along with expansion-based methods, such as estimating the bound for
all remaining set candidates by incrementally adding a single
facility and comparing it against current result to determine whether
expansion can be safely terminated.

\subsubsection{Charging Station Deployment}
\label{sec:charging}

Given the increasing popularity of electric vehicles, building more
charging stations has become a crucial problem.
Trajectory-driven charging station deployment aims to reduce the
detour distance required for charging.
\citet{Li2015c} developed an optimal charging station deployment
framework that uses historical electric taxi trajectory data,
road map data, and existing charging station information as input.
Then, it performs charging station placement and charging point
assignment (each charging station has multiple changing points).
% \shane{How do the last two differ? More
%solution details. I removed optimal. If it was NP-Hard and then
%approximated, it is not an optimal solution...}
The objective function is designed to minimize the average time to
the nearest charging station, and the average waiting time for an
available charging point, respectively, which can be reduced to the
\textit{integer linear programming (ILP)} problem
\cite{schrijver1998theory} that is NP-hard.
%\shane{Cite to NP-Hardness?}
%\shane{How exactly?}
%\citet{Han2016} developed an algorithm for charger placement based
%on charger installation costs and waiting delay using an evolutionary
%algorithm.
%\shane{Which one? You are back in ML world. What is the scope?}
\citet{Liu2017d} aimed to achieve two goals: (i) the overall revenue
generated by the EVCs is maximized, subject to (ii) the overall
driver discomfort (e.g., queueing time) for EV charging is minimized.
Hence, the charging station deployment is defined as a
multiple-objective optimization problem.

\subsubsection{Billboard Placement}
\label{sec:billboard}

Billboard placement aims to find a limited number of billboards which
maximize the influence on passengers and further increase profits.
Recently, several studies
\cite{Zhang2018c,Liu2017c,Guo2017,Wang2019a,Zhang2019a} have investigated
trajectory-driven billboard placement.
\citet{Guo2017} proposed the top-$k$ trajectory influence
maximization problem, which aims to find $k$ trajectories for
deploying billboards on buses to maximize the expected influence
based on the audience.
The model of \citet{Liu2017c} was based on traffic volume.
More specifically, the algorithm counts how many
trajectories traverse an edge or vertex containing a billboard,
and then identifies the $k$ most frequent for billboard placement.
\citet{Zhang2018c} applied a model on range and one-time impressions,
constrained by total budget available for billboard placement.
\citet{Zhang2019a} proposed a logistic influence model
which solves a key shortcoming in approaches that depend on 
one-time impressions~\cite{Zhang2018c}, which did not consider the
relationship between the influence effect and the impression counts
for a single user.
%\shane{What is the shortcoming?}
\citet{Wang2019a} placed billboards in a road network, and applied a
divide-and-conquer strategy to accelerate the processing.
%\shane{All bullet pointing. Insights please.}
As we conclude in Table~\ref{tab:site-select}, billboard placement
problem definition always have a budget, and it is also general for
other site selection problem in reality as public resource allocation
also needs to be considered in the budget.

\subsubsection{Facility Route Planning}
\label{sec:facility}
Instead of pointwise candidate set selection, a facility set can also
be routes covering multiple candidates, such as planning bike lanes
and route search.
\citet{Bao2017a} designed bike lanes based on bike trajectories,
where the constraint is a budget and the number of connected
components.
A greedy network expansion algorithm was proposed to iteratively
construct new lanes to reduce the number of connected components
until the budget is met.
\citet{Wang2018c} proposed the use of MaxRkNNT for planning bus
routes between a given source and destination using a route capacity
estimation query called \rknnt.
The key constraint is travel distance, and the objective function
maximizes the estimated capacity of the routes.
%\citet{Li2018d} proposed a new routing solution that 
%identifies parking facilities available in order to avoid traffic
%jams using historical trajectories, and further to minimize the
%on-road travel time. \shane{How can historical data predict a traffic
%jam? There is a global objective function that maximizes flow? More.}
Using transit trajectories, \citet{Wu2018c} defined various objective
functions for passenger preferences, and evaluated new transit routes
based on multiple factors on a real-world transport network,
including monetary cost, time cost, number of transfers, number of
choices, and transit mode.

 %\shane{Scope? No insight how or what they actually did here.}

\subsubsection{General Site Selection}
\label{sec:general}

There are several general site selection studies that are not limited
by any one scenario.
Instead of setting a cost budget, it may be more desirable to set a
parameter $k$ to choose a set of facilities from the candidate set.
Specifically, \citet{Wang2016g} aimed to identify the optimal
location ($k=1$) which can influence the maximum number of moving
objects by using the probabilistic influence.
An exact algorithm based on filtering-verification is proposed to
prune many inferior candidate locations prior to computing the 
influence.
%\shane{Provably optimal or
%approximate?}
\citet{Li2016g} identified the $k$ most influential locations
traversed by the maximum number of unique trajectories in a given
spatial region with an efficient algorithm to find the location set
using a greedy heuristic, in cases where $k$ and the spatial areas
are large.
\citet{Mitra2017} solved the trajectory-aware
inconvenience-minimizing placement of $k$ facility services which was 
proved to be NP-hard \cite{Chan2018}. %\shane{Again cites for these proofs is desirable}
The inconvenience is defined as the extra distance traveled to access the nearest facility location.% \shane{avail ?}
%An exact algorithm based on integer linear programming is proposed first to
%\citet{Ali2019} proposed two new coverage queries for trajectory
%databases: (i) $k$ Best Facility Trajectory Search ($k$BFT); and (ii)
%$k$ Best Coverage Facility Trajectory Search ($k$BCovFT), where a
%service value is computed and maximized. \shane{Solutions please.}


%\shane{Again.
%I think the categorization should be coming first to make it clear
%why these things are all here.}



==> 1-Survey-trajectory 2/conclusion.tex <==
\section{Conclusion}
\label{sec:conclude}
In this survey, we have reviewed recent progress in trajectory data
management and learning.
We first presented an overview of trajectory data management and
urban applications.
Then, we categorized the problems based on components and operators
shared across the tasks.
Similarity measures, top-$k$ similarity search, and fast clustering
are all widely used for many different problems and scenarios, and
were the focus of this study.
Finally, we reviewed important research advances on four common
analytics applications of trajectories for real-time smart cities.
New applications emerge daily that leverage trajectory data, such as
deep trajectory learning, and we hope this survey can provide readers
an overview of the landscape of trajectory data management and
applications.
Perspectives on how to choose the most appropriate solution for
pre-processing, storage, search, and advanced analytics to achieve
high efficiency and effectiveness can be applied in many different
problem domains beyond road networks.


%\myparagraph{Acknowledgment}

\vspace{-0.5em}
 \begin{acks}
Zhifeng Bao is supported in part by ARC DP200102611, DP180102050, and a Google Faculty Award.
J. Shane Culpepper is supported in part by ARC DP190101113.
Gao Cong is supported in part by a MOE Tier-2 grant MOE2019-T2-2-181, and a MOE Tier-1 grant RG114/19.
\end{acks}

==> 1-Survey-trajectory 2/deep-tab.tex <==
\begin{table}
	\ra{-0.5}
	\centering
	\caption{Recent work on deep trajectory learning.}
%	\vspace{-1em}
	\scalebox{0.82}{
	\hspace{-3em}	\begin{tabular}{ccccccccc}
		\toprule	\addlinespace[0pt]\rowcolor{gray!30}\rowcolor{gray!30}
		  \textbf{Work} &   \textbf{Tasks} & \textbf{Data sources}  & \textbf{\makecell{~~~Encoder/Input}} & \cellcolor{gray!30} \textbf{\makecell{Decoder/Output}} & \textbf{\makecell{Deep Model}} & \textbf{\makecell{More Feature}} & \textbf{\makecell{Loss Function}} \\ \addlinespace[-1pt] \midrule

		\cite{Wang2019i} & Data recovery  & Taxi  & LSTM  & BiLSTM &  seq2seq & \makecell{Spatial \\temporal\\ attention} & softmax \\
		\cite{Ouyang2018} &\makecell{Synthetic data \\generation} & Mobile GPS& \makecell{Matrix \\representation}&  \makecell{matrix \\representation} &GAN &\makecell{Semantic \\ duration}&WGAN-GP \\ 
%		\cite{Systems2017} &  \makecell{Mobility \\simulation}& Cellular data&IO-HMMs&  \makecell{Distribution\\ coefficients}&GAN-LSTM &\makecell{Activity \\Features}&\\
		\makecell{\cite{Liu2018}} &\makecell{Privacy \\protection}& APPs&Embedding& \makecell{Random\\ deviations}&CGAN&POI &minimax\\
		\makecell{\cite{Gupta2018} }&\makecell{Mobility \\prediction}& Video&LSTM&LSTM&GAN&Pooling&L2\\\midrule
		
		\cite{Li2018a} & \makecell{Similarity \\computation}&Taxi&\makecell{Token\\ embedding}&\makecell{Conditioned \\sequence}&RNN&\makecell{Sampling \\rate,\\noise}&\makecell{Spatial \\proximity\\ aware loss}\\
		\cite{Yao2017} &Clustering& vessels &LSTM &LSTM&Seq2Seq &\makecell{Moving \\behavior} &\\
		\makecell{ \cite{Yao2019} }&Metric learning&&\makecell{SAM-augmented \\LSTM}&-&RNN&\makecell{Attention \\on grids}&\makecell{weighted\\
		ranking loss}\\
		\cite{Gao2017b} &\makecell{Trajectory-User\\
		Linking}& segmentation&&&&\\
%		\cite{Wu2017a}&&\makecell{Trajectory \\modeling}& & & &RNN&- & \\
		\cite{Zhang2019d}  & \makecell{Similarity \\computation}&\makecell{Activity \\trajectory} &RNN&RNN&Seq2Seq&\makecell{Spatial\\temporal\\activity}&weighted loss \\
%		\cite{Boonchoo2019a} &&Embedding &&&&&&\\ 
		\midrule
		
%		\cite{Xuan2016} &&\makecell{Transportation\\ mode}&&LSTM&LSTM&\makecell{Shared\\memory \\LSTM}&&\\
		\cite{Liu2016c} &\makecell{Next \\location} &Check-in&&&ST-RNN& & \\
%		\cite{Jin2018} &&\makecell{Next \\ location\\ with time}&&\makecell{Multi-modal \\embedding} &&RNN & &\\
		\cite{Zhou2018a} &Next trajectory&Flickr &\makecell{variational\\ encoder}&LSTM &RNN &Attention & \\
		\cite{Wu2019} &\makecell{Query \\optimization}&Taxi&LSTM&LSTM&Seq2Seq&-&\makecell{minimum \\square error}\\
		\cite{Gao2019c} &Next POI &Check-in &\makecell{POI\\ embedding}&Classifier&CNN&\makecell{Variational\\ attention}&\makecell{empirical\\ risk }\\
		\cite{Lv2019} &Destination&Taxi&Image&&CNN&&\\
		\cite{Zhang2017e} &\makecell{Crowd \\prediction}&Taxi&Grid&-&ST-ResNet&\makecell{weather\\ holiday}&\makecell{Root Mean \\Square Error}\\
%		\cite{Jiang2019} &&\makecell{Online \\crowd}&Big events&Grid &LSTM&ConvLSTM&&\makecell{reconstruction \\error}\\
		\bottomrule
	\end{tabular}}
\label{tab:deep}
%\vspace{-1.5em}
\end{table}


==> 1-Survey-trajectory 2/deep-tab1.tex <==
\begin{comment}
	\ra{-0.5}
	\centering
	\caption{Recent work on deep trajectory learning.}
	\vspace{-1em}
	\scalebox{0.82}{
	\hspace{-3em}	\begin{tabular}{ccccccccc}
		\toprule	\addlinespace[0pt]\rowcolor{gray!30}\rowcolor{gray!30}
		 \textbf{Work} & \textbf{Tasks} & \textbf{Data sources} & \textbf{\makecell{Deep Model}} \\ \addlinespace[-1pt] \midrule

		\cite{Wang2019i} & Data recovery & Taxi & LSTM & BiLSTM & seq2seq & \makecell{Spatial \\temporal\\ attention} & softmax \\
		\cite{Ouyang2018} &\makecell{Synthetic data \\generation} & Mobile GPS& \makecell{Matrix \\representation}& \makecell{matrix \\representation} &GAN &\makecell{Semantic \\ duration}&WGAN-GP \\
%		\cite{Systems2017} & \makecell{Mobility \\simulation}& Cellular data&IO-HMMs& \makecell{Distribution\\ coefficients}&GAN-LSTM &\makecell{Activity \\Features}&\\
		\makecell{\cite{Liu2018}} &\makecell{Privacy \\protection}& APPs&Embedding& \makecell{Random\\ deviations}&CGAN&POI &minimax\\
		\makecell{\cite{Gupta2018} }&\makecell{Mobility \\prediction}& Video&LSTM&LSTM&GAN&Pooling&L2\\\midrule
		
		\cite{Li2018a} & \makecell{Similarity \\computation}&Taxi&\makecell{Token\\ embedding}&\makecell{Conditioned \\sequence}&RNN&\makecell{Sampling \\rate,\\noise}&\makecell{Spatial \\proximity\\ aware loss}\\
		\cite{Yao2017} &Clustering& vessels &LSTM &LSTM&Seq2Seq &\makecell{Moving \\behavior} &\\
		\makecell{ \cite{Yao2019} }&Metric learning&&\makecell{SAM-augmented \\LSTM}&-&RNN&\makecell{Attention \\on grids}&\makecell{weighted\\
		ranking loss}\\
		\cite{Gao2017b} &\makecell{Trajectory-User\\
		Linking}& segmentation&&&&\\
%		\cite{Wu2017a}&&\makecell{Trajectory \\modeling}& & & &RNN&- & \\
		\cite{Zhang2019d} & \makecell{Similarity \\computation}&\makecell{Activity \\trajectory} &RNN&RNN&Seq2Seq&\makecell{Spatial\\temporal\\activity}&weighted loss \\
%		\cite{Boonchoo2019a} &&Embedding &&&&&&\\
		\midrule
		
%		\cite{Xuan2016} &&\makecell{Transportation\\ mode}&&LSTM&LSTM&\makecell{Shared\\memory \\LSTM}&&\\
		\cite{Liu2016c} &\makecell{Next \\location} &Check-in&&&ST-RNN& & \\
%		\cite{Jin2018} &&\makecell{Next \\ location\\ with time}&&\makecell{Multi-modal \\embedding} &&RNN & &\\
		\cite{Zhou2018a} &Next trajectory&Flickr &\makecell{variational\\ encoder}&LSTM &RNN &Attention & \\
		\cite{Wu2019} &\makecell{Query \\optimization}&Taxi&LSTM&LSTM&Seq2Seq&-&\makecell{minimum \\square error}\\
		\cite{Gao2019c} &Next POI &Check-in &\makecell{POI\\ embedding}&Classifier&CNN&\makecell{Variational\\ attention}&\makecell{empirical\\ risk }\\
		\cite{Lv2019} &Destination&Taxi&Image&&CNN&&\\
		\cite{Zhang2017e} &\makecell{Crowd \\prediction}&Taxi&Grid&-&ST-ResNet&\makecell{weather\\ holiday}&\makecell{Root Mean \\Square Error}\\
%		\cite{Jiang2019} &&\makecell{Online \\crowd}&Big events&Grid &LSTM&ConvLSTM&&\makecell{reconstruction \\error}\\
		\bottomrule
	\end{tabular}}
\label{tab:deep}
\vspace{-1.5em}
\end{comment} 

==> 1-Survey-trajectory 2/deep.tex <==
\sheng{\section{Emerging trend on Deep Trajectory Learning}
\label{sec:deep}
In the last three years, deep learning \cite{Lecun2015} becomes a useful tool to solve several problems of trajectory analytics.
%We have also sporadically covered some work that utilizes deep learning in anomaly detection, clustering, and classification In previous sections.
Next, we will conclude three types of representative work systematically, Table~\ref{tab:deep} shows their solved problem, with the model used in each work and their loss functions.

\input{deep-tab}

\subsection{Trajectory Data Recovery and Generation}
Sharing raw trajectory data always faces concerns on privacy \cite{Guo2015b}, and some datasets choose to remove most information and just maintain the source and destination for each trajectory, such as the NYC taxi trip dataset. 
However, such cleaning makes it hard to conduct a precise analysis of real trends and demand from commuters.
%\citet{Systems2017} employed deep recurrent neural network architecture to generate human activity chains from cellular data, which provides transportation planners, policy-makers, and related stakeholders with detailed and timely travel demand models.
A novel Deep Hybrid Trajectory Recovery model \cite{Wang2019i} aims to recover low-sampled trajectory data between a source and a destination.
Different to trajectory data recovery from a source and a destination, trajectory synthetic data generation aims to learn an open trajectory based on a private dataset which is complete.
\citet{Ouyang2018} proposed a generative model for trajectory by considering the constraint of privacy in data sharing, and high-order geographic and semantic features of human mobility.
\citet{Liu2018} designed a framework which uses generative adversarial networks (GAN) \cite{Goodfellow2014} to protect privacy but still enable effective analytics over a synthetic dataset.
%\citet{Kulkarni2018} considered the semantic information when generating a synthetic trajectory using GAN.
\citet{Gupta2018} proposed to generate pedestrian trajectories with GAN, and the main difference is that it is for pedestrian walk trace under cameras.
Not only can the generative model work for data recovery and generation, but also for anomaly detection. \citet{Liu2020} predicted the probability of a new trajectory being an anomaly.% using a deep generative sequence model.
%\cite{Kulkarni2018} conducted an evaluation.
%trajectory privacy

\subsection{Trajectory Representation and Metric Learning}
Representation learning of trajectory aims to convert trajectories into vectors with a fixed dimension, and then most trajectory analytics can be done using existing mature analytics based on Euclidean distance.
The main objective of deep trajectory embedding is for classification \cite{Endo2016}, clustering \cite{Yao2017}, and fast trajectory similarity search \cite{Li2018a,Yao2019}.
\citet{Endo2016} proposed a method that automatically extracts additional features using a convolution neural network (CNN), for transportation mode classification problem, their method converts a raw trajectory data structure into an image data structure while maintaining effective spatiotemporal information.
%\citet{Gao2017b} embedding for human mobility prediction.
%
%\cite{Ouyang2018} proposed to use GAN to preserve privacy for trajectories.
%\citet{Wu2017a} proposed RNN-based models to model trajectory, for the tasks over road network-constrained trajectories.
The recurrent network is widely used in deep trajectory embedding inspired by the word2vec. \citet{Li2018a} transferred each spatial-only trajectory to a vector first based on a probability model, and proposed a new spatial proximity aware loss function and a cell representation learning approach that incorporate the spatial proximity into the deep learning model.
\citet{Zhang2019d} further learned the representation for activity trajectory similarity computation, and proposed a novel loss function based on the attention mechanism in natural language processing to distinguish these three kinds of information, and an encoder-decoder model is also used similar to \cite{Li2018a}.
%\cite{Taghizadeh2019}
%\citet{Boonchoo2019a} proposed embedding for the attribute-aware trajectories.
%\cite{Pandhre2018} 
%\subsection{Metric learning}
Metric learning aims to learn similarity scores with an existing measure \cite{Yao2019} when inputting two trajectories, and it is generic to accommodate any existing trajectory measure and fast to compute the similarity of a given trajectory pair in linear time. The basic idea is to samples a number of seed trajectories from the given database and then use their pair-wise similarities as guidance to approximate the similarity function with a neural metric learning framework.
%this is put as an explansion, temporal aware.
%\citet{Chen2019b} learned a deep embedding approach for clustering and profiling taxi trip purposes.

\subsection{Trajectory Prediction for Human Mobility Analytics}
As trajectory is a sequential set of points, predicting where to go next \cite{Monreale2009} has several applications, e.g., indicating future locations of taxi drivers to assign new passengers, and restaurant recommendation based on users' check-ins.
%A survey \cite{Wang2019g} presents an overview on trajectory prediction research using traditional methods, including Markov-based, time-series based, and compression-based.
%Generally, prediction based on historical trajectories can be divided into two types: 1) next-point prediction \cite{Xuan2016,Liu2016c}; 2) crowd flow prediction \cite{Zhang2017e,Jiang2019}.
%Predict the destination of taxi trips based on initial partial trajectories, in the ECML/PKDD competition.
%As prediction itself is a learning-based task, and 
%neural network gradually becomes a as it enables modeling complex patterns and prediction problems.
%\subsubsection{Next-point Prediction}
%Since individual next-point prediction has a common objective, improving prediction precision is the goal.
Temporal information is crucial to train an effective prediction model, and recurrent neural network (RNN) is widely used.
%\citet{Xuan2016} predict transport mode of the next movement.
\citet{Liu2016c} extended RNN and proposed a novel method called Spatial Temporal RNN (ST-RNN) for next-point prediction, which can model local temporal and spatial contexts in each layer with time-specific transition matrices for different time intervals and distance-specific transition matrices for different geographical distances.
%\cite{Lei2011,Besse2018a,Rossi2019} 
%\citet{Jin2018} proposed human mobility prediction model based on Attentional Recurrent Networks.
\citet{Zhou2018a} predicted the future trip that the user would travel rather than predicting a single point, which can also reconstruct users trajectory.
Their model everages two variational latent factors which are respectively the traditional latent variables and the variational hidden state attention, for learning trajectory-level context.
NEIST \cite{Wu2019} applies an RNN to predict future positions of moving objects based on observed trajectories, and further accelerate the spatial-temporal queries.

Instead of using RNN which cannot train long sequence, \citet{Gao2019c} firstly incorporated convolutional neural network (CNN) to capture long term and structural dependency among user check-ins, achieving comparable learning ability with the state-of-the-art RNN based methods, while significantly improving the learning efficiency.
\citet{Lv2019} proposed a novel prediction algorithm T-CONV, which models trajectories as two-dimensional images, and then feed them into a CNN architecture to extract multi-scale patterns for precise destination prediction.
%\cite{Alahi2016}
%\subsubsection{Crowd Prediction}
Since trajectory data in a wide range can also indicate the historical crowd flow from one area to another area, crowd flow prediction \cite{Zhang2017e}  aims to indicate the amount of people that will travel in a given region and time stamp.
Specifically, \citet{Zhang2017e} proposed a deep-learning-based approach, called ST-ResNet, to forecast the in-flow and outflow of crowds in each and every region of a city.}
%To meet the demand that crowd flow prediction needs to be done in real time for emergence response,
%\citet{Jiang2019} built an online system which can iteratively take citywide crowd dynamics from the current one hour as input and report the prediction results for the next one hour as output.

%Temporal information
%\input{appendix}

%\subsection{Remarks}
%Trajectory modeling in neural network is a start, here we briefly introduce two kinds of modeling method to fit into neural network.

==> 1-Survey-trajectory 2/deepsurvey.tex <==
\section{Emerging trends on Deep Trajectory Learning}
\label{sec:deep}
%In the last three years, deep learning \cite{Lecun2015} becomes a useful tool to solve several problems of trajectory analytics.
%%We have also sporadically covered some work that utilizes deep learning in anomaly detection, clustering, and classification In previous sections.
%Next, we will conclude three types of representative work systematically, Table~\ref{tab:deep} shows their solved problem, with the model used in each work and their loss functions.

Deep learning has been successfully used for trajectory data
analytics and applications for the last several years, which is attracting increasing
interest.
%
We group these methods into several categories, and discuss the
associated research problems in detail in this section.
%Table~\ref{tab:deep} summarizes the research problem, together with the deep learning model used in each work.
%
We then cover the emerging trends in deep learning for trajectory
data.

\input{deep-tab1}


%generative adversarial networks (GAN) \cite{Goodfellow2014}


\subsection{Trajectory Pre-processing}

\noindent {\bf Trajectory Data Generation.}
%
%Sharing raw trajectory data always faces concerns on privacy \cite{Guo2015b}, and some datasets choose to remove most information and just maintain the source and destination for each trajectory, such as the NYC taxi trip dataset.
%However, such cleaning makes it hard to conduct a precise analysis of real trends and demand from commuters.
%\citet{Systems2017} employed deep recurrent neural network architecture to generate human activity chains from cellular data, which provides transportation planners, policy-makers, and related stakeholders with detailed and timely travel demand models.
%Different to trajectory data recovery from a source and a destination, trajectory synthetic data generation aims to learn an open trajectory based on a private dataset which is complete.
Generating synthetic yet realistic location trajectories plays a
fundamental role in privacy-aware analysis on trajectory data.
A generative model was proposed for generating trajectories
~\cite{Ouyang2018} based on a set of training trajectories.
The proposed solution uses generative adversarial networks (GAN) to
produce data points in a metric space, which are then transformed to a
sequential trajectory.
Experimental results show that the model is able to capture the
correlation between visited locations in a trajectory and learn the
common semantic/geographic mobility patterns from the training
trajectories.
%
The idea of using a GAN to generate synthetic trajectories that can
preserve the summary properties of real trajectory data for data
privacy was introduced by~\citet{Liu2018}.

%\shane{A paper literally on vision or a visionary paper, or something else? Can't quite decipher the intent here.}

%\citet{Liu2018} designed a framework which uses generative adversarial networks (GAN) \cite{Goodfellow2014} to protect privacy but still enable effective analytics over a synthetic dataset.
%\citet{Kulkarni2018} considered the semantic information when generating a synthetic trajectory using GAN.

%\cite{Kulkarni2018} conducted an evaluation.
%trajectory privacy

\myparagraph{Trajectory Data Recovery}
%
As many trajectories are recorded at a low sampling rate, the
low-sampled trajectories cannot capture the correct routes of the
objects.
This problem has been studied in two settings previously, either with
road networks using map matching~\cite{Lou2009}, or without road
networks~\cite{Su2013}, as discussed in Section~\ref{sec:preprocess}.
%
Wang et al.~\cite{Wang2019i} aimed to recover the trajectory between
two consecutive sampled points of ``low-sampled'' trajectory data.
Using a seq2seq model, the proposed method uses spatial and
temporal attention to capture spatiotemporal correlations and
integrates a calibration component using a Kalman filter (KF) in
order to reduce the uncertainty.

\subsection{Trajectory Representation and Similarity Search }
Representation learning of trajectories aims to represent trajectories
as vectors of a fixed dimension.
Then the similarity of two trajectories can be computed based on the
Euclidean distance of their vector representations, which reduces the
complexity of similarity computation from $O(n^2)$ to $O(n)$, where
$n$ is the trajectory length.
%
\citet{Li2018a} proposed a seq2seq-based model to learn trajectory
representations, where the spatial proximity is taken into account
in the design of the loss function.
The trajectory similarity based on the learned representations is
robust to non-uniform, low sampling rates, and noisy sample points.
%
\citet{Yao2019} proposed the use of a deep metric learning framework
to approximate any existing trajectory measure, and is capable of 
computing similarity for a given trajectory pair in linear time.
The basic idea is to sample a number of seed trajectories from the
given database and then use their pairwise similarities as guide
to approximate the similarity function with a neural metric learning
framework.
The proposed solution adopts a new spatial attention memory module
that augments existing RNN for trajectory encoding.
\citet{Fu2020} proposed to exploit the road networks to learn the trajectory representation based on an encoder decoder model.
%
Deep trajectory representation was also extended to multi-trajectory
scenarios, such as trajectories encountered in sporting events with
several football players~\cite{Wang2019b}.
\citet{Wang2020c} applied deep reinforcement learning to enable
sub-trajectory similarity search, by splitting every trajectory into
a set of sub-trajectories that can be candidate solutions for a query
trajectory.
By learning an optimal splitting policy, the sub-trajectory
similarity search is more efficient than heuristics-based methods.
%The recurrent network is widely used in deep trajectory embedding inspired by the word2vec. \citet{Li2018a} transferred each spatial-only trajectory to a vector first based on a probability model, and proposed a new spatial proximity aware loss function and a cell representation learning approach that incorporate the spatial proximity into the deep learning model.
%\citet{Zhang2019d} extended the approach~\cite{Li2018a} to learn the
%representation of activity trajectory, i.e., trajectory
%with additional semantic information, for similarity computation.

%\cite{Taghizadeh2019}
%\citet{Boonchoo2019a} proposed embedding for the attribute-aware trajectories.
%\cite{Pandhre2018}
%\subsection{Metric learning}
%Metric learning aims to learn similarity scores with an existing measure \cite{Yao2019} when inputting two trajectories, and it is generic to accommodate any existing trajectory measure and fast to compute the similarity of a given trajectory pair in linear time.


\subsection{ Deep Trajectory Clustering, Classification, and Anomaly Detection}
%
\citet{Yao2017} transformed trajectories into feature sequences that
capture object movements, and then applied an autoencoder framework to
learn fixed length deep representations of trajectories for
clustering.
%
\citet{Xuan2016} proposed a model named DeepTransport to predict the
transportation mode such as walk, taking trains, taking buses, etc.,
from a set of individual peoples GPS trajectories. LSTM
is used to constructed DeepTransport to predict a user’s
transportation mode.
%
\citet{Endo2016} adopted stacked denoising autoencoder (SDA) to
automatically extract features for the transportation mode
classification problem.
%
\citet{Gao2017} considered a different trajectory classification
problem, namely Trajectory-User Linking (TUL), which aims to link
trajectories to users who generate them in the location-based social
networks.
An RNN based semi-supervised model was proposed to address the TUL
problem.
%
\citet{Liu2020} proposed a deep generative model, namely a Gaussian
Mixture Variational Sequence AutoEncoder (GM-VSAE), for online
anomalous trajectory detection based on Variational autoencoding.
%The GM-VSAE model is able to (1) capture complex sequential
%information enclosed in trajectories, (2) discover different types
%of normal routes from trajectories and represent them in a
%continuous latent space, and (3) support efficient online detection
%via trajectory generation.

%\vspace{-2em}
\subsection{Trajectory Prediction for Human Mobility Analytics}
%As trajectory is a sequential set of points, predicting where to go next \cite{Monreale2009} has several applications, e.g., indicating future locations of taxi drivers to assign new passengers, and restaurant recommendation based on users' check-ins.
%A survey \cite{Wang2019g} presents an overview on trajectory prediction research using traditional methods, including Markov-based, time-series based, and compression-based.
%Generally, prediction based on historical trajectories can be divided into two types: 1) next-point prediction \cite{Xuan2016,Liu2016c}; 2) crowd flow prediction \cite{Zhang2017e,Jiang2019}.
%Predict the destination of taxi trips based on initial partial trajectories, in the ECML/PKDD competition.
%As prediction itself is a learning-based task, and
%neural network gradually becomes a as it enables modeling complex patterns and prediction problems.
%\subsubsection{Next-point Prediction}
%Since individual next-point prediction has a common objective, improving prediction precision is the goal.
Recurrent neural networks (RNN) are widely used for trajectory
prediction, and most of the work reviewed also learns user
representations from trajectories to capture user preferences in addition
to the spatio-temporal contexts.
%\citet{Xuan2016} predict transport mode of the next movement.
\citet{Liu2016c} proposed Spatial-Temporal RNN (ST-RNN) for the next
location prediction of a given user using an RNN.
An ST-RNN model local temporal contexts, periodical temporal contexts,
and geographical contexts to learn the representation of users under
specific contexts.
%
%, which can model local temporal and spatial contexts in each layer with time-specific transition matrices for different time intervals and distance-specific transition matrices for different geographical distances.
%\cite{Lei2011,Besse2018a,Rossi2019}
%\citet{Jin2018} proposed human mobility prediction model based on Attentional Recurrent Networks.
\citet{Zhou2018a} adopted a seq2seq encoder-decoder framework
consisting of two encoders and two decoders to predict future
trajectories.
This method does not explicitly learn user representations.
%
%predicted the future trip that the user would travel rather than predicting a single point, which can also reconstruct users trajectory.
%to an,
%Their model everages two variational latent factors which are respectively the traditional latent variables and the variational hidden state attention, for learning trajectory-level context.
\citet{Wu2017a} designed two RNN models to model trajectories
that consider road network constraints on trajectories, and can be
used to predict the destination of a trajectory.
%

DeepMove~\cite{Jin2018} is based on a multi-modal embedding RNN to
capture the complex sequential transitions by jointly embedding
multiple factors such as time, user, and location.
DeepMove also applies
attention mechanism to capture the periodical effect of mobility.
%DeepMove also used a historical attention model with two
%mechanisms to capture the multi-level periodicity.
%
\citet{Chen2020} proposed a context-aware deep model called DeepJMT
for jointly performing mobility prediction (to know where) and time
prediction (to know when).
DeepJMT captures the user’s mobility regularities and temporal patterns using RNN, captures spatial context, periodicity context and social and temporal context using various mechanisms, e.g., co-attention mechanism to capture, and make time prediction using temporal point process.
% \shane{Feeling bullet-pointy again at this point.}
%The DeepJMT model is based on a hierarchical RNN and temporal point process and takes into account
%a spatial context, a periodicity context.% It also employs a co-attention based social \& temporal context extractor
%to extract the mobility and temporal evidence from social relationships.


A convolutional neural network (CNN) can also be used for trajectory
prediction.
%
\citet{Pozzi2018} proposed a CNN-based approach for representing
semantic trajectories and predicting future locations.
%In a semantic trajectory, each visited location
%is associated with a semantic meaning such as home, work,
%shoppint, etc.
The semantic trajectories are represented as a matrix of semantic
meanings and trajectory IDs.
A CNN is applied to the matrix to learn the latent features for next
visited semantic location prediction.
%
\citet{Gao2019c} developed a deep generative model called Variational
Attention based Next (VANext) POI prediction, which simultaneously
learns implicit relationships between users and POIs, and captures
sequential patterns of user check-in behavior for next POI
prediction.
A CNN is used to capture long term and structural dependency among
user check-ins, achieving comparable learning ability with the
state-of-the-art RNN based methods, while significantly improving the
learning efficiency.
\citet{Lv2019} proposed to model trajectories as two-dimensional
images, and employed CNN for trajectory destination prediction.
%\cite{Alahi2016}

\iffalse
In addition, \citet{Gupta2018} addressed a different trajectory
prediction problem, predicting all possible socially acceptable
(e.g., respecting personal space) future trajectories, given observed
motion trajectories of pedestrians.
The proposed method is based on GAN and a seq2seq model.
%
% proposed to generate pedestrian trajectories with GAN, and the main difference is that it is for pedestrian walk trace under cameras.
%
NEIST \cite{Wu2019} is a neural-enhanced index to process
spatial-temporal queries.
NEIST uses an RNN to predict future positions of moving objects based
on observed trajectories, which is used together with the existing moving object index techniques to answer the
spatial-temporal query more efficiently and accurately. %\shane{Again using the problem
%solved to distinguish solutions which is superficial. Generally
%there is much more going on to get such papers published.}
\fi

%%\subsubsection{Crowd Prediction}
%Since trajectory data in a wide range can also indicate the historical crowd flow from one area to another area, crowd flow prediction \cite{Zhang2017e} aims to indicate the amount of people that will travel in a given region and time stamp.
%Specifically, \citet{Zhang2017e} proposed a deep-learning-based approach, called ST-ResNet, to forecast the in-flow and outflow of crowds in each and every region of a city.}



%\vspace{-1em}
\subsection{ Travel Time and Route Estimation}
\citet{Wang2018} aimed to estimate the travel time of a path from the
mobility trajectory data.
Their approach used a CNN and an RNN to capture the features of a
path, and employed a multi-task learning component to estimate the
travel time.
%
\citet{Zhang2018h} developed a bidirectional LSTM based deep model,
called {DeepTravel}, to estimate the travel time of a path from the
historical trajectories.
%
\citet{Li2019c} proposed a deep generative model, DeepGTT, to learn
the travel time distribution for a route by conditioning on the
real-time traffic, which is captured by the trajectory data.
%
\citet{Lix2020} proposed a deep probabilistic model, DeepST, which
unifies three key explanatory factors, the past traveled
trajectories, the impact of destination, and real-time traffic for
the route decision of a pair of source and destination.
{\citet{Yuan2020} estimated the travel time of an origin-destination
pair at a certain departure time, and proposed a neural network based
prediction model.
This model exploits the fact that for a past OD trip its travel
time is usually affiliated with the trajectory it travels along,
whereas it does not exist during prediction.}
%To meet the demand that crowd flow prediction needs to be done in real time for emergence response,
%\citet{Jiang2019} built an online system which can iteratively take citywide crowd dynamics from the current one hour as input and report the prediction results for the next one hour as output.

%Temporal information
%\input{appendix}

%\subsection{Remarks}
%Trajectory modeling in neural network is a start, here we briefly introduce two kinds of modeling method to fit into neural network. 


==> 1-Survey-trajectory 2/future.tex <==
\section{Future Research Directions and Open Issues}
\label{sec:future}

Trajectory data has inspired many important research problems and
applications in both academia and industry.
However, open-source and commercial systems that can support the
entire pipeline of trajectory data management and analytics are still
non-existent.
To better cater to future applications, a unified trajectory data
management system would be an important contribution to the
community.
Desirata of such a system include:
\begin{itemize}
\item \textbf{Data Cleaning}: Map matching, re-sampling, and
calibration are fundamental building blocks in efficient and
effective analytics.
However, current solutions need to input a road network dataset given
by users manually, and also need to input several data-dependent
parameters.
An automated data cleaning pipeline for trajectory data is highly
desirable as manual data cleaning is time-consuming and often not
reproducible.
\item \textbf{Trajectory Data Repositories}: Cleaning trajectory is
computationally expensive.
Publicly available data repositories of raw and cleaned data would
not only improve reproducibility, it would also stimulate new
research in the area.
A standard data format for trajectory data is also not currently
defined.
Even though LineString and GPX can be used, their use is limited.
Labeled datasets for similarity search and classification problems
are also non-existent, hampering progress on this important problem.

\item \textbf{Data Integration and Operator Support}: In more
advanced data analytics applications, trajectory data is often
heterogeneous.
Data integration between trajectory databases and other databases,
including spatial databases (point data) and graph databases (road
networks) would be a valuable contribution.
Trajectory data from multiple devices, including cameras, UAV, and
RFID can also be integrated to build more comprehensive profiles of a
city.
Unstructured metadata from various sources also plays a vital role
when apply trajectory data in real-world application.
This data might include speed limits, transit timetables, and public
service opening hours. %(GTFS: General Transit Feed
%Specification\footnote{\url{https://gtfs.org/}}) 
While this information is used commonly in commercial applications,
the cost of using proprietary data sources is often too high
in the research community.

\item \textbf{Performance Benchmarks}: 
A trajectory performance benchmark similar to the TPC
benchmark\footnote{\url{http://www.tpc.org/information/benchmarks.asp}}
would greatly improve the quality of empirical comparisons of new
algorithms in research papers.
There are many different distance measures and indexing data
structures being applied to trajectory search with little
understanding of their true performance characteristics.
For efficiency, pruning power and I/O are important factors in total
running time; for the effectiveness, no ground-truth means that
search quality cannot truly be measured.


\item \textbf{Parameterization}: Parameter selection plays a critical
role in system performance of trajectory analytics.
Parameter-free algorithms are highly desirable, but not always
possible.
Automated parameter selection is an
essential requirement for automatic databases, and
for intelligent trajectory analytics.
It would also be interesting to investigate how to automate bounding
approximation ratios can be achieved during algorithm design.
%The input is a set of constraints selected interactively from budget
%costs, influence model, or the number of expected results.


\item \textbf{Deep Trajectory Learning}: Deep learning has made some progress in synthetic data generation, 
	representation learning, and mobility prediction. More advanced tasks, 
	including query optimization and learned index, can be investigated to 
	improve the query performance. Another promising topic can be the 
	online deep trajectory learning to meet the demand for timely decision 
	making over dynamic trajectory data.

\item \textbf{Self-Driving Trajectory}: {Self-driving \cite{Ma2018,Chang2019} will be one of the primary sources of trajectories in the near future.
Different from the typical long-term trajectories being currently analyzed in road-network which is the focus in this survey, self-driving trajectories will be short-term lane-level traces with high sampling rates, e.g., each trajectory only lasts for five seconds \cite{Chang2019}. Due to the requirement of real-time response for safe driving, managing and analyzing such trajectories will be crucial and challenging, especially in a streaming scenario.}

\item \textbf{Trajectory Analysis for Public Health}: Human movement data recorded by mobile phones has been analyzed to control Malaria in Africa \cite{Wesolowski2012} and dengue epidemics in Pakistan \cite{Wesolowski2015}. With mass outbreaks of diseases such as COVID-19 \cite{covid19,covid19-2} in dense urban areas, collecting and analyzing the trajectories of infected people and building real-time warning mechanisms will play an important role in disease traceability, disease control, and emergency response.
\end{itemize}



==> 1-Survey-trajectory 2/intro.tex <==
\section{Introduction}
\begin{figure}
	\subfigure[{\scriptsize {Human trajectories in surveillance} \cite{Zhou2012}} ]{\includegraphics[height=2.7cm]{graph/train.pdf}}~~~~~~~~~~~~~~~~~~~~
	\subfigure[ \scriptsize Monitoring cars by UAV \cite{Bock2019}]{\includegraphics[height=2.7cm]{graph/drone.png}}~~~~~~~~~~~~~~~~~~~~
	\subfigure[\scriptsize  Car localization by RFID \cite{rfid}]{\includegraphics[height=2.7cm]{graph/localization/vehicles-rfid-1.jpg}}
	\vspace{-1.5em}
	\caption{New localization techniques that can capture trajectory data more proactively than using GPS.}
	\vspace{-1.5em}
	\label{fig:more-devices}
\end{figure}

%\section{Background}
Just over twenty years ago, Global Positional System (GPS) satellites
began transmitting two additional signals to be used for civilian
(non-military) applications to improve aircraft
safety.\footnote{\url{https://www.pcworld.com/article/2000276/a-brief-history-of-gps.html}}
Demand for GPS-based navigation has grown steadily ever since,
and privately owned vehicles are now the dominant consumers of this
technology.
An increased reliance on GPS-equipped smartphones has also led to a
rise in the use of location-based services (\textbf{LBS}), such as
ride-sharing and social-network check-ins.


In addition to GPS data, other sensor devices such as traffic
surveillance cameras, unmanned aerial vehicles
(UAV),\footnote{\url{https://www.gpsworld.com/in-mit-project-drones-map-without-gps/}}
and Radio-frequency identification (RFID) can also collect location
data without deploying battery-dependent receiving devices to track
objects, as shown in Fig.~\ref{fig:more-devices}.
Such devices can accurately report precise locations and track
objects proactively and continuously.

\subsection{Trajectory Data}
Devices that track moving objects often generate a series of
ordered points representing a \textit{trajectory}.
More formally, a trajectory $T$ is composed of two or more
\textit{spatial-only} points and defined as: 


\begin{definition}{\textbf{(Point)}}
	\label{def:point} 
A point $p = \{\avar{x}, \avar{y}, t\}$ records the latitude
$\avar{x}$, the longitude $\avar{y}$ at timestamp $t$.
\end{definition}


\begin{definition}{\textbf{(Trajectory)}}
{A trajectory $T$ is a sequence of points
$\{(p_1, \gamma_1), (p_2, \gamma_2),\ldots,(p_{m}, \gamma_m)\}$}.%, where each $p_i$ is a point.
\end{definition}

%\shane{Why not make the length $m$. Is there a distinction between
%$|T|$ and $m$?}

The number of points in a trajectory $T$ is denoted as the
\textit{length} of the trajectory, and the \textit{sampling rate} is
the number of samples per second (or other time units).
Additional information $\gamma$ can be included with each point $p$ in a
trajectory $T$ generated from the location-based service.\footnote{{For spatial-only trajectories, we can set $\gamma=\emptyset$. Note that $\gamma$ can also be attached to the whole trajectory directly.}}
For example, textual data can be integrated into a trajectory from
social network check-in data or travel blogs, and has been referred
to as
\textit{spatial-textual trajectories} \cite{Kim2015b,Bao2012Location}, \textit{semantic trajectories} \cite{Zhang2014a}, or \textit{symbolic trajectories}~\cite{Damiani2015}.
This survey will focus primarily on these two closely related forms
of trajectory data as solutions and applications in recent research
work commonly overlap.

\myparagraph{Survey Scope} 
We focus primarily on urban trajectories.
Other studies of domain specific data such as aircraft
\cite{Ayhan2016} are not covered in this work. 
Note that the main difference between a moving object
\cite{Saltenis2000b} and a trajectory is the distinction between
a pointwise sequence and a continuous projection, and each of them
often employs fundamentally different storage and algorithmic
solutions.

\myparagraph{Public Trajectory Datasets}
Table~\ref{tab:alldatasets} shows several existing urban trajectory
datasets, which can be broadly divided into three groups: humans,
vehicles (car, truck, train, bus, tram, etc.), others (animals and
hurricanes).
%, and
%aircraft\footnote{\url{https://opensky-network.org/}}).
%Since several commonly used the aircraft datasets are not publicly
%available, and are therefore not included.
%\shane{I think you should drop it entirely.
%We already said above that we won't consider it ....}
We can observe that human derived 
trajectory data (including vehicles) is a common source of
trajectory data,
%Around 77\% of smartphone owners regularly use
%navigation %apps,\footnote{\url{https://themanifest.com/app-development/popularity-google-maps-trends-navigation-apps-2018}}
and is currently the largest source of trajectory data.
For example, $1.1$ billion (seventh row) individual taxi trips were
recorded in NYC from January 2009 through June 2015.
Other datasets including the movement of animals and hurricanes have
relatively few available trajectories, making such collections
much more tractable to process and analyze.
%Animal tracking is still rare as the cost benefit is low.
%For example, it costs up to \euro{1250} to equip a GPS collar.\footnote{\url{http://www.environmental-studies.de/products/02/gps-gsm_collars.html}}

%\sheng{The amount of trajectory data will sharply increase and has great applications on , how can we efficiently manage the big trajectory data and conduct}

\begin{table}
	\ra{1}
	\centering
	\caption{Publicly available trajectory datasets.}
	\vspace{-1em}
	\label{tab:alldatasets}
	\scalebox{0.75}{\begin{tabular}{cccccc}
			\cmidrule{1-5}\addlinespace[-2.7pt]\rowcolor{gray!30}
			\textbf{Categorization} &\textbf{Type} & \textbf{Exemplary Datasets}& \textbf{\#Trajectories} & \textbf{Applications} \\ \addlinespace[0pt]\cmidrule{1-5}
			\multirow{5}{*}{Human}	& {GPS tracking} & GeoLife \cite{Zheng2009} & \numb{17621} & Human mobility \cite{Zhang2016a} &
			\multirow{12}{*}{\hspace{-2em}$\left.\begin{array}{l}
				\\
				\\
				\\ \\ \\ \\ \\ \\ \\ \\ \\ \\ 
				\end{array}\right\rbrace{}\makecell{\text{Urban}\\\text{area}} $} 
			\\ %\cmidrule{2-4}
			& Check-in & \makecell{Foursquare \cite{Bao2012Location}\\ Gowalla \cite{Cho2011}} & \numb{104478} & \makecell{Tourism planning \cite{Wang2017} \\Mobility prediction \cite{Jin2018}}\\ %\cmidrule{2-4}
			&Online sharing & \makecell{OpenStreetMap \cite{osm} }& 8.7 million & Commuting analytics \\
			&{Video surveillance} & {Grand central station \cite{Zhou2012}}& \numb{20000} &Crowd behavior \\
			&{COVID-19} & \makecell{KCDC \cite{covid19-2}, JHU \cite{covid19}}& <100 & Disease control \\
			 
		%www	&Sport& STATS \cite{stats-ai} & 7500 &Sport analytics \cite{Sha2018}\\
		\cmidrule{1-5}
			\multirow{4}{*}{Vehicle}&Taxi trips & T-drive \cite{Yuan2010}, {Porto} \cite{portodata} & 1.7 million & Traffic monitoring\\ %\cmidrule{2-4}
			&Taxi trip-requests & NYC \cite{nyctaxidata}, Chicago \cite{nyctaxidata}& 1.1 billion& Ride sharing\\ %\cmidrule{2-4}
			&{Traffic cameras} & NGSIM \cite{NGSIM} & - & Traffic simulation\\
			&{Drones} & HighD \cite{Krajewski2018}, inD \cite{Bock2019}& \numb{110000} & Traffic prediction\\
			%	\cmidrule{2-4}
			& {Self-driving}& Argoverse \cite{Chang2019}, ApolloScape \cite{Ma2018} & \numb{300000} & Trajectory forecasting \\
			&Trucks & Greece Trucks \cite{greecetrucks} & \numb{1100} & Pattern mining\\ \cmidrule{1-5}
			\multirow{2}{*}{Others}&Hurricanes & Atlantic hurricanes~\cite{nhcdata}& \numb{1740} &Disaster detection \\ %\cmidrule{2-4}
			&Animals & Zebranet \cite{nhcdata}, Movebank \cite{Movebank}& 33 & Animal behavior \cite{LaPoint2013}\\
			\cmidrule{1-5} 
	\end{tabular}}
	\vspace{-1.4em}
\end{table}



\subsection{An Overview}
\label{sec:overview}
Fig.~\ref{fig:data-query} provides an overview of trajectory data
management, analytics, and learning. % for: 1)
%pre-processing; 2) storage; 3) similarity measures and queries; 4)
%clustering and classification; and 5) upstream urban analytic tasks.
Briefly, a trajectory data management and analytic system
has several fundamental components:

\begin{itemize}
\item \textbf{Cleaning}: Common techniques to clean common sensor
errors in raw trajectories and normalize sampling rates.

\item \textbf{Storage}: Open-source, commercial, and other commonly
deployed storage formats that are used to represent trajectory data.

\item \textbf{Similarity Measures}: 
The most commonly used measures for top-$k$ similarity search,
similarity joins, and clustering.

\item \textbf{Indexing}: State-of-the-art solutions for indexing
spatial and spatial-textual trajectory data, as well as effective
pruning solutions to improve performance.

\item \textbf{Query and Analytics}: The most common trajectory queries, including
range queries, top-$k$ similarity search, and trajectory joins.

%\item \textbf{Pruning algorithms}: Common pruning techniques applied
%in data access and distance computations.\shane{You say this in indexing
%too. Is that redundant? Maybe that sentence goes here about bounds?}

\item \textbf{Upstream Urban Applications}: The four most common offline urban
applications of trajectory data with problem formulations and
solutions.
% \shane{Not there yet. But we might want to think
%carefully about how we justify only these four?}
\end{itemize}

\begin{figure}
	\centering
	\includegraphics[width=14cm]{graph/framework-deep.pdf}
	\vspace{-2.5em}
	\caption{{Overview of trajectory data collection, management,
		representative applications, and widely used deep learning models (indicated by the green labels, and the full names of models can be found in Section~\ref{sec:deep})}.}
	\vspace{-1em}
	\label{fig:data-query}
\end{figure}


\begin{table}
	\centering
	\caption{Survey contributions relative to prior trajectory surveys.}
	\vspace{-1em}
	\label{tab:distinction}
	\scalebox{0.75}{
	\begin{tabular}{lccccccc}
		\toprule
		\addlinespace[0pt]\rowcolor{gray!30}
		\textbf{Survey} & \textbf{Datasets} & \textbf{\makecell{Commercial\\ systems}} & \textbf{\makecell{Similarity\\measures}} & \textbf{\makecell{Pruning\\mechanisms}} & \textbf{Indexing} & \textbf{\makecell{Processing\\ pipeline \\decomposition}} & \textbf{\makecell{Deep\\ learning} } \\
		\addlinespace[0pt]\midrule
		2011 \cite{Zheng2013a} & \xmark & \xmark & spatial & spatial & spatial & \xmark & \xmark \\
		2013 \cite{Parent2013a} & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
		2015 \cite{Zheng2015b} & only GPS & \xmark & spatial & \xmark & spatial & mining & \xmark \\
		2016 \cite{Feng2016a} & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
%		2018 \cite{Kong2018} & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
		2018 \cite{Richly2018} & \xmark & \xmark & \xmark & \xmark & spatial & \xmark & \xmark \\ 
%		2019 \cite{Su2019b} & \xmark & \xmark & \xmark & \xmark & spatial & \xmark \\ 
		\midrule
%		\textbf{\makecell{This \\survey}} & \makecell{ \cmark \\taxonomy,\\property,\\diversity} & \makecell{\cmark \\functions,\\format,\\extensibility} & \makecell{\cmark \\spatial,\\textual,\\robustness} & \makecell{\cmark \\ filtering,\\ verification\\ } & \makecell{\cmark \\ spatial,\\textual,\\footprint} & \makecell{ \cmark\\decomposition,\\semantic \\ pattern mining} & \makecell{\cmark \\ privacy, \\embedding,\\ mobility} \\ \bottomrule
\textbf{\makecell{This survey}} & \makecell{ \cmark } & \makecell{\cmark } & \makecell{\cmark } & \makecell{\cmark} & \makecell{\cmark } & \makecell{ \cmark} & \makecell{\cmark } \\ \bottomrule
	\end{tabular}}
	\vspace{-1.5em}
\end{table}

\subsection{New Expository Contributions Found from this Survey}
\label{sec:new}
Managing large-scale trajectory data has many important challenges
in efficiency and scalability due to its size and diversity.
A survey covering state-of-the-art and open problems in each stage, from data pre-processing all the way to upper-stream applications, is valuable to both research and industrial communities.
While several surveys on trajectory data exist, none review
trajectory data management and applications as outlined in
Fig.~\ref{fig:data-query}.
Prior surveys have covered trajectory data mining \cite{Zheng2015b},
semantic trajectory modeling \cite{Parent2013a}, and related
applications \cite{Richly2018}.
Table~\ref{tab:distinction} compares and contrasts prior surveys with
our own, highlighting the new areas covered.
%applications of
%trajectory data in transportation \cite{Markovic2019}, 
%, and %sport trajectory \cite{Gudmundsson2017}.
A couple of surveys from closely related areas which do partially
overlap with the content of this survey include: trajectory
similarity measures \cite{Su2019b}, trajectory privacy
\cite{Guo2015b}, and trajectory classification
\cite{Bian2019}.
In these instances, this survey includes more recent work from these
important areas.
%human mobility prediction \cite{Wang2019g}
The closest related review work is the textbook ``Computing with spatial
trajectories'' \cite{Zheng2013a}, published in 2011.
Current techniques have advanced significantly in the last ten
years, including the quickly growing area of spatial-textual trajectories,
which were not covered previously.
The key contributions of this survey can be summarized as:

\begin{itemize}

\item \textbf{Scalability and Storage}.
This survey comprehensively reviews trajectory storage, which is
commonly required in scalable offline analytics.

\item \textbf{Processing Pipeline Decomposition}. 
We provide insights into the connections among all components in
the entire data processing pipeline.
For the backend, we compare trajectory storage systems (academic and
commercial); for middleware, we compare similarity measures, queries,
and index structures; for upstream trajectory applications, we
propose a taxonomy for key operators used across multiple
tasks.

\item \textbf{Representative Applications}.
Based on a comprehensive review of recent research in SIGMOD, PVLDB,
ICDE, KDD, SIGSPATIAL, VLDBJ, TKDE, IJGIS, and TITS, we focus on
urban applications requiring real-time responses or timely decision
making, including: 1) road traffic; 2) green transport; 3) tourism
planning; 4) site selection.
These applications depend heavily on downstream analytics tools.
For example, clustering is commonly used to generate candidate routes
and to generate a fixed number of results for traffic monitoring.

\item \textbf{Deep Trajectory Learning}.
New trends on using deep learning for various trajectory data
analytics tasks, including trajectory recovery and generation,
trajectory representation and similarity search, clustering,
classification, anomaly detection, and trajectory prediction.

\item \textbf{Perspectives on Future Trajectory Data Management Challenges}.
We conclude with a list of key challenges and associated open problems
for researchers working in the area.
\end{itemize}

\subsection{Outline of This Survey}
The remainder of the survey is organized as follows:
Section~\ref{sec:manage} presents techniques for trajectory data
storage and pre-processing.
Section~\ref{sec:distance} compares common trajectory similarity
measures.
Section~\ref{sec:spatialonly} illustrates
queries and indexing techniques for spatial-only trajectory data and
spatial-textual trajectory data, respectively.
Section~\ref{sec:clustering} reviews trajectory clustering from a
data management perspective.
Section~\ref{sec:application} presents a taxonomy of four application
types commonly encountered in trajectory data management.
Section~\ref{sec:deep} introduces the latest progress in deep
trajectory learning.
Section~\ref{sec:future} discusses the future of trajectory data
system management.
Section~\ref{sec:conclude} concludes the paper.


\iffalse
How do we collect the papers? we use DBLP (Google scholar is also used to track the impact by citations).

Conferences: 
SIGMOD\footnote{\url{https://dblp1.uni-trier.de/search?q=trajector\%20venue\%3ASIGMOD\%20conference\%3A}},
KDD\footnote{\url{https://dblp1.uni-trier.de/search?q=trajector\%20venue\%3AKDD\%3A}},
PVLDB\footnote{\url{https://dblp1.uni-trier.de/search?q=trajector\%20venue\%3APVLDB\%3A}}, 
ICDE\footnote{\url{https://dblp1.uni-trier.de/search?q=trajector\%20venue\%3AICDE\%3A}}, 
CIKM\footnote{\url{https://dblp1.uni-trier.de/search?q=trajector\%20venue\%3ACIKM\%3A}}, 
SIGSPATIAL\footnote{\url{https://dblp1.uni-trier.de/search?q=trajector\%20venue\%3ASIGSPATIAL\%2FGIS\%3A}}\footnote{\url{https://dblp1.uni-trier.de/search?q=trajector\%20venue\%3AGIS\%3A}}, 
EDBT\footnote{\url{https://dblp1.uni-trier.de/search?q=trajector\%20venue\%3AEDBT\%3A}}, 
MDM\footnote{\url{https://dblp1.uni-trier.de/search?q=trajector\%20venue\%3AMDM\%3A}}.
More conferences can be added, such as ICDM, SSTD, DASFFA, BIGData; 

Journals: TKDE\footnote{\url{https://dblp1.uni-trier.de/search?q=trajector\%20venue\%3AIEEE_Trans._Knowl._Data_Eng.\%3A}}, 
Geoinformatica\footnote{\url{https://dblp1.uni-trier.de/search?q=trajector\%20venue\%3AGeoInformatica\%3A}},
VLDBJ\footnote{\url{https://dblp1.uni-trier.de/search?q=trajector\%20venue\%3AVLDB\%20journal\%3A}},
TITS\footnote{\url{https://dblp1.uni-trier.de/search?q=trajector\%20venue\%3AIEEE_Trans._Intelligent_Transportation_Systems\%3A}}, IJGIS\footnote{\url{https://dblp1.uni-trier.de/search?q=trajector\%20venue\%3AInternational_Journal_of_Geographical_Information_Science\%3A}},
Transportation Research Part C (it is not indexed by dblp),

The difference with five previous surveys. \cite{Zheng2015b}: no indexing, and the mining has great progress, \cite{Zheng2013a}: the indexing has been more advanced, it is spatial-only and more attributes are considered, system levels (industry and commercial).
More surveys: \cite{Feng2016a}, \cite{Kong2018}, \cite{Richly2018}.

We also point out several future research problems and promising applications. TSQL, Systems. Indoor trajectory.

\begin{figure}
	\centering
	\includegraphics[height=4.5cm]{graph/amount.pdf}
	\caption{Increasing number of published papers on trajectory data.}
	\label{fig:amount}
\end{figure}

We can generate a wordle to illustrate the keywords based on the title.
\begin{figure}
	\centering
	\includegraphics[height=13cm,angle=270]{graph/all.pdf}
	\caption{An overview of trajectory research using wordle on the paper titles.}
	\label{fig:wordle}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[height=13cm,angle=270]{graph/all-after-2014.pdf}
	\caption{An overview of trajectory research using wordle on the paper titles (published in recent five years).}
	\label{fig:wordle2015}
\end{figure}

GPS is not the only trajectory, new device such as RFID, Cameras.
The latest 5 years, what is the new trend?

Trip planning, 
Transportation Optimization and Planning.
Traffic Monitoring.

ACM Survey \footnote{\url{https://dblp1.uni-trier.de/search?q=ACM\%20Comput.\%20Surv.}}: \cite{Castro2013a}, \cite{Ilarri2010}, \cite{Parent2013a},\cite{Siabato2018},\cite{Silva2019}.


Contributions survey. Taxonomy, data, index, reproducibility, industry and academic.

Trajectory data is huge.

\fi


==> 1-Survey-trajectory 2/literature1.tex <==
\section{Management Systems and Pre-processing}
\label{sec:manage}
%To have an intuitive understanding of trajectory data, we first
%discuss trajectory representations and storage systems
%currently available for trajectory data.

\subsection{Trajectory Representation and Storage}
A list of coordinates denoted by two floats (e.g.,
{\small``-37.807302, 144.963242''}) are the traditional representation
of a spatial point location.
Two or more such points can be used to represent a trajectory for
storage, search, and analytics, and is the most common method in both
research and industry.
Table~\ref{tab:systems} shows several representative research systems
specifically designed for trajectory data, as well as several
commercial systems which were not necessarily designed for only
trajectory data, but can store and manipulate trajectory data through
module extensions.
Since commercial systems are designed to handle many different types
of data, they can incur additional cost overheads.

In the academic field, several trajectory storage systems have been
built to manage trajectory data
\cite{Cudre-Mauroux2010,Wang2014e,Shang2018,Ding2018,Xie2016a,Wangsheng2018}, and
store trajectories as a set of points.
These trajectory management systems
\cite{Cudre-Mauroux2010,Wang2014e,Xie2016a} only support a single
storage format, and often only a single query type such as a range
query (finding trajectories in a rectangle).
More recently, distributed systems \cite{Shang2018,Li2020,Ding2018} have
been developed to store point-based trajectory datasets scalably, and
can perform more advanced queries such as $k$NN search over
trajectories.

Existing commercial or open-source systems (e.g., a general database
such as Oracle
Spatial\footnote{\url{https://www.oracle.com/technetwork/database/options/spatialandgraph/overview/index.html}},
SQL
Server\footnote{\url{https://docs.microsoft.com/en-us/sql/relational-databases/spatial/spatial-data-sql-server}},
and
MySQL\footnote{\url{https://dev.mysql.com/doc/refman/5.7/en/gis-linestring-property-functions.html}},
or geospatial databases such as
ArcGIS\footnote{\url{http://www.arcgis.com/index.html}},
Tile38\footnote{\url{https://github.com/tidwall/tile38}},
PostGIS\footnote{\url{https://postgis.net/}},
GeoMesa\footnote{\url{https://www.geomesa.org/}}) can
also be extended for trajectory management.
For example, {\em LineString} defined
a portable data-interchange
format-GeoJSON\footnote{\url{https://en.wikipedia.org/wiki/GeoJSON}}
which is a geographical representation for an array of point coordinates.
A trajectory can be stored as a {\em LineString} using this format.
\textit{GPX} (the GPS Exchange Format) \cite{foster2004gpx} is
another format used by OpenStreetMap for routing and tracking.
Figures~10 and ~11 in Appendix~\cite{Wang2020} show an example of
these two formats.
However, operator support for LineString and GPX data is limited,
e.g., return the number of points, the starting the ending point, or
the $i$-th point.
Range and \knn queries are supported over all points, but not the
trajectories themselves.
%
%JSC I am not sure why you were so aggressive is space in the below. Space
% is not an issue.
%
%\ref{fig:linstring}
%\ref{fig:gpx}
\begin{table}
	\centering
	\ra{1}
	\caption{An overview of existing trajectory database systems.}
	\vspace{-1em}
	\scalebox{0.75}{\begin{tabular}{cccccc}
		\toprule
		\addlinespace[0pt]\rowcolor{gray!30}
		\textbf{System} & \textbf{Data} & \textbf{Indexing} & \textbf{Range} & \textbf{$k$NN} & \textbf{Similarity Measure} \\
		\addlinespace[-1pt]\midrule
		TrajStore \cite{Cudre-Mauroux2010} & Trajectory & Quad-tree & \cmark & \xmark & \xmark \\
		SharkDB \cite{Wang2014e} & Trajectory & Frame structure & \cmark & \cmark & Point-to-trajectory \\
		UITraMan \cite{Ding2018} & Trajectory & R-tree & \cmark & \cmark & Point-to-trajectory \\
		TrajMesa \cite{Li2020} & Trajectory & Z-order curve & \cmark & \cmark & Point-to-trajectory \\
		DITA \cite{Shang2018} & Trajectory & R-tree & \cmark & \cmark & Trajectory-to-trajectory \\ 
		Torch \cite{Wangsheng2018} & Trajectory & Grid-index & \cmark & \cmark & Trajectory-to-trajectory \\ 
		\midrule
		Oracle & LineString & R-tree & \cmark & \cmark & Point-to-point \\
		PostGIS & LineString & R-tree & \cmark & \cmark & Point-to-point \\
		SQL Server & LineString & Grid-index & \cmark & \cmark & Point-to-point \\
		GeoMesa & LineString & Z-order curve & \cmark & \cmark & Point-to-point \\
		Tile38 & LineString & R-tree & \cmark & \cmark & Point-to-point \\
%		Magellan & LineString & \xmark & \cmark & \xmark & \xmark \\
		GeoSpark \cite{Yu2015} & LineString & R-tree & \cmark & \cmark & Point-to-point \\
		SpatialSpark \cite{You2015a} & LineString & R-tree & \cmark & \xmark & \xmark \\ \bottomrule
	\end{tabular}}
	\label{tab:systems}
		\vspace{-1.5em}
\end{table}

SpatialSpark \cite{You2015a} and GeoSpark \cite{Yu2015} are two
representative open-source systems from the research field of spatial
databases, which also support the storage and querying of LineString.
Range and $k$NN queries are supported for the point data, but not
trajectories.
Nevertheless, these spatial database systems could be extended
to support any number of trajectory search operators
in the future since trajectory data is an extension point data.
In Section~\ref{sec:spatialindexing}, we will review indexing
techniques for point data in more detail.


\subsection{Trajectory Pre-processing}
\label{sec:preprocess}
\myparagraph{Trajectory Cleaning}
Since trajectory data is often collected with GPS devices
that have an average user range error (URE) of 7.8 m (25.6 ft), with
95\% probability, trajectory point data is \textit{noisy}
\cite{Zheng2015b}.
Moreover, the sampling rate of GPS devices varies by application.
For example, two vehicles following an identical path can produce
trajectories that contain a different number of sampled points.
These factors can directly affect distance or
similarity computations, and degrade result quality.
Hence, when processing raw trajectory datasets, data cleaning is not
only beneficial, but in certain circumstances a requirement.
\textit{Data segmentation} \cite{Buchin2011},
\textit{calibration} \cite{Su2013} and \textit{enrichment}
\cite{Alvares2007} are the three most common cleaning techniques
for trajectory data.
Specifically, segmenting data splits a long trajectory into several
short trajectories.
For example, analysis of a single taxi ``trip'' makes more sense than
analyzing the movements of the taxi for an entire day.
\citet{Buchin2011} addressed the problem of segmenting a trajectory
based on spatiotemporal criterias, including location, heading, speed, velocity, curvature, sinuosity, curviness, and shape. %\shane{What is the criteria?}
%\citet{AAlewijnse2014} proposed an algorithmic framework to improve
%the scalability of criteria-based segmentation.
%\shane{Is the 2011 paper 
%above and this one related in any way? In a survey, you are absolutely
%expected to articulate very specific details about every paper you
%cite. The reader should be able to know exactly what was in the paper
%without having to read it!}
%\citet{Biljecki2013} segmented trajectories according to
%transportation mode, e.g., walking, bus, and driving.

\citet{Su2013} proposed a calibration method that transforms a heterogeneous trajectory dataset to one with (almost) unified sampling strategies, such that the similarity between trajectories can be computed more accurately.
For noisy points, calibration identifies outliers
and adds statistical correction instead of filtering out
these points directly. 
Such calibration also plays an important role in precise similarity computation \cite{ranu2015indexing}, which we will introduce later.
%\shane{Is this right? They somehow reweight
%the point location to align it better with others in the trajectory?}
\citet{Liu2012a} further considered the constraint of road network topology, geometry
information, and historical information to re-calibrate noisy data
points.
% \shane{You put these two together. Is the math different?
%Just the data? Something else?}
For trajectories of sparse data points, \citet{Alvares2007}
proposed that the data can be enriched with additional points and
semantic information about the types of visited places.
%\citet{Yan2011} proposed an annotation framework 
%for heterogeneous trajectory data which supports any moving
%object that uses semantic data provided from multiple 3rd party
%sources.
%\shane{I have to admit the use of the word semantic is throwing
%me off here. It implies NLP. Word/sentence meaning. What is
%semantic in the context of spatial?}
Conversely, trajectory simplification \cite{Zhang2016e} can be
applied to remove redundant points.% when the sampling rate is
%high.

\myparagraph{Trajectory Compression}
Existing trajectory compression techniques can be divided into two
groups: simplification-based and road network-based.
Excluding extra points is a common space reduction method when the
sampling rate is high, and is commonly referred to as {\em trajectory
simplification} \cite{Zhang2016e}, and also used in
trajectory cleaning as discussed above.
Removing points can reduce size, but must be used carefully as it can
also reduce the resolution when analyzing the data.
To alleviate this problem, an error ratio can be applied to bound the
loss for specific computations and data processing operations that
are predefined before data simplification~\cite{Long2013}.

Alternatively, a road network can be used to enable better
compression \cite{Song2014} with little or no
reduction in quality, for certain types of data.
Each trajectory is projected onto a road network as a sequence of
road segments.
Next, each road segment is uniquely encoded using \textit{Huffman coding}
\cite{cormen2009introduction}.
Each trajectory is succinctly represented as a concatenation
of the codewords, and is significantly more effective than
attempting to compress the raw floating point value pairs (latitude
and longitude).
Further, string compression techniques \cite{Yang2017b} can
be used directly on the trajectory data, and any temporal information
can also be succinctly stored using these techniques.

\myparagraph{Map-matching}
Using a road network, map-matching \cite{Lou2009,Newson2009} projects
a raw trajectory onto a real path, and supports cleaning and
compression.
%--JSC-- Good to know but not really important here is it?
%The road network dataset for the whole world is available from
%\textsc{OpenStreetMap}\footnote{\url{https://www.openstreetmap.org/}}.
A road network is modeled as a weighted graph
\cite{cormen2009introduction}, where a road segment is an edge, and
its weight represents the length of this road.
Consequently, a path mapped from a raw trajectory is a set of connected edges
in a road network.

\vspace{-0.5em}
\begin{definition}\textbf{(Road Network)}
A road network is a directed graph $G=(V, E)$, where $V$ is a set of
vertices $v$ representing the intersections and terminal points of
the road segments, $E$ is a set of edges $e$ representing road
segments, and each vertex has a unique id allocated from $1$ to $|V|$.
\end{definition}

\begin{definition}\textbf{(Mapped Trajectory)}
Given a raw trajectory $T$ and a road network $G$, we map ${T}$ to a
road network path $P$ which is composed of a set of connected edges
in $G$, such that ${T}:e_1\rightarrow e_2\rightarrow
\ldots\rightarrow e_{m}$, and denoted as $T$ containing a series of
edge IDs.
\end{definition}

Map-matching techniques should consider both effectiveness and
efficiency.
Efficient algorithms enable us to find the nearest road segments for
each point in the trajectory, and are required in order to connect the
candidate road segment to the best path.
Uncertainty is often the biggest hurdle, and is a reflection of 
parameter selection, which would reduce the number of potential candidate
paths during shortest path search in $G$.
For effectiveness, mapping a trajectory to the true traversal
path of a vehicle when errors in the data can be substantial is
a key limiting factor.

To measure effectiveness, a ground truth is required, and is a
problem in its own right.
There are three common ways to generate a ground truth for the
map-matching problem: 1) using real vehicles equipped with GPS
devices on the road~\cite{Newson2009}; 2) human
adjudication~\cite{Lou2009}; and 3) simulated GPS sampling
\cite{Jagadeesh2004} which is the least costly approach. %, but has its
%own limitations.% \shane{Presumably we discuss in detail what
%these limitations are somewhere?}

\section{Trajectory Similarity Measures}\label{sec:distance}
This section will introduce the most widely used
similarity measures to compare two trajectories.
Fig.~\ref{fig:distance-example} presents two different types
of query-to-trajectory similarity measures.
Labels on each dashed line denote the distance from a query point to
a point in the trajectory.

\subsection{Point-to-Trajectory}
A $k$ Best Connected Trajectories search
(\kbct)~\cite{Chen2010a,Qi2015,Tang2011} is arguably the most commonly
employed formulation of point-to-trajectory similarity search.
To compute the result, each query point $q \in Q$ is paired with the
closest point $p \in T$, and the sum of the distances for all pairs
are aggregated to generate the final distance (similarity) score: $d_{\svar{kBCT}}(Q,T) = \sum_{q\in Q}{\min_{p\in T} d(q, p)}$.
\begin{comment}\small
\label{equ:kbct}
d_{\svar{kBCT}}(Q,T) = \sum_{q\in Q}{\min_{p\in T} d(q, p)}
\end{comment}

For example, applying $d_{\svar{kBCT}}(Q,T)$ to
Fig.~\ref{fig:distance-example} yields
$d_{\svar{kBCT}}(Q_1, T_1)=1+1.7+2.2=4.9$, computed as
(a) is the sum of the distance between every query point in $Q$ to
its nearest neighbor in $T$ (the three dotted lines).
When there is only a single query point, the problem reduces to a
\knn query~\cite{Ding2018,Wang2014e}.
Since this solution requires every point in every trajectory in a
collection to be considered in order to locate the the nearest point
for all $q\in Q$, the complexity of a brute force solution is
quadratic.
Note that this distance measure can only be computed when the query
$Q$ is a set of points, and does not obey the symmetry rule, i.e.,
$d(Q,T)\ne d(T,Q)$.

\begin{figure}
	\centering
	\includegraphics[height=1.6cm]{graph/distance-measure1.pdf}
	\vspace{-1em}
	\caption{Two types of similarity measures: (a) a query is a set of points; (b) a query is a trajectory.}
	\vspace{-1.5em}
	\label{fig:distance-example}
\end{figure}
%or precisely $O(|Q|n|T|)$ where $n$ is the number of
%trajectories in the collections, and $|Q|$ and $|T|$ are the number
%of points in the query and trajectory respectively.
%\shane{This is clearly a naive bound. Even without indexing there
%are textbook solutions for NN which are nlogn. Might be advisable
%to ignore complexity entirely at this point of the paper?}


An alternative to summing the distances between all nearest neighbor
pairs is another well-known measure called the \textit{closest-pair
distance (CPD)}
\cite{Zheng2015b}, which minimizes distance as follows: 
$d_{\svar{CPD}}(Q,T) = \min_{q\in Q}{\min_{p\in T} d(q, p)}$.
%\vspace{-0.5em}
\begin{comment}
\small
d_{\svar{CPD}}(Q,T) = \min_{q\in Q}{\min_{p\in T} d(q, p)}
\end{comment}
Then $d_{\svar{CPD}}(Q_1, T_1)=1$ in Fig.~\ref{fig:distance-example}.
%\shane{This is referencing the example?
%Need to make it clear.}
When compared with $d_{\svar{kBCT}}$, $d_{\svar{CPD}}$ is more robust
when erroneous points exist in a trajectory.

\subsection{Trajectory-to-Trajectory}
One weakness in point-to-trajectory measures is that they do not
capture the true ordering of points.
However, many applications of trajectory search expect an ordering
constraint to hold.
That is, the similarity measure should satisfy a 
\textit{local time shifting} \cite{Chen2005a} constraint.

\begin{table}
	\ra{1}
	\centering
	\caption{An overview of existing trajectory-to-trajectory similarity measures.}
	\vspace{-1em}
	\scalebox{0.75}{\begin{tabular}{cccccccc}
		\toprule\addlinespace[0pt]\rowcolor{gray!30}
		 & & & & & \multicolumn{3}{c}{\textbf{Robustness}} \\ \addlinespace[-1pt]\cmidrule{6-8}\addlinespace[-2.5pt]\rowcolor{gray!30}
		\multirow{-2}{*}{\textbf{Type}} & 	\multirow{-2}{*}{\textbf{Measures}} & \multirow{-2}{*}{\textbf{Complexity}} & \multirow{-2}{*}{\textbf{Metric}} & \multirow{-2}{*}{\textbf{\makecell{No Parameter}}} & \textbf{\small GPS Error} & \textbf{\small Sampling Rate} & \textbf{\small Point Shift} \\ \addlinespace[0pt]\midrule
		\multirow{2}{*}{Curve} & Hausdorff \cite{Roh2011} & $\mathcal{O}(n^2)$ & \cmark &\cmark&\xmark&\xmark &\xmark\\ %	\cmidrule{2-8}
		& DFD \cite{Eiter1994} & $\mathcal{O}(n^2)$ & \cmark&\cmark &\xmark&\xmark &\xmark \\\midrule				
		\multirow{2}{*}{Real} & {\dtw} \cite{yi1998efficient} & $\mathcal{O}(n^2)$ & \xmark&\cmark&\xmark&\xmark &\xmark\\ %\cmidrule{2-8}
		& {\erp} \cite{Chen2004} & $\mathcal{O}(n^2)$ & \cmark&\xmark &\xmark&\xmark &\xmark\\ \midrule
		\multirow{2}{*}{Edit} & {\edr} \cite{Chen2005a} & $\mathcal{O}(n^2)$ & \xmark &\xmark &\cmark&\xmark &\xmark\\ %\cmidrule{2-8}
		& {\lcss} \cite{vlachos2002discovering} & $\mathcal{O}(n^2)$ & \xmark&\xmark &\cmark&\xmark &\xmark \\ \midrule
		\multirow{2}{*}{Temporal}		& {DISSIM} \cite{Frentzos2007} & $\mathcal{O}(n^2)$ & \xmark&\xmark &\xmark&\cmark &\xmark \\ 
					& {EDwP} \cite{ranu2015indexing} & $\mathcal{O}(n^2)$ & \xmark&\cmark &\xmark&\cmark &\xmark \\ \midrule
			\multirow{2}{*}{Segment} 		& \makecell{{LORS} \cite{Wangsheng2018}, LCRS \cite{Yuan2019}} & $\mathcal{O}(n^2)$ & \xmark&\cmark &\cmark&\cmark &\cmark \\
					& {EBD} \cite{Wangaclustering} & $\mathcal{O}(nlog(n))$ & \cmark&\cmark &\cmark&\cmark &\cmark \\ 					 
		\bottomrule
	\end{tabular}}
	\label{tab:distancemeasures}
		\vspace{-1em}
\end{table}


\subsubsection{Pointwise Measures}
%Several similarity measures have been proposed for trajectory data in
%recent years.
We now provide a taxonomy of similarity measures that can be used to compare and contrast each of them.
As shown in Table~\ref{tab:distancemeasures},  we broadly divide the
most commonly used similarity measures into five categories:
curve-based, real-distance, edit-distance, temporal-aware, and
segment-based.
Each of these will now be described in more detail, and the example
shown in Fig.~\ref{fig:distance-example}(b) will be used to more
concretely illustrate important properties for each measure.

Since a trajectory can also be viewed as a \textit{geometric curve},
Hausdorff distance~\cite{Roh2011} measures the
separation between two subsets of a metric space adversarially, without
imposing an ordering constraint.
Informally, it is the maximum of the distances between each point in a
set $Q$ to the {\em nearest} point in the reference set (trajectory $T$): {\small $d_{\tvar{Hau}}(Q,T)=\max_{q\in Q}{\min_{\ p\in T} {d(p,q)}}$}.\footnote{Note that $d_{\tvar{Hau}}(Q,T)$ is the directed distance from $Q$ to $T$. A more general definition which obeys the symmetry and triangle inequality would be: $\max \{d_{\tvar{Hau}}(Q,T), d_{\tvar{Hau}}(T,Q)\}$, and is metric as shown in Table~\ref{tab:distancemeasures}.}

%\vspace{-0.5em}
\begin{comment}\small
\label{equ:hau}
d_{\tvar{Hau}}(Q,T)=\max_{p\in T}{\min_{\ q\in Q} {d(p,q)}}
\end{comment}

Discrete Fr\'echet Distance~{\cite{Eiter1994}} (DFD) extends the
Hausdorff distance to account for location and ordering of the points
along the curve, as shown in Equation~\ref{equ:fre}, where $p$ and
$q$ are the head (first) point of $T$ and $Q$, respectively, and
$T_h$ and $Q_h$ are the sub-trajectory excluding the head $p$ and
$q$.
Accordingly, using the example in Fig.~\ref{fig:distance-example}(b),
$d_{\tvar{Hau}}$ and $d_{\tvar{DFD}}$ will return the same value
$3.1$, since the matching shown in the figure not only finds the nearest
neighbor for each point but also obeys local time shifting (the order
constraint discussed above).
If any two points in $T_5$ swap locations, $d_{\tvar{Hau}}$ does not
change while $d_{\tvar{DFD}}$ could.

\vspace{-1em}
\begin{equation}\small
\label{equ:fre}
d_{\tvar{DFD}}(Q,T)=\begin{cases}d(p, q),\ \text{if}\ Q=\{q\}\ and\ T=\{p\}\\
\infty,\ \text{if}\ Q=\emptyset\ or\ T=\emptyset\\
\max\{d(q, p), \min\{d_{\tvar{DFD}}(Q_h,T_h),\ d_{\tvar{DFD}}(Q, T_h), d_{\tvar{DFD}}(Q_h, T)\}\},\ \text{otherwise}
\end{cases}
\end{equation}
%\vspace{-1em}

\medskip

Since a trajectory can be also viewed as a time series, many similarity
measures originally designed for time series search can be leveraged
in trajectory related problems~{\cite{Zheng2015b}}.
Time-series measures which have been applied to trajectory data
include Dynamic Time Warping (\dtw) \cite{yi1998efficient}, Longest
Common Subsequence (\lcss)
\cite{vlachos2002discovering}, and Edit Distance for Real
sequences (\edr) \cite{Chen2005a} and Edit distance with Real Penalty
{(\erp)}~\cite{Chen2004}.
{\dtw} computes the distance based on the sum of minimum distances,
instead of choosing the maximum as in Discrete Fr\'echet Distance, as shown in
Equation~\ref{equ:dtw}.
To compute {\dtw} for Fig.~\ref{fig:distance-example}(b), every
possible pairing of points in $T_5$ and $Q_3$ are compared in order,
and the sum of the minimum of each pairing
{\small $d_{\tvar{DTW}}(Q_3,T_5)=1.2+3+1+2.2+3.1=10.5$}.
%Note that {\dtw} satisfies an ordering constraint, which is enforced
%using a window constraint $w$ that controls the match point order
%such that $|o(p)-o(q)|\le w$, where $o(p)$ denotes the order of $p$
%in $T$. %\shane{is this $r$ or $w$? I think you mean $w$?}
%The window parameter $w$ is widely used in time series data,
%and may or may not be applied to trajectories, depending on the
%problem.

\vspace{-0.5em}
\begin{equation}\small
\label{equ:dtw}
d_{\tvar{DTW}}(Q,T)=\begin{cases}d(p, q),\ \text{if}\ Q=\{q\}\ and\ T=\{p\}\\
\infty,\ \text{if}\ Q=\emptyset\ or\ T=\emptyset\\
d(q, p)+\min\{d_{\tvar{DTW}}(Q_h,T_h),\ d_{ \tvar{DTW}}(Q, T_h),\ d_{\tvar{DTW}}(Q_h, T)\},\ \text{otherwise}
\end{cases}
\end{equation}
%\vspace{-0.5em}

\medskip

Instead of computing the real distance, computing an edit distance (0
or 1) can be more robust for noisy data as outliers can heavily
impact {\dtw}-based comparisons.
To judge whether two points are matched, edit-distance based measures
set a range threshold $\tau$, i.e., $\var{match}(p, q)=\var{true},\ \text{if}\ |p_x- q_x|\le\tau\ \text{and}\ |p_y-q_y|\le\tau$, where $| |$ denotes the absolute value, and $p_x$
and $p_y$ denote the latitude and longitude of point $p$,
respectively. % \shane{DANGER. Notation issue. We use $|x|$ to this point
%to denote length. It can also denote absolute value. You should fix.
%Maybe $\|x\|$ for L1?}
Now \lcss and \edr can be defined as shown in Equation~\ref{equ:lcss}
and Fig.~\ref{equ:edr}.
The main difference between \lcss and \edr is that \lcss 
measures the similarity between two trajectories, while \edr 
measures the {\em dissimilarity}.
For example, consider $\tau=0.5$ for each of these in
Fig.~\ref{fig:distance-example}(b).
The result is no matching point for $d_{\scriptscriptstyle
\tvar{LCSS}}(Q_3,T_5)=0$ and $d_{\scriptscriptstyle
\tvar{EDR}}(Q_3,T_5)=4$.
If $\tau=5$, then every point can be matched, and
$d_{\scriptscriptstyle
\tvar{LCSS}}(Q_3,T_5)=4$ and $d_{\scriptscriptstyle
\tvar{EDR}}(Q_3,T_5)=0$.
Hence, both measures are sensitive to the hyperparameter
$\tau$.

%\vspace{-0.5em}
\begin{comment}\small
\label{equ:match}
\var{match}(p, q)=\begin{cases}\var{true},\ \text{if}\ |p_x- q_x|\le\tau\ \text{and}\ |p_y-q_y|\le\tau\\
\var{false},\ \text{otherwise}
\end{cases}
\end{comment}


\vspace{-0.5em}
\begin{equation}\small
\label{equ:lcss}
d_{\scriptscriptstyle \tvar{LCSS}}(Q,T)=\begin{cases}0,\ \text{if}\ Q=\emptyset\ \text{or}\ T=\emptyset\\
1+d_{\scriptscriptstyle \tvar{LCSS}}(Q_h, T_h),\ \text{if}\ \var{match}(p,q)=\var{true}\\
\max\{d_{\scriptscriptstyle \tvar{LCSS}}(Q, T_h),\ d_{\scriptscriptstyle \tvar{LCSS}}(Q_h, T)\},\ \text{otherwise}
\end{cases}
\end{equation}

%\medskip

\vspace{-0.5em}
\begin{flalign}\small
\label{equ:edr}
d_{\scriptscriptstyle \tvar{EDR}}(Q,T)=\begin{cases}
|Q|\ or\ |T|,\ \text{if}\ T=\emptyset\ or\ Q=\emptyset\\
\min\{d_{\scriptscriptstyle \tvar{EDR}}(Q_h,T_h), d_{\scriptscriptstyle \tvar{EDR}}(Q, T_h)+1,\ d_{\scriptscriptstyle \tvar{EDR}}(Q_h, T)+1\},\ \text{if}\ \var{match}(p,q)=\var{false} \\
\min\{1+d_{\scriptscriptstyle \tvar{EDR}}(Q_h,T_h), d_{\scriptscriptstyle \tvar{EDR}}(Q, T_h)+1,\ d_{\scriptscriptstyle \tvar{EDR}}(Q_h, T)+1\},\ \text{otherwise}
\end{cases}
\end{flalign}
%\vspace{-0.5em}

\medskip

Since these measures (\dtw, \lcss, and \edr) do not obey the triangle inequality, which is
an essential requirement for \textit{metric} space pruning, all of the
time-series similarity measures are \textit{non-metric} except for
{\erp} \cite{Chen2004}.
In \erp, a point $g$ can be any fixed point in a metric space, and is used as
the reference origin point $g=\{0,0\}$.
Changing $g$ can also change
distance scores similar to \lcss, which can result in 
{\knn}-based algorithms being non-deterministic. %so care should be used
%when applying this similarity metric to trajectory data. \shane{Do
%we have a cite for this?}
%Hence, parameter-free measures are highly desirable for
%trajectory-based search applications.

\vspace{-1em}
\begin{flalign}\small
\label{equ:erp}
d_{\scriptscriptstyle \tvar{ERP}}(Q,T)=\begin{cases}\sum_{p\in T}d(g, p),\ \text{if}\ Q=\emptyset\\
\sum_{q\in Q}d(q, g),\ \text{if}\ T=\emptyset\\
\min\{d_{\scriptscriptstyle \tvar{ERP}}(Q_h,T_h)+d(q, p),d_{\scriptscriptstyle \tvar{ERP}}(Q, T_h)+d(g, p),d_{\scriptscriptstyle \tvar{ERP}}(Q_h, T)+d(q, g)\},\ \text{otherwise}
\end{cases}
\end{flalign}
%\vspace{-1em}

\subsubsection{Temporal-aware Pointwise Similarity}
The aforementioned six measures are the representative of commonly
deployed similarity measures for spatial-only trajectory applications.
In addition to spatial information, temporal information is also an
important factor in accurate sample rate calibration.\footnote{{Actually all aforementioned spatial-only measures can be easily extended to handle the spatio-temporal case, by performing two separate distance calculations on the spatial and temporal features, and then combining the score by using a balancing factor $\alpha$.}}
\citet{Frentzos2007} proposed a measure called {\footnotesize \textsf{DISSIM}} to compute the
dissimilarity: $d_{\svar{DISSIM}} = \int_{t_1}^{t_n}d(Q_t, T_t)dt$. Here, $Q_t$ and $T_t$ denote the points of $Q$ and $T$ at timestamp
$t$ in the range $[t_1, t_n]$.
The core idea is to integrate time w.r.t.\ Euclidean distance for
trajectories occurring in the same period.
%\vspace{-0.5em}
\begin{comment}\small
d_{\svar{DISSIM}} = \int_{t_1}^{t_n}d(Q_t, T_t)dt 
\end{comment}
%\vspace{-0.5em}
{\footnotesize \textsf{DISSIM}} can resolve various sampling rate problems commonly
encountered through integration, but can also be computationally
expensive.
To alleviate this issue, {\footnotesize \textsf{EDwP}}
\cite{ranu2015indexing} calibrates trajectory manipulations by adding
or removing points to align the sampling rate between any two
trajectories, and computes similarity as described for {\edr}.

\subsubsection{Segment-based Similarity}
\label{sec:segmentsim}
Temporal-aware pointwise methods can compute similarity
in much richer trajectory data, but results often have precision
issues unless sample-rate calibration is applied.
Another alternative is to convert trajectories to segments.
This approach has been shown to reduce sample mismatch effects
as well as reducing the complexity of the similarity computations
applied.
\citet{Tiakas2009} was among the first to propose this solution for
road networks.
The approach uses the sum of the distances between nodes in the road
network that contribute to the final distance, but the trajectory
pairs must have the same length in order to guarantee point-to-point
matching.
%\shane{More? What measure did they use? How does it reduces the complexity? In theory? In practice?}
To circumvent the length constraint, \citet{Mao2017} proposed a
related solution which used \dtw after converting pointwise
trajectories to paths on a road network.
In both approaches, the similarity is still computed based on
the end-points of road segments, so map matching is only applied once to
clean trajectory data and to align sampling rates, but it still needs
to compute the Euclidean distance between nodes which can be computationally
expensive even is small data sets.

%\shane{Why? How? Theory? Do you
%mean its not scalable? The bottleneck is map-matching or DTW?}
To reduce the costs in when computing the distances,
\citet{Wangsheng2018} proposed the use of
\textit{longest overlapped road segments} (\lors). 
%\shane{Again,
%complexity? Theoretically or practically? Every time I see the 
%word complexity I and most others will expect a provable order of
%magnitude improvement.}
This measure was inspired by {\lcss} and adapted to leverage the
properties inherent in map-matched data.
{\lors} does not compute the Euclidean distance between points to
determine if they adhere to a threshold distance constraint.
Instead, overlapping segments between trajectories are identified
first, and then reused to compute the similarities.

\vspace{-0.5em}
\begin{equation} \small
\label{equ:lors}
d_{\svar{LORS}}(Q,T)=
\begin{cases}
0,\ \ \ \ \text{if}\ Q\ \text{or}\ T\ \text{is empty} \\
|e_{1m}|+d_{\svar{LORS}}(Q_h,T_h), 
\ \ \ \ \text{if}\ e_{1m}=e_{2x}\ \\
\max(d_{\svar{LORS}}(Q_h,T),d_{\svar{LORS}}(Q,T_h)),\text{otherwise}
\end{cases}
\end{equation}
%\vspace{-1em}

\smallskip

Here, the inputs are $Q=(e_{11},e_{12},...,e_{1m})$ and
$T=(e_{21},e_{22},...,e_{2x})$, where $e_{1m}$ are the end edge of
trajectory $Q$, and $|e_{1m}|$ is the travel length of a graph edge
$e_{1m}$.
\citet{Yuan2019} further extended and normalized {\lors} to account for 
trajectory length effects in $|Q|$ and $|T|$.
The resulting measure LCRS can be defined as: {\small
$d_{\svar{LCRS}}(Q,T) =
\frac{d_{\svar{LORS}}(Q,T)}{|Q|+|T|-d_{\svar{LORS}}(Q,T)}$}.
%\vspace{-0.5em}
\begin{comment}
\small
d_{\svar{LCRS}}(Q,T) = \frac{d_{\svar{LORS}}(Q,T)}{|Q|+|T|-d_{\svar{LORS}}(Q,T)}
\end{comment}
%\vspace{-0.5em}
By modeling network-constrained trajectories as strings in a similar
manner, {\citet{Koide2020}} proposed a generalized metric called
\textit{weighted edit distance} ({\small WED}), which supports
user-defined cost functions that can be used with several important
similarity functions such as {\erp} and {\edr}.

Both {\lors}, {\small LCRS}, and {\small WED} satisfy the local time
shift constraint, and have a quadratic complexity using dynamic
programming.
\citet{Wangaclustering} later simplified the computational 
costs of \lors further.
The key insight was to exploit ordered integer intersection (through
finger search), where ordered integers represented unique IDs
assigned to road segments during map-matching.
The resulting method called {\em edge-based distance}-EBD: {\small
$d_{\svar{EBD}}(Q, T) = \max(|Q|,|T|)-|Q\cap T|$}, was shown to have
comparable precision to {\lors} and was also highly scalable in
practice.

%\vspace{-0.5em}
\begin{comment}\small
\label{equ:ebd}
d_{\svar{EBD}}(Q, T) = \max(|Q|,|T|)-|Q\cap T|
\end{comment}
%\vspace{-1em}

%Note that converting all trajectories in a collection to
%fixed-dimension vectors of the same length enables Euclidean distance
%computations in linear time~\cite{Yao2017,Yao2019,Li2018a,Sanchez2016}, \sheng{which is known as \textit{trajectory embedding} and we will elaborate in Section~\ref{sec:deep}.}
%However, these are machine learned approaches, requiring additional
%training in order to model effective transformations.
%\shane{Is this right?
%It is a little unclear what you were asserting.}
%Several common trajectory operations such as range queries or
%sub-trajectory search can not be applied to the new vector
%representations.

\subsection{Complexity and Robustness}

Table~\ref{tab:distancemeasures} compares characteristics of
similarity measures based on four different properties: complexity,
metricity, parameter independence, and robustness.
Since parameters such as $\tau$ in \lcss and \edr can be easily
observed from their definitions, we will elaborate the other three
characteristics next.

\myparagraph{Complexity} Many trajectory-based similarity measures
were designed to allow search to be more resilient to variance
produced by local time shifting.
However, computing optimal distances with ordering constraints
generally requires dynamic programming solutions with quadratic
complexity ($\mathcal{O}(n^2)$) as well as the associated space
overheads.
\iffalse
One alternative is to employ learned embeddings~\cite{Yao2017} to
compute the Euclidean distance based on vectors with fixed length,
allowing linear ($\mathcal{O}(n)$) computational costs, but machine
learned solutions bring their own trade-offs, such as training time
and loss of bounded performance guarantees. \shane{It may not be
appropriate to compare ML and algorithmic solutions in this way.
They are not the same at all really.
You might argue that we do not consider ML as other related surveys
focus on this much more.}
\fi

%\vspace{1em}
\begin{figure}
	\begin{minipage}{0.67\textwidth}
		\centering
		\includegraphics[width=1\linewidth]{graph/robustness.pdf}
		\vspace{-1.5em}
		\caption{A similarity measure that is sensitive to point shift, error, and sampling rate.
			}\vspace{-1.2em}
 \label{fig:robustness}
	\end{minipage}\hfill
	\begin{minipage}{0.3\textwidth}
		\centering
		\includegraphics[width=1\linewidth]{graph/spatial-only-queries.pdf}
		\vspace{-1.5em}
		\caption{Three kinds of spatial-only trajectory queries.}
		\vspace{-1.2em}
 \label{fig:queries}
	\end{minipage}
\end{figure}

\myparagraph{Metricity} Fully metric compliance is often crucial for
a similarity measure, as obeying the triangle inequality provides
both theoretical and practical advantages.
Here, we use an example to illustrate the concept.
Consider the computation of the well-known metric similarity measure,
Euclidean distance.
Given a query point $q$ with $p_1$ and $p_2$ as the two next
candidates for a \knn query, $d(q,p_1)$ is computed.
Before distance is computed for $p_2$, the lower and upper bound of
$d(q,p_2)$ can be estimated based on $d(q,p_1)$ and $d(p_1, p_2)$ as:
{\small $ |d(q, p_1)-d(p_1, p_2)|<d(q,p_2)<d(q,p_1)+d(p_1, p_2) $},
where $d(p_1, p_2)$ can be precomputed off-line for any query.
The lower bound can be compared with $d(q, p^{'})$ where $p^{'}$ is
currently the best nearest neighbor candidate.
If the bound is greater than the current best result, we can discard
$p_2$ directly as it can never replace $p^{'}$.

\myparagraph{Robustness}
In addition to complexity and metricity, many similarity measures are
sensitive to noise, sampling rate, and point shifting (points are
shifted on the path where the trajectory lies).
The existence of noise due to GPS errors or other common sensor data 
collection approaches result in more
(or fewer) sampled points, point shifting, and other quality issue.
\citet{Wang2013a} systematically compared the robustness of 
six common similarity measures in a real-world trajectory
dataset, and a complete version \cite{Su2019b} was published later
with additional point-based measures.
However, the most recent segment-based measures
\cite{Wangsheng2018,Yuan2019} were not covered.
%\shane{And concluded what?}
%\citet{Toohey2015} implemented an R package capable of easily
%computing these measures in a single, integrated environment.
%\shane{This seems out of place.
%Maybe earlier when they are introduced?}

Fig.~\ref{fig:robustness} illustrates several common robustness
problems encountered in trajectory data.
$T_1$ and $T_2$ are two vehicle trajectories in a road network that
overlap.
After sampling, a set of points represents each one, with perfect
data resulting in (b).
In reality, sampling rates can vary, resulting in a point shift
(c).
GPS errors (d) can also occur in sampled points that are not on the
same road, and inconsistent sampling rates (e) lead to a different
number of points being produced for the two trajectories.
Each of the above issues can lead to distance scores greater than
those found in error free data, and can even result in incorrect
solutions for certain query types.
Robust similarity measures are therefore highly desirable.%when
%being applied to real-world data.



\section{Trajectory Search and Join}
\label{sec:spatialonly}

\subsection{Spatial-only Trajectory Search}
Fig.~\ref{fig:queries} shows three exemplar queries $Q_1$, $Q_2$,
$Q_3$ for the spatial-only trajectories $T_1$ to $T_6$.
Given three points ($q_1$, $q_2$, $q_3$), $Q_1$ finds the best
connected trajectory.
Among all six trajectories, $T_1$ and $T_2$ are both possible 
solutions.
For a pointwise similarity search as shown in $Q_1$,
the similarity measure used should ideally be able to reliably
distinguish between the two candidates.
Given a target range (red box), $Q_2$ finds all trajectories covered
(partially or fully).
Valid results are $T_3$ and $T_4$, and can not be computed using any
of the similarity measures shown.
In comparison, if $Q_3$ is the query for the top-$k$ search, a
similarity measure must to be defined that can capture all of the
properties of $Q_3$, including points and ordering.

\begin{table*}
	\centering
	\ra{0.8}
\caption{{An overview of common operations applied to trajectory and
point data.}}
\vspace{-1em}
	\begin{comment}
	$k$NN: $k$ 
	Nearest Neighbour \cite{Guttman1984},
	TkSK: Top-k Spatial Keyword Query~\cite{chen2013spatial}, 
	ANN: Aggregate Nearest Neighbour Query~\cite{Papadias2005},
	ATNN: Aggregate Textual Nearest Neighbour Query~\cite{Li2010,Yao2016},
	kBCT: k Best-Connected-Trajectory Query~\cite{Chen2010a}, 
	TkSTT: Top-$k$ Spatial-Textual Trajectory Query~\cite{Wang2017,Shang2012a}.
	\end{comment}
	\label{tab:methods}
	\scalebox{0.76}{\begin{tabular}{ccccccc}
			\toprule\addlinespace[0pt]\rowcolor{gray!30}
			\textbf{Data}&\textbf{Type}&\textbf{Query} & \textbf{Input} & \textbf{Output} & \textbf{Measure}& \textbf{Index} \\\addlinespace[-2pt]
			\midrule
			\multirow{9}{*}{\makecell{Spatial\\-only}}	&\multirow{2}{*}{Basic}& Range \cite{SanduPopa2011,Krogh2016} & range & trajectories& N/A & R-tree \\
			&& Path \cite{Krogh2016,Koide2015} & path & trajectories& N/A & R-tree \\
			\cmidrule{2-7}
			&\multirow{4}{*}{$k$NN}&\knn~\cite{Guttman1984,beckmann1990r} & point & points & Euclidean & R-tree \\
			&&$k$NNT \cite{vlachos2002discovering,Chen2005a,Shang2018}& trajectory & trajectories& LCSS, DTW & R-tree \\
			&&\kbct \cite{Chen2010a,Tang2011}& points & trajectories& Aggregate & R-tree \\
			\cmidrule{2-7}
			& \multirow{2}{*}{\makecell{Reverse\\ $k$NN}} & \rknn \cite{Tao2004}& \makecell{point} & points& Euclidean & R-tree \\
			& & \rknnt~\cite{Wang2018c}& {trajectory} & trajectories & CPD & N/A \\
			\cmidrule{2-7}
			& \multirow{2}{*}{Clustering} & Density \cite{Lee2007}& \makecell{thresholds} & paths& N/A & N/A \\
			& & Partition \cite{Wangaclustering}& \makecell{$k$} & trajectory& EBD & Inverted index \\ 	\cmidrule{2-7}
			 & \multirow{2}{*}{Join} & \makecell{similarity join} \cite{Ta2017,Yuan2019}& threshold & pairs& Normalized CPD & signature \\
			 & & \knn join \cite{Fang2016}& $k$ & pairs& CPD & Grid-index \\
			\midrule
			\multirow{3}{*}{\makecell{Spatial\\-textual}}	& &\textbf{KS} \cite{Broder2003,Ding2011a} & keywords & points & TF-IDF & Inverted list \\
		& \multirow{2}{*}{Top-$k$} &\tksk \cite{zhang2014processing,Li2011} & \begin{tabular}{c}point, keywords\end{tabular} & points & Aggregate & IR-tree \\
			& &\tkstt \cite{Shang2012a,Zheng2013c}& \begin{tabular}{c}points, keywords\end{tabular} & trajectories & Aggregate & \begin{tabular}{c}Grid-index, \\Inverted list\end{tabular} \\
			\bottomrule
	\end{tabular}}
	\vspace{-1em}
\end{table*}

Table~\ref{tab:methods} compares and contrasts several common
trajectory queries by input, output, similarity measure, and most
appropriate index.
The ``Index'' column shows the preferred indexing approach.
Many other alternatives exist.
A more comprehensive analysis and discussion of indexing solutions is
in Section~{\ref{sec:spatialindexing}}.
Query types range from basic trajectory search, top-$k$ trajectory
similarity search (spatial-only and spatial-textual), to more complex
operations such as reverse $k$ nearest neighbors search, and
trajectory clustering.
We now discuss each of these query operations in detail along with
several indexing techniques which have been proposed to accelerate
performance.

\subsubsection{Basic Trajectory Search}
Basic trajectory search includes three classic query
formulations.
The most basic is a {\em Range Query}
({RQ})~{\cite{SanduPopa2011,Krogh2016,Song2014,Roh2011}} which finds
all (sub-)trajectories located in a spatial or temporal region.
Range queries has many applications in traffic monitoring such as
returning all vehicles at a road intersection.
The second is a {\em Path Query} ({PQ}) which retrieves the
trajectories that contain any edge of the given path query.
The third is a {\em Strict Path Query}
({SPQ})~{\cite{Krogh2016,Koide2015,SanduPopa2011}} which
finds all trajectories that traverse an entire path from
beginning to end.
Interestingly, path queries and strict path queries share many common
properties with disjunctive (OR) and conjunctive (AND) Boolean
queries~{\cite{Christopher2009}}.


\begin{definition}\textbf{(Range Query)}
Given a trajectory database $D = \{T_1,
\ldots, T_{|D|}\}$ and query rectangular region $Q_r$, a range query
	retrieves the trajectories:
$\avar{RQ}(Q_r)=\{T\in D|\exists p_i \in T(p_i\in Q_r)\}$.
\end{definition}


\begin{definition}\textbf{(Path Query)}
Given a $Q_p$ which is a path in $G$, a path query retrieves the
trajectories {$T$ that pass through at least one edge $e_j$ of $Q_p$}: $
\avar{PQ}(Q_p)=\{T \in D|\exists e_i \in {T}, e_j \in Q_p (e_i = e_j)\}
$.
\end{definition}

\begin{definition}\textbf{(Strict Path Query)} 
Given a $Q_p$, a strict path query retrieves the trajectories whose edges can all be found in $Q_p$: $
\avar{SPQ}(Q_p)=\{T\in D|\exists i,j(T_{ij}=Q_p)\}
$, where $T_{ij}=\{e_i,e_{i+1},\cdots,e_j\}$ is the
sub-trajectory of $T$.
\end{definition} 

\subsubsection{$k$ Nearest Neighbors Query}

To find a relevant subset from a large set of objects for a given query object, $k$ nearest neighbor queries have been widely applied in spatial databases. For trajectories, the query can be either a trajectory or a set of points.

\begin{definition}\textbf{(k Nearest Neighbors Query over Trajectories)}
Given a trajectory database $D = \{T_1, \ldots, T_{|D|}\}$ and query
$Q=\{q_1, q_2, \cdots, q_{|Q|}\}$, a $k$ Nearest Neighbors Query
($\knn(Q)$) retrieves a set $D_s \subseteq D$ with $k$ trajectories
such that: $\forall T \in D_s, \forall T^{'} \in D - D_s, d(Q,T) <
d(Q,T^{'})$.
\end{definition}

\myparagraph{Search by Trajectory}
Given a query trajectory $Q$, a $k$ Nearest Neighbor Trajectories
Query aims to find the $k$ most similar/nearest trajectories to
$Q$, based on a given trajectory similarity measure \cite{Xie2017a,Wangsheng2018}.
Such a query can be used to find the most similar trips in traffic
flow analysis.
For the special case when the trajectory is a single point, which is
also known as \knn search (we use \textit{kNNT} to denote trajectory
search), with the default similarity being Euclidean distance.

\myparagraph{Search by Points}
There has also been previous work targeting search on spatial-only
trajectory data where the input query is a set of
points~\cite{Chen2010a,Tang2011,Qi2015}.
\citet{Chen2010a} initially proposed the problem of querying over a
set of points with spatial-only trajectories.
They proposed incremental expansion using an R-tree
to prune candidate points from consideration.
They referred to the approach {\em Incremental K Nearest Neighbors
(IKNN)}.
To optimize the IKNN algorithm,
\citet{Tang2011} devised a qualifier expectation measure that ranks
partially matched candidate trajectories.
The approach accelerates query processing significantly when
non-uniform trajectory distributions and/or outlier query locations
exist in the solution space.
%\citet{Qi2015} went on to combine {\em IKNN} and the qualifier
%expectation model to further improve the efficiency using a
%range-based algorithm and an R-tree.

\subsubsection{Reverse $k$ Nearest Neighbor Query}
\label{sec:rnns}
Instead of searching the most relevant objects to a query object, {\em Reverse $k$ Nearest Neighbors} ({{\rknn}}) queries attempt to locate objects which will take the query as one of their $k$ nearest neighbors. Formally, \rknn is defined as below:


\begin{definition}\textbf{(Reverse k Nearest Neighbor)}
Given a set of points (or trajectories) $D$ and a query point (or trajectory) $Q$, a $\rknn(Q)$
retrieves all objects $\tran \in D$ {that take $Q$ as $k$NN}, i.e., $\forall\tran$,
$Q\in\textbf{\knn}(\tran)$.
\end{definition}

\rknn queries for spatial
point data have attracted considerable attention in the research
community~{\cite{Tao2004}} as it can be used to solve a
wide variety of industry-relevant problems.
An {\rknn} query aims to identify all (spatial) objects that have a
query location as a $k$ nearest neighbor.
Important applications of the {\rknn} query include resource allocation \cite{Wang2018c} and profile-based marketing \cite{Zhang2018c}.
For example, {\rknn} queries can be used to estimate the number of
customers a new restaurant would attract based on location, and was
initially referred to as a \textit{bichromatic} \rknn based on the
dual-indexing solution proposed to solve the problem~\cite{Tao2004}.

Instead of querying a set of static points,
\citet{Cheema2012} proposed the \textit{continuous reverse nearest
	neighbors} query to monitor a moving object.
The goal is to find all static points that contain the moving object
as a $k$ nearest neighbor.
%More recently, \citet{Emrich2014} extended the problem to
%``uncertain'' moving objects and proposed the use of a Markov model.
%A moving object is treated as a result when it always takes the query
%object as the nearest neighbor within a given time interval.
This approach targets a single point rather than a commuter
trajectory of multiple-points, which was later solved in \rknnt~\cite{Wang2018c}.% which is the focus of our work.
%\shane{Presumably the sentence should be replaced with the TKDE
%result with the corresponding explanation?}

\myparagraph{Reverse Trajectory Search}
%\shane{This section was a mess.
%I tried to fix it, but it needs to be reviewed carefully.
%Multiple problems are somewhat randomly combined here.}
%Instead of finding the most similar or nearest trajectories,
%reverse $k$ nearest neighbor queries for trajectory data
%can have several different formulations.
The ``Reverse $k$ Nearest Neighbor Query over Trajectories''
(\rknnt~\cite{Wang2018c}), and can be defined as follows.
Given a trajectory dataset $\mathcal{D}_T$ and a set of routes
$\mathcal{D}_R$ (also defined as trajectory) and a candidate point
set $Q=\left( o_1,o_2,\ldots,o_m \right)$ as a query, \rknnt~returns all
the trajectories in $\mathcal{D}_T$ that will take $Q$ as $k$ nearest
routes using a point-to-trajectory similarity measure.
The main application of \rknnt~is to estimate the capacity of a new
bus route and can be further used to plan a route with a maximum
capacity between a source and destination, which was defined as
a \maxrknnt~in \cite{Wang2018c}.
The main challenge in solving \rknnt~is how to prune the
trajectories which cannot be in the results without explicitly
accessing the whole dataset $\mathcal{D}_T$.
All of the pruning methods commonly used for {\rknn} may work for
trajectories.
For example \textit{half-space} pruning~\cite{Tao2004}, which can prune
an area by drawing a perpendicular bisector between a query point and
a data point will not work.
\citet{Wang2018c} proposed the use of an R-tree of the trajectory
routes (an example can be seen in Fig.~\ref{fig:R-tree-indexing}).
By drawing bisectors between the route points and the query, an area
can be found where all trajectory points contained in a region can
not have the nearest route for the query.
%\citet{Shang2011} found a point $p$ for $\mathcal{D}$ such
%that the number of moving objects that choose $o_i$ as the nearest
%neighbor is maximized. \shane{Not right. Fix. RNN for all points? One
%point? I have no idea what you intended here.}

%\vspace{-1em}

\subsection{Spatial Indexing Algorithms}
\label{sec:spatialindexing}
Trajectory indexing is commonly applied to improve efficiency in 
trajectory related search problems.
Trajectory data is processed off-line to improve scalability and
prune the search space.
Existing approaches to trajectory indexing have two components:
indexable point data and mapping tables.

\myparagraph{Point Indexing}
Space-efficient index representations and processing frameworks are
crucial for trajectory data, and the majority of trajectory
search solutions~\cite{Chen2010a} rely on an
R-tree~{\cite{Guttman1984}}, which store all points from the raw
trajectories, and are historically the dominant approach deployed for
spatial computing applications.
As shown in Fig.~\ref{fig:R-tree-indexing}, trajectories are
decomposed to points first, then an R-tree is used to index each 
point.
A mapping table identifies the trajectory that contains each point.
Since trajectory datasets such as 
T-drive~{\cite{Yuan2010}} can easily contain millions of
points, the R-tree must manage an enormous number of maximum bounding
rectangles (MBR), which have prohibitive memory costs in practice.
So, traditional methods employed for spatial pruning can be
infeasible on raw trajectory data.
Simpler Grid-index solutions can sometimes be more appropriate in
such scenarios~{\cite{Zheng2013c,Wang2021}}.
Nevertheless, the core problem is compounded by the fact that many of
the similarity measures proposed for trajectory search are
non-metric.
%, which creates additional issues that must be overcome as well.

\myparagraph{Mapping Table}
A mapping table is used to map points to trajectories
\cite{Chen2010a,Zheng2013c}.
After searching for a point, the mapping table identifies the
trajectory containing the point.
Ensure that the mapping is unambiguous, every point has a unique
identifier ranging from $[1, |\mathcal{D}.P|]$, each trajectory
has a unique identifier ranging from $[1, |\mathcal{D}|]$,
$|\mathcal{D}.P|$ and $|\mathcal{D}|$ are the number of points and
trajectories.
With the mapping table in Fig.~\ref{fig:R-tree-indexing}(c), we can know that $p_1$ is a point of $T_3$ and $p_2$ belongs to $T_4$.

\myparagraph{Pruning Mechanism}
For range queries, most existing approaches employ MBR-based pruning,
as MBR intersection with a query trajectory can be used to
effectively and efficiently prune the search space.
If a node intersects with a query range, the object covered
can be removed from consideration.
For example, the nodes $N_7$ and $N_8$ in
Fig.~\ref{fig:R-tree-indexing}(a) do not intersect with $N_2$, so
they can be eliminated from consideration, leaving only $N_9$.
For \knn trajectory search, there are two common pruning techniques:
\textbf{early termination} and \textbf{early abandoning}.
Early termination is initially proposed in the threshold algorithm
\cite{Fagin2003}.
Given an index, the algorithm scans a sorted list, and early
terminates when all remaining items exceed some precomputed upper
bound.
It is similar to pruning in {\knn} search with an R-tree where
the minimum distance between the query and a node in
the index can be used to determine if the distance for the
items contained must be computed.
In contrast to early termination which can prune many items
in a single operation, early abandoning must consider each
item but exploits a bound to minimize the number of expensive
computations applied during processing.
This technique is commonly used to accelerate time series similarity
search and {\knn} search~\cite{vlachos2002discovering}.
By estimating the upper bound of the similarity score and comparing
it to the $k$-th item in a max-heap (for top-$k$ search for example),
an algorithm can determine if a full similarity computation must be
made for the item under consideration.

\begin{figure}
	\centering
	\includegraphics[height=4cm]{graph/spatial-indexing.pdf}
	\vspace{-0.5em}
	\caption{Indexing spatial-only trajectories using an R-tree and a mapping table.}
	\vspace{-1.5em}
	\label{fig:R-tree-indexing}
\end{figure}

\subsection{Trajectory Join}
\begin{definition}\textbf{(Trajectory Join)}
	\label{def:join}
	Given two sets of trajectories $S_1$ and $S_2$, and a similarity
	threshold $\epsilon$ (or $k$ in \knn search), a trajectory join
	operation will return all pairs of trajectories $T_i$ and $T_j$ from
	$S_1$ and $S_2$ with a similarity that exceeds $\epsilon$ (or $T_i\in
	\knn(T_j)$).
\end{definition}

The main applications of trajectory joins are in trajectory data
cleaning, near-duplicate detection, and carpooling.
For example, given a driver trajectory database and a rider
trajectory database, a trajectory join will match riders with similar
trajectories to drivers.
Trajectory join operations can be divided into two categories: trajectory similarity joins~\cite{Ta2017} and
trajectory $k$ Nearest Neighbors joins~\cite{Fang2016}.
A simple baseline is to conduct a similarity search or {\knn} search
for each trajectory.
Given the quadratic complexity of this solution, scaling can be
problematic.

To reduce the complexity, many
different indexing techniques can be used.
\citet{Bakalov2008} considered the moving object trajectory similarity
join, which is a pointwise join in a specific timestamp, and
similarity is computed between points and not trajectories.
\citet{Ta2017} proposed a signature-based solution to filter
trajectory pairs before distance computation, 
where the signature is built for each trajectory to help prune, 
based on its crossed and neighbor grids.
%\shane{Same or different
%problem. Not clear.}
\citet{Shang2017} explored the spatial-temporal trajectory similarity
join problem for road networks.
A two-step algorithm is applied to each trajectory: expansion and
verification, similar to trajectory similarity search in
Section~\ref{sec:spatialonly}.

\myparagraph{Distributed Trajectory Similarity Join} Distributed computing is often applied to solve the
trajectory join problem due to the high computational costs of the
distance computation.
\citet{Fang2016} proposed a distributed trajectory \knn join method using MapReduce.
Their solution used Hadoop, and the algorithm can also run on a
single machine.
\citet{Shang2018} computed distributed trajectory similarity joins
using Spark, where a global index is deployed over multiple computer
nodes and used to prune the search space.
%\shane{How? Insights? What made the solution
%interesting?}
\citet{Yuan2019} also explored the distributed trajectory similarity
join problem using similar techniques to \citet{Shang2018}, but 
applied the similarity measure {LCRS}~described in Section~\ref{sec:segmentsim} to compute.

\subsection{Spatial-Textual Trajectory Search}
\label{sec:spatialtextual}
Spatial-textual trajectory search incorporates text and keywords
to the data, and relevant trajectories have more than one
dimension of similarity that must be considered.
For example the keywords ``\textit{seafood}'', ``\textit{coffee}''
and ``\textit{swimming}'' might be contained in a query and a
trajectory.% as shown in Fig.\ref{fig:running}.
%In this example, we see (a): six target trajectories and a query $Q$;
%(b): Keywords with a weight of $T_1$ in each point; (c) Pointwise
%matching between $Q$ and $ T_1 $.)

\begin{comment}
	\begin{center}
		\includegraphics[width=0.66\textwidth]{graph/Running.pdf}
%		\vspace{-1em}
		\caption{An example of top-$k$ spatial-textual trajectory search.}
%		\vspace{-1em}
		\label{fig:running} 
	\end{center}
\end{comment}

\begin{comment}
	\ra{1}
	\centering
	\caption{Comparison between related work on spatial-textual
		trajectory search.}
%	\vspace{-1em}
	\label{tab:com}
	\scalebox{0.8}{\begin{tabular}{cccccccc}
			\toprule\addlinespace[0pt]\rowcolor{gray!30}
			& \multicolumn{2}{c}{\textbf{Input}} & & \multicolumn{2}{c}{\textbf{Search Metric}} & \\ \addlinespace[-2pt]\cmidrule{2-3} \cmidrule{5-6}\addlinespace[-2pt]\rowcolor{gray!30}
			\multirow{-2}{*}{\textbf{Work}}& Query & Data Model & \multirow{-2}{*}{\textbf{Search Semantic}} & Spatial & Textual & \multirow{-2}{*}{\textbf{Output}} \\\addlinespace[-2pt] \midrule
			{\em \pats-based \tkstt} & \makecell{Points with\\keywords} & Trajectory & Disjunctive & Eu & TF$\cdot$IDF & \makecell{Top-$k$ \\Trajectories} \\ \midrule
			\citet{Zheng2013c} & \makecell{Points with\\keywords} & Trajectory & Conjunctive & Eu & N/A & \makecell{Top-$k$ \\Trajectories} \\ \midrule
			\citet{Shang2012a} & \makecell{Points,\\Keywords} & \makecell{Spatial-only \\Trajectory\\ and Keywords} & Disjunctive & Eu & Jac & \makecell{Top-$k$ \\Trajectories} \\ \midrule
			\citet{Cong2012} & \makecell{Point,\\ Keywords} & Trajectory & Conjunctive & Eu & N/A & \makecell{Top-$k$ sub-\\Trajectories}\\ \midrule
			\citet{Zheng2015} & Keywords & Trajectory & Conjunctive & Eu & ED & \makecell{Top-$k$ sub-\\Trajectories}\\ \midrule
			\citet{HanWZZL15} & \makecell{Region, Keywords} & Trajectory & Conjunctive & N/A & N/A & Trajectories \\ \bottomrule
	\end{tabular}}
%	\vspace{-1.5em}
\end{comment}

%\vspace{-1em}

\subsubsection{Top-$k$ Spatial-Textual Trajectory Search}
\label{sec:literature-etq}

\myparagraph{Similarity Measures}
In contrast to spatial-only similarity measures, spatial-textual
measures for an activity trajectory depend on both spatial and
textual components.
Linear combinations of two distinct similarity measures is a common
solution for spatial-textual data~\cite{Cong2009a,zhang2014processing}.
The spatial distance is combined with TF$\cdot$IDF similarity for the
text, with a user-defined weight between the two to balance
importance based on the target application.
Such a measure was also extended by \citet{Shang2012a}, where the
spatial-distance is computed in a manner similar to the \textit{$k$
Best Connected Trajectories query} (\kbct).
The textual similarity was then computed using simple keyword
intersection.
%\shane{This cannot be correct given the next sentence. Fix.}
Since the text relevance is
computed as a part in the final score, it is more flexible in real
applications.
Conversely, a conjunctive approach \cite{Zheng2013c,Cong2012}
tightens the constraint, requiring that the result trajectory should
contain all of the query keywords, and results are ordered by spatial
distance.

\myparagraph{Pointwise Search with Keywords} Several recent papers
have explored the problem of spatial-textual trajectory search in a
range of different scenarios.
%Table~{\ref{tab:com}} reports the differences and similarities
%between existing work in terms of query and data models, search
%semantics, metrics, and result output, where ``Eu'' stands for
%``Euclidean'', ``Jac'' stands for ``Jaccard'' and ``ED'' stands for
%``Edit Distance''.
\citet{Cong2012} proposed a sub-trajectory based solution to find the
minimum travel distance for a single query point using a Boolean
keyword match.
\citet{Shang2012a} presented a disjunctive solution for 
multiple points, where the distance is measured between
points, but keywords are assigned to an entire trajectory instead of
each point.

\citet{Zheng2013c} attached the keywords to a specific point in the
trajectory to allow finer-grained matching of textual information.
However, their work only supported conjunctive text matching, so
results must contain all query keywords, simplifying the more
general keyword search problem.
To handle the case when users do not have a preferred locations
or exact text matching should not be guaranteed,
\citet{Zheng2015} proposed an approximate query solution over
trajectories that use a set of keywords, and the similarity is
measured as the travel distance, just as
\citet{Cong2012} did.
A special case of this problem is when the query contains only
keywords, and is known as a keyword-only search (\textbf{KS})
\cite{Broder2003}.
Another special case is when the trajectory data and query are a
single point, and is known as Top-$k$ Spatial Keyword Search (\tksk)
\cite{zhang2014processing}.

\subsubsection{Boolean Range and Top-$k$ Query}\citet{Hariharan2007} utilized the Boolean range queries to find all objects
containing query keywords, all of which must be located within a bounded
range.
Boolean Top-$k$ queries \cite{DeFelipe2008a} find the $k$ nearest
objects using conjunctive Boolean constraints on the text, i.e., it
conducts a {\knn} search over all the points that contain all the
keywords from query.
%\shane{What is the spatial angle here?
%Not clear at all.}
\citet{HanWZZL15} investigated Boolean range queries on trajectories,
and considered spatial, temporal, and textual information in the
solution, and an index based on an octree and inverted index is proposed to
answer their proposed query. %\shane{Is it octree or octtree?}

%\shane{Not enough. How did they solve
%these problems exactly. What were the challenges and why is their
%solution novel/interesting?}

\subsubsection{Pruning with an Inverted Index}
Inverted indexes~\cite{Zobel2006} are widely used to efficiently
manage text information for spatial-textual problems.
Related algorithms and data structures for inverted indexes have
benefited from many years of practical improvements to support web
search and related applications, making them an obvious candidate
to manage textual components in heterogeneous data collections.
A unique object identifier is mapped to every keyword contained,
and an inverted list of all objects containing each keyword
can only represent existence, or contain auxiliary data such as
the frequency of the keyword in the object text.
The auxiliary data can also be a precomputed similarity score or
even offsets for phrase reconstruction.
Most prior work~\cite{zhang2014processing} attaches
inverted lists to nodes in an existing tree-based spatial index
(a Grid-index for example) in order to support spatial-textual
similarity computations during tree traversal.

\section{Trajectory Clustering and Classification}
\label{sec:clustering}
\subsection{Clustering Large-Scale Trajectories}
Clustering similar trajectories to produce representative exemplars can be a powerful visualization tool to track the mobility
of vehicles and humans.
It has been investigated in many different applications, such as
spatial databases
\cite{Hung2015, Agarwal2018, Lee2007}, data mining
\cite{Pelekis2009}, transportation \cite{Wu2015}, and visualization
\cite{Ferreira2013}.
Clustering is most often applied to spatial-only
trajectories, with prior work on spatial-textual trajectory
clustering being relatively rare.
%Different clustering frameworks consider various features and
%constraints for different scenarios.
Trajectory clustering can be broadly divided into two categories:
Partition-based:
\cite{Chan2018,Ferreira2013,Yao2017,Pelekis2009,Gudmundsson2015,Hung2015} and
Density-based:
\cite{Lee2007,Han2015a,Li2010b,Agarwal2018,Andrienko2009}.
Both the partition and the density-based trajectory clustering require
extensive similarity computations, with the only distinction being if
it is computed for whole trajectories or using only sub-trajectories.

\begin{comment}
	\centering
	\ra{1.2}
	\caption{A summary of existing trajectory clustering work.}
%	\vspace{-1em}
	\label{tab:literature}
	\scalebox{0.8}{
		\begin{tabular}{ccccccc}
			\toprule\addlinespace[0pt]\rowcolor{gray!30}
			\textbf{Type} &\textbf{Work} & \textbf{Measure} & \textbf{Data Scale} & \textbf{\#Parameter} & \textbf{Time} & \\ \addlinespace[0pt]\midrule
				& \citet{Wangaclustering} & $\ebd$ & Million (Vehicle) & 1 & Minute & \\ 
			&\citet{Chan2018} & Hausdorff & 422 (Vehicle) & 4 & Hours & \\
			&\citet{Yao2017} & DTW & 4700 (Vessels) & 2 & N/A & \\
			& \citet{Ferreira2013} & Euclidean & \numb{372601} (Vehicle) & 2 & 2,497s & \\
			Partition& Gudmundsson et al. \cite{Gudmundsson2015} & Fr\'echet & 2 soccer players & 2 & 700s & \\
			&\citet{Pelekis2009} & ERP & 1100 (Vehicle) & 4 & 10s & \\
			&\citet{Wu2015} & EDR & 100 (Cellular) & 3 & 400s & \\
			\midrule
			& \citet{Andrienko2009} & - & \numb{176000} (Vehicle) & $|\mathcal{D}|$ & N/A & \\
			&\citet{Li2010b} & - & 7000 (Vehicle) & 3 & 100s & \\
			Density&\citet{Han2015a} & Hausdorff & 5000 (Vehicle) & 6 & 120s & \\
			&\citet{Lee2007} & - & 570 (Hurricane) & 2 & N/A & \\
			&\citet{Agarwal2018} & Fr\'echet & \numb{20000} (Vehicle) & 3 & 50hours & \\ \bottomrule
	\end{tabular}}
%	\vspace{-1.5em}
\end{comment}
{
\subsubsection{Partition-based Clustering}
Given a set of trajectories, partition-based clustering divides
trajectories into a limited number ($k$) of groups (clusters).
%, and each group has a representative trajectory.
The similarity measure (Section~\ref{sec:distance}) and parameter $k$
are selected a priori depending on the use case.

\begin{definition}\textbf{(Partition-based Trajectory Clustering)}
Given a set of trajectories $\{{T}_1,{T}_2,\cdots,{T}_n\}$,
partition-based clustering aims to partition $n$ trajectories
into $k$ ($k\le n$) clusters $S=\{S_1, S_2, \cdots,S_k\}$ by minimizing
the objective function: $O=\argmin_{S}{\sum_{j=1}^{k}{\sum_{T_i\in
S_j}{d(T_i,\mu_j)}}}$.
\end{definition}

Here, each cluster $S_j$ has a centroid trajectory or path $\mu_j$,
and $d(T_i,\mu_j)$ is a similarity measure.
Many different similarity measures such as the ones introduced in
Section~\ref{sec:distance} have been used for trajectory clustering.
%and new measures have been proposed specifically the clustering
%problem, such as the \textit{Clue-Aware Trajectory Similarity} (CATS)
%\cite{Hung2015}. \shane{Why not define it and explain it?}
For partition-based clustering, the most appropriate similarity
measure used in the application scenario can vary widely (e.g.,
vehicle \cite{Chan2018,Ferreira2013,Pelekis2009,Hung2015}, soccer
player \cite{Gudmundsson2015}, cellular \cite{Wu2015}, large vessels
\cite{Yao2017}).
Parameterization can also be an important hurdle as well as several
approaches need to optimize multiple parameters in addition to $k$ in
order to produce high quality results.
As an extension of {\kmeans}, which is NP-hard when computing an exact
solution, is partition-based trajectory clustering, which can also be
computationally intractable for large collections when certain
similarity measures are required.
So, often the only solution is to find ways to reduce the number of
trajectories compared through similarity thresholding
\cite{Pelekis2009} or through approximation ratios if an exact
algorithm, which cannot be achieved in polynomial time
\cite{Chan2018}.
%\shane{It is not clear why clustering would yield non-polynomial
%solutions (NP-Hard).
%Clarify?}

One possible approach is to use {\kpath}
clustering~\cite{Wangaclustering}, which is an extension of {\kmeans}
for trajectories on a road network.
The key idea in {\kpath} is to use a quasilinear similarity
measure-\ebd and prune the search space based with an inverted index
and exploit the metric properties of {\ebd}.
As we described in Section~\ref{sec:distance}, {\ebd} computes
similarity by performing a set intersection over edges, which
substantially improves the performance of pairwise similarity
computation, and also maintains comparable precision to common
measures that have a quadratic computational complexity.
Then, an indexing technique based on an edge inverted index and a tree structure for metric similarity measure is used to further reduce the number
of similarity computations in the assignment and refinement phases.
%\shane{what precisely is the new index?}
%\shane{Say more about the solution.
%Put it into proper context of a survey which should not be biased
%towards your own work.
%This is really just dangling here and seems pretty out of place.
%Arguably it could be removed entirely unless the context is more
%clear.}

\subsubsection{Density-based Clustering}
Density-based trajectory clustering first finds dense ``segments'',
and then connects these segments to produce representative routes.
However, the most appropriate approach to identifying dense segments
highly dependent on properties of the data.
\traclus~\cite{Lee2007} is the most cited trajectory clustering
algorithm which solves this problem in two steps, each trajectory is
partitioned into a set of line segments (sub-trajectory), and then,
similar line segments are grouped together into clusters.
A distance threshold $\tau$ is the most common parameter used in
density-based clustering solutions, which specifies the neighborhood
radius.
%\shane{You said "density standard" but
%I have no idea what that means. Is there a formal definition
%of this parameter and density-based clustering that should be
%here?}
%Driven by a human analyst through an interactive visual interface,
%\citet{Andrienko2009} proposed an approach to extract meaningful
%clusters from large databases by combining clustering and
%classification. \shane{Why is this here? Context is unclear.} 

Based on \traclus~\cite{Lee2007}, \citet{Li2010b} proposed an
incremental clustering framework to allow new trajectories to be
added to a database, and a new parameter is further introduced for a new
step-\textit{generating micro-clusters before the final clusters}.
%\shane{Why? What does the new parameter do? What is the secret sauce?}
%\citet{Han2015a} proposed a road-network aware approach for fast and
%effective clustering of trajectories of mobile objects traveling in
%road networks, but with three phases and six parameters. %\shane{And
%this is important why? Context is wrong.}
Similarly, \citet{Agarwal2018} reduced the clustering problem
to finding a frequent path in a graph, which allowed standard
graph traversal techniques to be applied to identify
\textit{pathlets} that could be used to represent each cluster with common sub-trajectories.
{Each cluster's pathlet is defined as a sequence of points that is not necessarily a subsequence of an input trajectory.
	The main difference with \traclus is that the pathlets are the result of optimizing a single objective function to best represent the trajectories, while \traclus generates a set of common segments through density-based clustering, then connects them to form several common paths to represent the trajectories.}
Unfortunately, finding pathlets has been proved to be an NP-hard
problem, so exact solutions are intractable. %\shane{cite?}
%\shane{This paper proved it or another did?}
%Since density-based clustering involves various parameters in
%different work, here we will not give a definition for it.
%\shane{Why? This is not an objective point of view and should
%not be in the survey. There are clearly case where density-based
%clustering is the best approach.}

%, which is similar to \kpath \cite{Wangaclustering}, but not on the road networks
%\sheng{Needs more thinking here.}

\subsection{Trajectory Classification}
For urban data, there are mainly two types of trajectory
classification problems: 1) similarity-based classification
\cite{Lee2008}; 2) transportation modes and
activities classification \cite{Zheng2008,Dabiri2019} which was
reviewed recently by \cite{Zheng2015b}.
%It is worth mentioning that \citet{Bian2019} have reviewed video
%trajectory classification as well recently, where the main
%application is to recognize actions and perform video categorization,
%which is interesting, but not applicable to urban trajectory data.
Next, we will mainly focus on the similarity-based
classification, and also introduce a new classification task for
travel-based inferences~\cite{Nair2019,Chen2019b,Gong2016,Wang2017f}.
%shane{Not clear what you are arguing here. No ground truth? Different ground truths?}

%Verifying the effectiveness of traditional clustering is most
%commonly evaluated using a labeled ground-truth for classification
%problems
\subsubsection{General Similarity-based Classification}
Several studies have investigated trajectory classification problems which
also require extensive similarity computations
\cite{Lee2008,Patel2012, Sharma2010}.
The main distinction in trajectory clustering is that classification
assigns a label to an individual trajectory based on its features,
while clustering is conducted over all items in a dataset.
Specifically, {\citet{Lee2008}} proposed a feature generation
framework for trajectory classification, where two types of
clustering, region-based and trajectory-based \cite{Lee2007}, are
used to generate features for traditional classifiers such as
decision tree or an SVM.
%\shane{which two? what features? more, more, more.}
%\citet{Panagiotakis2009} proposed voting algorithms for trajectory
%classification. \shane{more}
\citet{Sharma2010} proposed a nearest neighbor classification for
trajectory data by computing distance with trajectory sampled and
then choosing the nearest trajectory as the label.
%\citet{Patel2012} considered the duration information of trajectory
%in the classification.% \shane{No idea what this means.}
\citet{AndresFerrero2018} found relevant sub-trajectories
as features for robust classification, where the distance is
computed between two equal-length sub-trajectories.

\subsubsection{Trip Purpose Classification}
Inferring the purpose of a trip has potential applications for 
improving urban planning and governance~\cite{Wang2017f}, but it is
normally conducted by through manual surveys.
With the proliferation of trajectory data availability, trip purposes
can be also classified.
%For transportation mode detection, there are always a fixed number of groups, e.g., bus, train, taxi, private vehicle, and cycling. %including walking, riding a bus, or taking a train.
%\citet{Dabiri2019} proposed to use deep learning for transportation mode classification using trajectories.
\citet{Gong2016} categorized the spatiotemporal characteristics of
nine daily activity types based on inference results, including their
temporal regularities, spatial dynamics, and distributions of trip
lengths and directions.
\citet{Wang2017f} proposed a probabilistic framework for inducing trip
ordering in massive taxi GPS trajectories collections.
The key idea is to augment the origin and destination with neighbor
POIs and identify POI links based on time periods.
Then the trip intents can be explained semantically.
\citet{Nair2019} learned a model to automatically infer the purpose
of a cycling trip using personal data from cyclists, GPS trajectories,
and a variety of built-in and social environment features extracted
from open datasets characterizing the streets.

%\myparagraph{Conclusion} Trajectory clustering and classification has been studied for several years. %however.
%\shane{A summary and conclusion might be good here. It just seems to end.}
%\citet{Chen2019b} further learned a deep embedding approach for profiling taxi trip purposes.
%Unfortunately, no publicly available datasets exist for trajectory
%classification problems as described above. So, while interesting
%and valuable, new work in this area is hampered by this limitation.

%\sheng{\cite{Bian2019} has a review on trajectory classification.}
}

%\shane{It is a little tricky to understand what the takeaway message
%is from this subsection. More thought required in my opinion.}



==> 1-Survey-trajectory 2/package.tex <==
\usepackage{url}
\usepackage[linesnumbered,ruled,vlined,noend]{algorithm2e}
\usepackage{xcolor}
\usepackage{colortbl}
\usepackage{tabularx}
\usepackage{threeparttable}
\usepackage{booktabs}
\usepackage{cellspace}
\usepackage{makecell}
\usepackage{multirow}
\usepackage{natbib}
\usepackage{url}
\usepackage[group-separator={,}]{siunitx}
\usepackage{rotating}
\usepackage{wrapfig}
\usepackage{graphicx,subfigure}
\usepackage{tikz}
\usetikzlibrary{tikzmark}
\usetikzlibrary{decorations.pathreplacing,shapes,snakes}
\usetikzlibrary{arrows}


\iffalse
\usepackage{graphicx}
\usepackage{enumerate}
\usepackage{epstopdf}
\usepackage[normalem]{ulem}
\usepackage{soul}

\usepackage{multirow}
\usepackage{float}

\usepackage{color}
\usepackage{amsmath}
%\usepackage{algorithm}
\usepackage{multirow}
\usepackage{verbatim}
\usepackage{graphicx}

%\usepackage[rm]{caption}
%\DeclareCaptionType{copyrightbox}


\usepackage{xspace}
\usepackage{times}
%\usepackage{enumerate}
\usepackage{shortvrb}
%\usepackage{algpseudocode}
%\usepackage{mathtools}
\usepackage[mathscr]{eucal}
\let\Bbbk\relax         %%redefined in newtxmath.sty
\usepackage{amssymb}
\usepackage{tikz}
%\usetikzlibrary{matrix,decorations.pathreplacing,calc,positioning}
\usepackage{times}

\usepackage{mathtools}

\usepackage{fancyvrb}
%self-defined command

\usepackage{graphicx,subfigure}


\usepackage{epstopdf}

\usepackage{makecell}

%\usepackage{changepage}
%\usepackage{amssymb}% http://ctan.org/pkg/amssymb
%\usepackage{pifont}% http://ctan.org/pkg/pifont
\usepackage{footnote}

\usepackage{titlesec}
\fi


==> 1-Survey-trajectory 2/query.tex <==

\section{Trajectory Similarity Measures}\label{sec:distance}
In this section, we will introduce the widely used trajectory similarity measures.
As shown in Figure~\ref{fig:distance-example},
two different kinds of similarity measures are computed between the query and trajectory separately. \sheng{The float number on each dotted line denotes the distance from a query point to a point in the trajectory.}
\begin{figure}[htp]
	\centering
	\includegraphics[height=2.1cm]{graph/distance-measure1.pdf}
	\caption{Two kinds of similarity measures: (a) a query is a set of points; (b) a query is a trajectory.}
	\label{fig:distance-example}
\end{figure}

\subsection{Points to Trajectory}
To measure the distance between a set of points $Q$ and a trajectory $T$ in the $k$ Best Connected Trajectories search problem (\kbct) \cite{Chen2010a,Qi2015,Tang2011},
each query point  {q} will find the nearest point  {p} in $T$, then all the distances from each query point to their nearest neighbor are aggregated to generate the final distance, i.e.,
\begin{equation}
d_{\svar{kBCT}}(Q,T) = \sum_{q\in Q}{\min_{p\in T} d(q, p)}
\end{equation}

Based on the above equation, $d_{\svar{kBCT}}(Q_1, T_1)=1+1.7+2.2=4.9$ in Figure~\ref{fig:distance-example}(a) is the aggregation of distance between every query point in $Q$ to its nearest neighbor point in $T$ (\sheng{three dotted lines}).
\sheng{When there is only one query point, it is a specific and simple case of \kbct and is also the only supported \knn in \cite{Ding2018,Wang2014e}.}
Since scanning every point in the trajectory returns the nearest point, then the complexity of this measure is quadratic.
Note that this measure only works when the query $Q$ is a set of points, and it does not obey the symmetry rule, i.e., $d(Q,T)\ne d(T,Q)$.
Instead of summing up the distance with the nearest neighbor, another well-known measure called the \textit{closest-pair distance (CPD)} \cite{Zheng2015b} which chooses the minimum distance as the final distance, i.e.,
\begin{equation}
d_{\svar{CPD}}(Q,T) = \min_{q\in Q}{\min_{p\in T} d(q, p)}
\end{equation}
\sheng{
Then $d_{\svar{CPD}}(Q_1, T_1)=1$. Compared with $d_{\svar{kBCT}}$, $d_{\svar{CPD}}$ will be more robust when there is an error point which is far to all the query points in the trajectory.}

\subsection{Trajectory to Trajectory}
Since the query above is a set of discrete points, the order among points in trajectory is not considered when computing the distance. 
However, when we compute the distance between trajectories, the order constraint should be met, i.e., the similarity measure for trajectory should obey the \textit{local time shifting} \cite{Chen2005a}. 

\begin{table}
	\ra{1}
	\centering
	\caption{An overview of existing trajectory-to-trajectory similarity measures.}
	\scalebox{0.9}{\begin{tabular}{cccccccc}
		\toprule\addlinespace[0pt]\rowcolor{gray!30}
		 &    &  & & & \multicolumn{3}{c}{\textbf{Robustness}} \\ \addlinespace[-1pt]\cmidrule{6-8}\addlinespace[-3pt]\rowcolor{gray!30}
		\multirow{-2}{*}{\textbf{Categorization}}      &                     	\multirow{-2}{*}{\textbf{Measures}}                     & \multirow{-2}{*}{\textbf{Complexity}} & \multirow{-2}{*}{\textbf{Metric}} & \multirow{-2}{*}{\textbf{\makecell{Parameter-\\free}}} &  \makecell{GPS \\Error} & \makecell{Sampling\\Rate} & \makecell{Point\\ Shift}   \\ \addlinespace[0pt]\midrule
		\multirow{2}{*}{Curve distance}          & Hausdorff  \cite{Nutanong2011} & $\mathcal{O}(n^2)$ & \xmark &\cmark&\xmark&\xmark &\xmark\\ 	\cmidrule{2-8}
		& Fr\'echet \cite{Eiter1994} & $\mathcal{O}(n^2)$  & \xmark&\cmark &\xmark&\xmark &\xmark \\\midrule				
		\multirow{2}{*}{Real distance}           &     {dtw} \cite{yi1998efficient}      & $\mathcal{O}(n^2)$ & \xmark&\cmark&\xmark&\xmark &\xmark\\ \cmidrule{2-8}
		&   {erp} \cite{Chen2004}      & $\mathcal{O}(n^2)$  & \cmark&\xmark &\xmark&\xmark &\xmark\\ \midrule
		\multirow{2}{*}{Edit distance}           &   {edr} \cite{Chen2005a}  & $\mathcal{O}(n^2)$  & \xmark &\xmark &\cmark&\xmark &\xmark\\ \cmidrule{2-8}
		&   {lcss} \cite{vlachos2002discovering}  & $\mathcal{O}(n^2)$  & \xmark&\xmark &\cmark&\xmark &\xmark  \\   \bottomrule
	\end{tabular}}
	\label{tab:distancemeasures}
\end{table}

%\bao{1) Flat description of each measure, 2) no example on the pros and cons of each class of measure. 3) need to distinguish them well in your table 2.2.}
Several similarity measures have been proposed for trajectory data
in recent years.
As shown in Table~\ref{tab:distancemeasures}, we broadly divide the widely used six similarity measures into three kinds: curve-based, real-distance, and edit-distance.
We will elaborate each measure with the formal definitions and Figure~\ref{fig:distance-example}(b).
As a trajectory can also be viewed as a \textit{geometric curve}, Hausdorff distance~\cite{Nutanong2011,Roh2011} measures
how far two subsets of a metric space are from each other by choosing the max-min distance, without considering the order constraint.

\begin{equation}
\label{equ:hau}
d_{\tvar{Hau}}(Q,T)=\max_{p\in T}{\min_{\ q\in Q}  {eucdis}}
\end{equation}

Fr\'echet distance~{\cite{Eiter1994,Agarwal2014}} extends the Hausdorff
distance to account for location and ordering of the points along the
curves, as shown in Equation~\ref{equ:fre}, where $p$ and $q$ are the head (first) point of $T$ and $Q$, respectively, and $T_h$ and $Q_h$ are the sub-trajectory excluding the head $p$ and $q$.
\sheng{
Taking Figure~\ref{fig:distance-example}(b) as an example, $d_{\tvar{Hau}}$ and $d_{\tvar{Fre}}$ will return the same value $3.1$, as the matching shown in the figure not only finds the nearest neighbor for each point, but also obeys the local time shifting (order constraint).
If any two points in $T_5$ swap the location, $d_{\tvar{Hau}}$ does not change, while $d_{\tvar{Fre}}$ will change as the order is broken.}

As a trajectory can be also viewed as a time series, many similarity
measures originally designed for time series search can be deployed in
trajectory top-$k$ search~{\cite{Zheng2015b}}, such as Dynamic
Time Warping (\dtw) \cite{yi1998efficient}, Longest Common
Subsequence (\lcss) \cite{vlachos2002discovering,Morse2007}, and Edit
Distance on Real sequence (\edr) \cite{Chen2005a} and Edit distance with Real Penalty {(\erp)}~\cite{Chen2004}.
\sheng{\dtw computes the distance based on the sum of minimum distances, instead of choosing the maximum in Fr\'echet distance.}
Equation \ref{equ:dtw} shows the formal definitions of \dtw.
Figure~\ref{fig:distance-example}(b) shows the distance computation using 
\dtw, where every point in $T_5$ and $Q_3$ is matched with each other and will contribute to minimizing the final aggregated distance without breaking the order constraint, i.e., $d_{\tvar{DTW}}(Q_3,T_5)=1.2+3+1+2.2+3.1=10.5$.
\sheng{Note that \dtw has a parameter sometimes when it considers the window constraint $r$ on the matching points' order, e.g., $|o(p)-o(q)|\le w$, where $o(p)$ denotes the order of $p$ in $T$. The window parameter $w$ is widely used in time series data. However, there is always no such constraint on trajectory data.}

\begin{equation}\small
\label{equ:fre}
d_{\tvar{Fre}}(Q,T)=\begin{cases}0,\ \text{if}\ Q=\emptyset\ and\ T=\emptyset\\
\infty,\ \text{if}\ Q=\emptyset\ or\ T=\emptyset\\
\max\{d(q, p), \min\{d_{\tvar{Fre}}(Q_h,T_h),\ d_{\tvar{Fre}}(Q, T_h), d_{\tvar{Fre}}(Q_h, T)\}\},\ \text{otherwise}
\end{cases}
\end{equation}

\begin{equation}\small
\label{equ:dtw}
d_{\tvar{DTW}}(Q,T)=\begin{cases}0,\ \text{if}\ Q=\emptyset\ and \ T=\emptyset\\
\infty,\ \text{if}\ Q=\emptyset\ or\ T=\emptyset\\
d(q, p)+\min\{d_{\tvar{DTW}}(Q_h,T_h),\ d_{ \tvar{DTW}}(Q, T_h),\ d_{\tvar{DTW}}(Q_h, T)\},\ \text{otherwise}
\end{cases}
\end{equation}

%
%, while no vehicle trajectory data is used.
%As a trajectory can also be viewed as a \textit{geometric curve},
%similarity measures between curves can also be used for trajectory
%similarity search~{\cite{Xie2017a}}.

Instead of computing the real distance, computing the edit distance (0 or 1) is more robust to the GPS error as two far points will lead to a big distance if using \dtw.
To judge whether two points are matched, edit-distance based measures need to set a range threshold $\tau$, as shown in Equation~\ref{equ:match}, where $||$ denotes $L1$ norm, and $p_x$ and $p_y$ denote the latitude and longitude of point $p$, respectively.
Then we can define \lcss and \edr as shown in Equation~\ref{equ:lcss} and \ref{equ:edr}.
The basic difference between \lcss and \edr is that \lcss is defined to measure how similar two trajectories are, while \edr is for measuring how different two trajectories are.
\sheng{
For example, if we set $\tau=0.5$ in Figure~\ref{fig:distance-example}(b), then there is no matched point, $d_{\scriptscriptstyle \tvar{LCSS}}(Q_3,T_5)=0$ and $d_{\scriptscriptstyle \tvar{EDR}}(Q_3,T_5)=4$; if we set $\tau=5$, then every point can be matched, and $d_{\scriptscriptstyle \tvar{LCSS}}(Q_3,T_5)=4$ and $d_{\scriptscriptstyle \tvar{EDR}}(Q_3,T_5)=0$. Hence, these two measures highly depends on the parameter $\tau$.}
\begin{equation}
\label{equ:match}
\var{match}(p, q)=\begin{cases}\var{true},\ \text{if}\ |p_x- q_x|\le\tau\ \text{and}\ |p_y-q_y|\le\tau\\
\var{false},\ \text{otherwise}
\end{cases}
\end{equation}

\begin{equation}\small
\label{equ:lcss}
d_{\scriptscriptstyle \tvar{LCSS}}(Q,T)=\begin{cases}0,\ \text{if}\ Q=\emptyset\ \text{or}\ T=\emptyset\\
1+d_{\scriptscriptstyle \tvar{LCSS}}(Q_h, T_h),\ \text{if}\ \var{match}(p,q)=\var{true}\\
\max\{d_{\scriptscriptstyle \tvar{LCSS}}(Q, T_h),\  d_{\scriptscriptstyle \tvar{LCSS}}(Q_h, T)\},\ \text{otherwise}
\end{cases}
\end{equation}

\begin{flalign}\small
\label{equ:edr}
d_{\scriptscriptstyle \tvar{EDR}}(Q,T)=\begin{cases}
|Q|,\ \text{if}\ T=\emptyset \\
|T|,\ \text{if}\ Q=\emptyset \\
\min\{d_{\scriptscriptstyle \tvar{EDR}}(Q_h,T_h), d_{\scriptscriptstyle \tvar{EDR}}(Q, T_h)+1,\ d_{\scriptscriptstyle \tvar{EDR}}(Q_h, T)+1\},\ \text{if}\ \var{match}(p,q)=\var{false} \\
\min\{1+d_{\scriptscriptstyle \tvar{EDR}}(Q_h,T_h), d_{\scriptscriptstyle \tvar{EDR}}(Q, T_h)+1,\ d_{\scriptscriptstyle \tvar{EDR}}(Q_h, T)+1\},\ \text{otherwise}
\end{cases}
\end{flalign}


As they do not obey the triangle inequality which is an essential requirement in the \textit{Metric} space pruning, all the existing measures are \textit{non-metric} except for {\erp}.
\citet{Chen2004} defined a metric trajectory similarity measure, as shown in Equation \ref{equ:erp}, where
point $g$ can be any constant point in the space, it is always set as the origin, i.e., $g=\{0,0\}$.
However, $g$ is also a parameter, the changes will also lead to the change of distance value similar to \lcss and \edr, and further affect the results of \knn search.
Hence, a parameter-free measure is essential for trajectory search.

\begin{flalign}\small
\label{equ:erp}
d_{\scriptscriptstyle \tvar{ERP}}(Q,T)=\begin{cases}\sum_{p\in T}d(g, p),\ \text{if}\ Q=\emptyset\\
\sum_{q\in Q}d(q, g),\ \text{if}\ T=\emptyset\\
\min\{d_{\scriptscriptstyle \tvar{ERP}}(Q_h,T_h)+d(q, p),d_{\scriptscriptstyle \tvar{ERP}}(Q, T_h)+d(g, p),d_{\scriptscriptstyle \tvar{ERP}}(Q_h, T)+d(q, g)\},\ \text{otherwise}
\end{cases}
\end{flalign}



%\sheng{The scenarios, there is not }
\subsection{Complexity and Robustness}
Table~\ref{tab:distancemeasures} compares characteristics of six similarity measures in four-fold: complexity, metric, parameter, and robustness.
\sheng{Since the parameter can be easily observed from their definitions, we will elaborate the other three characteristics next.}

\myparagraph{Complexity}These similarity measures were designed to make search more robust
against local time shifting.
However, existing similarity measures always try to find the best matching
point without breaking order constraints, thus requiring dynamic
programming solutions with a quadratic complexity ($\mathcal{O}(n^2)$).
%New measures such as {\small $\textsf{EDwP}$} \cite{ranu2015indexing} were proposed to reduce the complexity and maintain precision.
Learning an embedding for a trajectory \cite{Li2018a,Yao2017} to compute the Euclidean distance based on vectors with fixed length is promising as it achieves linear ($\mathcal{O}(n)$) computation, but requires long training time for the learning models.
%However, {\erp} has a complexity of $\mathcal{O}(n^2)$ despite being
%metric, and is therefore not useful for problems such as {\kpath} 
%in large collections.

%Effectiveness evaluation of these similarity measures over
%time series data~{\cite{UCRArchive}} was performed by
%{\citet{Wang2013b}}.
\myparagraph{Metric}\sheng{Being metric or not is crucial for a similarity measure, as obeying the triangle inequality is a fundamental feature for reducing distance computation. Here, we use an example to illustrate how to avoid distance computation for a metric similarity measure-Euclidean distance.
In Figure~\ref{fig:triangle}, a query point $q$ is searching the nearest neighbor, $p_1$ and $p_2$ are the two points to be scanned next, and we just computed $d(q,p_1)$. Before conducting distance computation with $p_2$, we can estimate the lower and upper bound of $d(q,p_2)$ based on $d(q,p_1)$ and $d(p_1, p_2)$, where $d(p_1, p_2)$ can be computed off-line for any query.
With the lower bound, we can compare it with $d(q, p^{'})$ where $p^{'}$ is the current founded nearest neighbor. If the lower bound is bigger, we can discard $p_2$ directly as it cannot beat $p^{'}$ to be the nearest neighbor.}
\begin{figure}[htp]
	\centering
	\includegraphics[height=2.5cm]{graph/metric.pdf}
	\caption{Using triangle inequality to estimate the bounds.}
	\label{fig:triangle}
\end{figure}

\myparagraph{Robustness}Besides the high complexity and metric,
most similarity measures are sensitive to noise, sampling rate, and point shift (points are shifted on the path where the trajectory lies). In other words, the existence of noise (due to GPS errors), more (less) sampled points or point shift on a trajectory will make it be judged as dissimilar to the original trajectory using the existing measures in Table~\ref{tab:distancemeasures}.
\sheng{\citet{Wang2013a} also conducted an effectiveness evaluation on the robustness of these six measures over a real-world trajectory dataset.
	
Here, we use an example in Figure~\ref{fig:robustness} to illustrate why they are not robust, where $T_1$ and $T_2$ are two similar vehicle trajectories in the road network as they crossed the same path. After sampling, we will use a set of points to denote them, the ideal sampling (b) will record the same number of points which are also pair-wise close. Nevertheless, in the real case, the sampling rate and time are various, e.g., the point shift (c) will sample the same number of points in the road, but not pair-wise close. The GPS error (d) will sample points that are not in the road, and the inconsistent sampling rate (d) will lead to a different number of points for two similar trajectories. Each of the above three factors will lead to a distance value bigger than that of the ideal sampling using existing similarity measure. 
However, a robust similarity measure should always return the same value if such cases occur, and we find that existing similarity measures are not robust to the point shift, error, and sampling.}


\subsection{Metric learning}
\cite{Yao2017,Li2018a} learns same length vector, and further use the Euclidean distance.



%We further show the complexity.

\begin{figure}
	\centering
	\includegraphics[height=4cm]{graph/robustness.pdf}
	\caption{A similarity measure is sensitive to the point shift, error, and sampling rate.}
	\label{fig:robustness}
\end{figure}


\subsection{Research Gaps}
\sheng{
	Even though the trajectory similarity measure is under-explored in the past two decades, there is still no such a robust measure with low complexity to our best knowledge. Specifically, the research gaps are two-fold:
	\begin{itemize}
		\item An effective similarity measure needs to be robust to the GPS error, point shift, and sampling rate, and should also be parameter-free. However, there is no such a measure as we concluded in Table~\ref{tab:distancemeasures}.
		%Moreover, evaluating the effectiveness toward robustness for the similarity search is another gap.
		
		\item The complexity of existing measures is quadratic, and most of them are non-metric. When we need to conduct \knn search over a vital amount of data, it is unscalable in two-fold: 1) point-wise computation is expensive; 2) distance computation pruning by triangle inequality cannot be applied.
	\end{itemize}
}

%\subsection{Beyond Pre-processing: Trajectory Search}
%Pre-processing over trajectories mainly serve for the effective analytics.
\section{Spatial-Only Trajectory Search}
%As one of the most important data discovery tools, query over the trajectory can help select the most relevant data instead of digesting all the dataset for a specific application.
%As we can see, existing work on trajectory pre-processing deal all the data with a same representation-points for the generality of point data management.
%However, for different trajectory data, the modeling method highly depends on the data type and applications.

%To explain the difference of these queries clearly, we will use an exemplar figure.

%Note that trajectory is composed by points, so we also cover the related work on point data search.
%In the next two sections, we will elaborate the queries over spatial-only and spatial-textual trajectory data, respectively.
\begin{table}
	\centering
	\ra{1}
	\caption{{An overview of existing queries over trajectory data.}} 
	\begin{comment}
	%IR: Information Retrieval \cite{Broder2003}, 
	$k$NN: $k$ 
	Nearest Neighbour \cite{Guttman1984},
	TkSK: Top-k Spatial Keyword Query~\cite{chen2013spatial}, 
	ANN: Aggregate Nearest Neighbour Query~\cite{Papadias2005},
	ATNN: Aggregate Textual Nearest Neighbour Query~\cite{Li2010,Yao2016},
	kBCT: k Best-Connected-Trajectory Query~\cite{Chen2010a}, 
	TkSTT: Top-$k$ Spatial-Textual Trajectory Query~\cite{Wang2017,Shang2012a}.
	\end{comment}
	\label{tab:methods}
	\scalebox{0.9}{\begin{tabular}{ccccccc}
			\toprule\addlinespace[0pt]\rowcolor{gray!30}
			\textbf{Data}&\textbf{Type}&\textbf{Query} & \textbf{Input} & \textbf{Output} & \textbf{Measure}&  \textbf{Index} \\\addlinespace[-2pt]
			\midrule
			&\multirow{2}{*}{Boolean}& Range \cite{SanduPopa2011,Krogh2016} & range & trajectories& N/A & R-tree \\
			\cmidrule{3-7}
			&& Path \cite{Krogh2016,Koide2015} & path & trajectories& N/A & R-tree \\
			\cmidrule{2-7}
			&\multirow{4}{*}{$k$NN}&\knn~\cite{Guttman1984,beckmann1990r,Sellis1987} & point & points & Euclidean & R-tree  \\
			\cmidrule{3-7}
			&&$k$NNT \cite{vlachos2002discovering,Chen2005a}& trajectory & trajectories& LCSS, DTW & R-tree \\
			\cmidrule{3-7}
			&&\kbct \cite{Chen2010a,Tang2011}& points & trajectories& Aggregate & R-tree \\
			\cmidrule{3-7}
			{\makecell{Spatial\\-only}}&&\ann \cite{Papadias2005,Yiu2005}& points & points & Aggregate & R-tree \\
			\cmidrule{2-7}
			& \multirow{2}{*}{\makecell{Reverse\\ $k$NN}} & \rknn \cite{Tao2004,Chan2008}& \makecell{point} & points& Euclidean & R-tree \\
			\cmidrule{3-7}
			& & R-PNN \cite{Shang2011}& \makecell{point} & trajectories & Euclidean & N/A \\
			\cmidrule{2-7}
			& \multirow{2}{*}{Clustering} & Density-based \cite{Lee2007}& \makecell{thresholds} & paths& N/A & N/A \\
			\cmidrule{3-7}
			& & Partition-based \cite{Chan2018}& \makecell{$k$} & trajectory& Hausdorff & N/A \\
			\midrule
			& &KS \cite{Broder2003,Ding2011a,Daoud2016} & keywords & points & TF-IDF & Inverted list \\
			\cmidrule{3-7}
			%IR \cite{Zobel2006} & keywords & points & TF-IDF & Inverted list \\
			%\hline
			\multirow{4}{*}{\makecell{Spatial\\-textual}}& \multirow{4}{*}{Top-$k$} &\tksk \cite{zhang2014processing,Li2011} & \begin{tabular}{c}point, \\ keywords\end{tabular} & points & Aggregate & IR-tree \\
			\cmidrule{3-7}
			& &\atnn \cite{Li2010,Yao2016}& \begin{tabular}{c}points, \\ keywords\end{tabular} & points & Aggregate& IR-tree\\
			\cmidrule{3-7}
			& &\tkstt \cite{Shang2012a,Zheng2013c}& \begin{tabular}{c}points, \\ keywords\end{tabular} & trajectories &  Aggregate & \begin{tabular}{c}Grid-index, \\ Inverted list\end{tabular} \\
			\bottomrule
			%$\dddot{Q}_{n}^m$
	\end{tabular}}
\end{table}

Figure~\ref{fig:queries} shows three exemplary queries $Q_1$, $Q_2$, $Q_3$ for spatial-only trajectories $T_1$ to $T_6$.
Given three points ($q_1$, $q_2$, $q_3$), $Q_1$ finds the best connected trajectory. Among all six trajectories, $T_1$ and $T_2$ are both possible final results. A similarity measure needs to be defined to distinguish which trajectory is closer to $Q_1$.
Given a range (red box), $Q_2$ finds all the trajectories crossing in it, then $T_3$ and $T_4$ will be returned, it is much simple than $Q_1$ as no similarity measure is needed.
Given a trajectory $Q_3$, it will search the most similar trajectories. Similar to $Q_1$, a similarity measure needs to be defined, while it is between two trajectories rather than points and trajectories.

\begin{figure}[h]
	\centering
	\includegraphics[height=5.5cm]{graph/spatial-only-queries.pdf}
	\caption{Three kinds of spatial-only trajectory queries.}
	\label{fig:queries}
\end{figure}

Table~\ref{tab:methods} concludes different kinds of common queries on trajectory data in terms of four aspects: input, output, similarity measure, and index. The column for ``Index" only lists the representative index structure, we will further elaborate in the following sections.
The queries range from basic trajectory search, top-$k$ trajectory similarity search (spatial-only and spatial-textual), reverse $k$ nearest neighbors search, and trajectory clustering.
Next, we will elaborate on each query, and introduce the common indexing structures used for accelerating the performance.
\subsection{Query Types}
\subsubsection{Basic Trajectory Search}
A basic trajectory search includes three main types of queries.
The first one is a {\em Range Query}
( {rq})~{\cite{SanduPopa2011,Krogh2016,Song2014,Roh2011}} that
finds all (sub-)trajectories located in a spatial region or a temporal region.
The range query has many applications in traffic monitoring, e.g., return all the vehicles in a road intersection.
The second is a {\em Path Query} ( {pq}) which retrieves the
trajectories that contain any edge of the given path query.
%, or more generally, any trajectory that contains an edge of the query can be a result.
The third is a {\em Strict Path Query}
( {spq})~{\cite{Krogh2016,Koide2015,SanduPopa2011,kim2008path}}
which finds all trajectories that strictly follow the entire path from
beginning to end. %\shane{detours? can we be more precise?}
Interestingly, the path query and strict path query
share many commonalities with disjunctive (OR) and conjunctive (AND)
Boolean queries~{\cite{Christopher2009}}. 
The main difference is that an SPQ is order-sensitive.

%Keywords can be a query constraint when the target is the activity trajectory, coupled with the range query, it can further shrink the searched results, e.g., finding all the Mexican restaurants in the CBD.

\subsubsection{$k$ Nearest Neighbors Query}
%Top-k trajectory search is a very broad area, so we first review the top-k spatial-only trajectory search.

\myparagraph{Search by Trajectory}
{Given a query trajectory $Q$, the $k$ Nearest Neighbor Trajectories Query aims to search the $k$ most similar/nearest trajectories to $Q$, based on a given trajectory similarity measure.
Such a query can be used to find the most similar trips for traffic flow analysis.}
For the special case when the trajectory is a single point, which is also known as \knn search (we use \textit{kNNT} to denote trajectory search), where the Euclidean distance between two points is utilized.
%However, the distance measure between two trajectories is more complex than points as trajectories can have different number of points.
%There are more than $10$ distance measures for trajectory data, and choosing the right distance measure for the dataset is essential.

\myparagraph{Search by Points}
There have also been various work
targeting search on spatial-only trajectory data using 
a set of points as the input query~\cite{Chen2010a,Tang2011,Qi2015,Yan2014,Qi2016}.
%Edit Distance on Real sequences (EDR)~{\cite{chen2005robust}}, Edit distance with Real Penalty (ERP)~{\cite{chen2004marriage}}, Longest Common Subsequences (LCSS)~{\cite{vlachos2002discovering}},
%and Dynamic Time Warping (DTW)~{\cite{yi1998efficient}}. 
%Despite various similarity metrics adopted for various purposes/scenarios, the commonality among these work is that the trajectory distance is computed as an aggregation of point-to-point distances.
\citet{Chen2010a} initially formulated the problem of
querying over a set of points with spatial-only trajectories.
They proposed an incremental expansion method which used an R-tree for
pruning and referred to the search algorithm as {\em Incremental K Nearest
	Neighbors (IKNN)}.

\citet{Tang2011} proposed a qualifier expectation measure
that ranks partial-matching candidate trajectories to accelerate
query processing for non-uniform trajectory distributions and/or
outlier query locations.
\citet{Qi2015,Qi2016} went on to combine {\em
	IKNN} and the qualifier expectation model to improve the efficiency,
and presented a range-based method to improve the efficiency
even further.
By extending a point-wise similarity measure, {\citet{Yan2014}}
assigned an {\em importance value} to each point based on a timestamp to distinguish between points where a user spends more
time within a trajectory.
Given a set of points, \citet{Papadias2005} searched $k$ Nearest 
Neighbor points in term of the aggregate distance of each neighbor to query points, 
and with an \textit{Aggregate Nearest Neighbor} (\ann) search.


\subsubsection{Reverse $k$ Nearest Neighbor Query}
\label{sec:rnns}
\myparagraph{Search over Trajectories}
Different from finding the most similar or nearest trajectories, the reverse $k$ nearest neighbors query will find the trajectory who will take the query as the nearest neighbor.
Formally, 
given a moving object dataset
$\mathcal{D}$ and a candidate point set $Q=\left( o_1,o_2,...,o_m \right)$ as a
query, \citet{Shang2011} aimed to find the optimal point from
$\mathcal{D}$ such that the number of moving objects that choose $o_i$ as the
nearest neighbor is maximized.
Specifically, they proposed a {\em Reverse Path Nearest Neighbor}
(R-PNN) search to find the nearest point {in $\mathcal{D}$ for the trajectory of a moving object, and returned the 
point in $\mathcal{D}$ that is the nearest point for the maximal number of 
	trajectories of moving objects.}
%Shang et al. introduced the concept of {\em influence-factor} to determine the
%optimal point.
%The influence-factor of $o$ is $f$ if $o$ is the nearest neighbor of
%$f$ trajectories for all candidate points in $O$.
%\revione{Given two sets of trajectories and a threshold $\theta$, \textit{trajectory similarity join} \cite{Shang2017} returns all pairs of trajectories from the two sets with similarity above $\theta$, which can be extended to answer our query when $k=1$, by checking whether the query trajectory lies in the result set of each trajectory. While it does not work with arbitrary $k$ as the result set may contain less than $k$ trajectories.}

\citet{Cheema2012} proposed a \textit{continuous
	reverse nearest neighbors} query to monitor a moving object and find
all static points that take the moving object as one of the $k$ nearest
neighbors.
Recently, \citet{Emrich2014} proposed a solution for
the problem of \rknn search with ``uncertain'' moving object
trajectories using a Markov model approach.
A moving object is treated as a result when it always takes the query
object as the nearest neighbor within a given time interval.
All of these approaches target a single point rather than a
commuter trajectory of multiple-points, which is the focus of our work.

\begin{figure}
	\centering
	\includegraphics[height=3.5cm]{graph/TPL.pdf}
	\caption{Half-space pruning used in {\rknn} for query point $q$.}
	\label{fig:tpl}
\end{figure}

\myparagraph{Search over Points}
Most existing {\rknn} search
work focuses on static point data, and often use pruning-refinement
frameworks to avoid scanning the entire dataset.
However, these approaches cannot easily be translated to route search
where both queries and collections consist of multi-point
trajectories.
%Given a set of candidates as a query, a maximizing {\rknn} query
%finds the optimal point with the maximum number of
%results~{\cite{Zhou2011}}.
Improving search performance has attracted much attention
in previous work.
The basic intuition behind filtering out a point $p$ is to find
another point which is closer to $p$ than the query point $q$
~{\cite{Tao2004,Chan2008,Cheema2011}}.

Here, we review the half space method and use a simple example to
show how pruning works.
Figure~\ref{fig:tpl} shows a query point $q$ and a data point $p$.
As we can see, a perpendicular bisector divides the whole space into
two sub-spaces, and all points inside the lower subspace prefer 
$p$ as the nearest neighbor, such as point $r$.
For the reverse nearest neighbor search, $r$ may be filtered 
from the candidate set of query $q$.
More specifically, $r$ can be filtered out if it can be pruned by at
least $k$ such points.


\iffalse
\subsection{Trajectory Planning}
\label{sec:bnp}

Trajectory query is not limited to searching from a trajectory dataset, but also searching the trajectory from a road network, which is known as the \textit{route planning}.
%Trajectory (route) planning is also an area in robot, our trajectory planning is conducted in road network by default.

\myparagraph{Traditional Transit Route Planning}Bus network design is
known to be a complex, non-linear, non-convex, 
NP-hard problem~{\cite{Chen2014a}}.
Based on existing bus networks, \citet{Shivraj1997}
proposed a heuristic method which uses a genetic algorithm to
minimize the cost of passengers and operators.
Population estimation and user surveys~{\cite{Xian2013}} around the
planned route are traditional ways to estimate the number of
passengers that may use the planned travel route, such as
\textit{Journey to Work}\footnote{\url{https://en.wikipedia.org/wiki/Journey_to_work}}
which is data collected as part of a census that describes aspects of
commuting behavior.
However, the data is usually out-of-date, and may not reflect current travel
patterns.

{\myparagraph{Data-driven Transit Network Planning}A general
	approach to \textit{transit network design} is to use {\em demand}
	data from passengers in addition to {\em supply} data from existing
	routes~{\cite{Guihaire2008}}.
	Supply and demand data is usually abstracted as origin-destination
	(OD) pairs, and can be used to identify the most profitable routes.
	With the proliferation of GPS devices on mobile phones and vehicles,
	demand data can be collected via multiple channels in real time, and
	several previous studies have exploited such data.}

By mining taxi data, \citet{Chen2014a} tried to
approximate night time bus route planning by first clustering all
points in taxi trajectories to determine ``hot spots'' which could be
bus stops, and then created bus routes based on the connectivity
between two stops.
Similarly, based on human mobility patterns extracted from taxi data
and smart card data, \citet{Liu2016} proposed a localized
transportation choice model, which predicts travel demand for
different bus routes by taking into account both bus and taxi routes.

{\citet{Toole2015162} used census records and
	mobile phone location information to estimate demand in
	transit routes.
	Historical traffic data~\cite{6878453}, smart cards~\cite{Zhang2017},
	sensors~\cite{Lv2014}, and cellular data~\cite{Pinelli2016} can
	provide more comprehensive demand data and be used to further improve
	data-driven transit network design.
	Most of these studies employ data mining methods, which scan the
	static and historical records for all the customers.
	In contrast, {\rknnt}-based approaches can efficiently maintain
	up-to-date results whenever there is an update on the trajectory
	data; moreover, \rknnt~query can be answered efficiently which is
	critical to real-time decision making.
	In other words, {\rknnt} augments the existing data-driven methods
	for transit network design.}

\myparagraph{Optimal Route Searching}Given a starting vertex and an
ending vertex, the classical problem is to find the
shortest path in a graph.
\textit{Best-first Search} (BFS) and \textit{Depth-first Search}
(DFS) are two commonly used algorithms for this problem.
An extension of this problem is {\em $k$ Shortest Path searching}
($k$SP) ~{\cite{Yen1971,Aljazzar2011}}, which aims to find the $k$
shortest paths from a start vertex $s$ to a target vertex $t$ in a
directed weighted graph $G$.
Yen's algorithm~{\cite{Yen1971}} is a derivative algorithm for
ranking the $k$ shortest paths between a pair of nodes.
The algorithm always searches the shortest paths in a tree containing
the $k$ shortest loop free paths.
The shortest one is obtained first, and the second shortest path is
explored based on the previous paths.
The {\em Constraint Shortest Path} (CSP) problem
{\cite{Lozano2013,Bolivar2014,Wang2016d}} applies resource
constraints on each edge, and solves the shortest path problem
based on these constraints.
An example constraint in this scenario is the time cost.
\fi


\subsection{Spatial Indexing Structures}
\label{sec:spatialindexing}
Trajectory indexing is proposed for efficient search; it organizes the trajectory data in advance, and can avoid scanning every trajectory until returning the result.
Existing trajectory indexing employs two components: indexing points, and mapping tables.
%R-tree \cite{Guttman1984} is one of the most popular index structures for efficient spatial searching.

\myparagraph{Indexing Points}
To achieve scalable efficiency, a space-efficient index
representation and processing framework are crucial, but existing
indexes for trajectory
search~\cite{Vlachos2003,Pfoser2000,ranu2015indexing} rely on an
R-tree~{\cite{Guttman1984}}, which stores all points from the raw
trajectories.
As shown in Figure~\ref{fig:R-tree-indexing}, trajectories are decomposed to points first, then R-tree is used to index all the points, and the mapping table links the point to its belonging trajectory.
It should be noted that trajectory datasets like \texttt{T-drive}~{\cite{Yuan2010}} can have millions of points, and an R-tree has to manage a massive number of maximum
bounding rectangles ( {mbr}), which is not space efficient in practice.
\sheng{
It often requires a prodigious amount of space in order to
accelerate search, and the pruning method originally devised for
point search is not effective for trajectory search as many of the
similarity measures are
non-metric\footnote{\url{https://en.wikipedia.org/wiki/Metric_(mathematics)}}.}
A simple Grid-index can be a more useful index structure in such
scenarios~{\cite{Zheng2013c}}.
%Z-curve and Hilbert curve further enable a simple accessing in Grid-index instead of traversing in a tree.

Rather than storing all the points, a moving object index can be built over the points.
\citet{Pfoser2000} proposed the TB-tree and STR-tree for trajectory data based on an R-tree.
\citet{G2010} built the R-tree in a special way to obtain coverage functions that are effective for trajectory pruning. Similar moving object index such as TPR-trees \cite{Tao2003,Saltenis2000b}, and MVR-trees \cite{Mokbel2003} have been further proposed based on R-tree.
Note that the moving object index cannot support trajectory search as the similarity measure is limited to the Euclidean distance between points.

\myparagraph{Mapping Table}
A mapping table is used to map points to trajectories \cite{Chen2010a,Zheng2013c}.
After searching for a point, the mapping table will help find the correct trajectory it belongs.
To save space, every point will have a unique identifier ranging from $[1, |\mathcal{D}.P|]$ and every trajectory will have a unique identifier ranging from $[1, |\mathcal{D}|]$, where $|\mathcal{D}.P|$ and $|\mathcal{D}|$ are the number of points and trajectories in the dataset $\mathcal{D}$.
This index is widely used in most trajectory search work on point-based indexes.
Moreover, a table can be built for mapping trajectory to points, i.e., a trajectory is then denoted as a list of point integers.
%A mapping table can be compressed when a point is mapped to multiple trajectories.

\myparagraph{Pruning Mechanism}
%In this section, we mainly investigate the index structure for trajectories, and the pruning methodology.
There are two kinds of index pruning: early termination and early abandoning.
Early termination is used for the threshold algorithm \cite{Fagin2003}.
Given an index, the algorithm gradually scans the sorted lists, and early termination can discard the objects directly based on the upper bound of unseen nodes.
For range query, most of the existing approaches use MBR-based pruning, as
MBR intersection with the query trajectory can be used to prune
out irrelevant trajectories~\cite{Keogh2002}.
By judging whether the minimum distance between the query and the node  {node} of the index is bigger than the distance to the current $k$-th result, 
or whether the node intersects with the query range, a batch of objects can be skipped directly.

For example, the nodes $N_7$ and $N_8$ in Figure~\ref{fig:R-tree-indexing}(a) do not intersect with $N_2$, and can be pruned directly, and we only need to check node $N_9$.
Bounded computations are another method used to accelerate search
\cite{Rakthanmanon2012,vlachos2002discovering}.
This is achieved by estimating the upper bound of the similarity
score and comparing it with the current top-$k$ result set to
determine if the exact distance must be computed.
This approach is often referred to as \textit{early
	abandoning}~\cite{Rakthanmanon2012}.


\begin{figure}
	\centering
	\includegraphics[height=5cm]{graph/spatial-indexing.pdf}
	\caption{Indexing spatial-only trajectories based on R-tree and mapping table.}
	\label{fig:R-tree-indexing}
\end{figure}

\iffalse
\subsection{Research Gaps}
\sheng{
	The research gaps in spatial-only trajectory queries are three-fold:
	\begin{itemize} 
		\item There is no work on reverse $k$ nearest neighbors search over trajectory (\rknnt) which has a promising application on transport capacity estimation as we described in Chapter~\ref{chap-introduction}, where the input data is the users' commuter trajectories and transport routes.
		
		\item There are various kinds of queries over trajectory, while no trajectory system which can support all the common spatial-only trajectory queries.
		
		\item Existing indexing structures are for point-based trajectory, which will suffer from the drawback of high cost from the tree-structured index. There is still no index and pruning algorithm for the mapped trajectory which we intend to manage.
	\end{itemize}
}
\fi

\section{Spatial-Textual Trajectory Search}
%In the top-$k$ trajectory search, defining the distance or similarity measure between the query and trajectory is the first step, and several distance measures have been proposed for various scenarios
Spatial-textual search further supports attaching keywords to a query and trajectory, and the relevant trajectories should not only be close to the query trajectory, but also contains keywords from the query, such as $T_1$ shares the keywords ``\textit{seafood}", ``\textit{coffee}'' and ``\textit{swimming}'' with $Q$, as shown in Figure~\ref{fig:running}. ((a): six trajectories
and the query $Q$; (b): Keywords with
a weight of $T_1$ in each point; (c) Point-wise
matching between $Q$ and $ T_1 $.)

\begin{figure}
	\begin{center}
		\includegraphics[width=0.8\textwidth]{graph/Running.pdf}
		\caption{An example of top-$k$ spatial-textual trajectory search.}
		\label{fig:running} 
	\end{center}
	\vspace{-1em}
\end{figure}



\begin{table*}[!ht]
	\ra{1}
	\centering
	\caption{Comparison between related work on spatial-textual
		trajectory search.}
	\label{tab:com}
	\scalebox{0.9}{\begin{tabular}{cccccccc}
			\toprule\addlinespace[0pt]\rowcolor{gray!30}
			& \multicolumn{2}{c}{\textbf{Input}} &   & \multicolumn{2}{c}{\textbf{Search Metric}} & \\ \addlinespace[-2pt]\cmidrule{2-3} \cmidrule{5-6}\addlinespace[-2pt]\rowcolor{gray!30}
			\multirow{-2}{*}{\textbf{Work}}& Query         & Data Model         &  \multirow{-2}{*}{\textbf{Search Semantic}}        & Spatial      & Textual    & \multirow{-2}{*}{\textbf{Output}} \\\addlinespace[-2pt] \midrule
			{\em \pats-based \tkstt}   &    \makecell{Points with\\keywords}           &         Trajectory    &         Disjunctive &     Eu        &       TF$\cdot$IDF     & \makecell{Top-$k$ \\Trajectories} \\ \midrule
			\citet{Zheng2013c}    &     \makecell{Points with\\keywords}          &     Trajectory       &    Conjunctive      &    Eu          &       N/A    & \makecell{Top-$k$ \\Trajectories}  \\ \midrule
			\citet{Shang2012a}   &        \makecell{Points,\\Keywords}         &      \makecell{Spatial-only \\Trajectory\\ and Keywords}      &    Disjunctive      &       Eu       &       Jac    &  \makecell{Top-$k$ \\Trajectories} \\ \midrule
			\citet{Cong2012}   &        \makecell{Point,\\ Keywords}         &     Trajectory      &       Conjunctive   &       Eu       &      N/A       & \makecell{Top-$k$ sub-\\Trajectories}\\ \midrule
			\citet{Zheng2015}    &        Keywords       &     Trajectory        &    Conjunctive      &      Eu        &      ED      &  \makecell{Top-$k$ sub-\\Trajectories}\\ \midrule
			\citet{HanWZZL15}   &    \makecell{Region,\\ Keywords}           &         Trajectory    &         Conjunctive &      N/A        &       N/A     & Trajectories \\ \bottomrule
	\end{tabular}}
\end{table*}


\subsection{Top-$k$ Spatial-Textual Trajectory Search}
\label{sec:literature-etq}
\myparagraph{Similarity Measures}
Different from spatial-only similarity measures, spatial-textual measures for activity trajectories depend on two parts: spatial and textual.
An aggregated similarity measure is a common solution for spatial-textual points \cite{Cong2009a,Yao2016,zhang2014processing}, i.e., the spatial distance can be normalized as proximity, then coupled with the relevance in the textual dimension with a weight to balance the importance.
Such a measure is also extended by \citet{Shang2012a}, where the spatial-distance is computed in a manner similar to the \textit{$k$ Best Connected Trajectories query} (\kbct).
The textual relevance is computed based on the intersection of all the keywords in the trajectory.
Such a measure is a disjunctive measure, as the textual relevance is computed as a part in the final score, which is more flexible in real applications.
Conversely, a conjunctive measure \cite{Zheng2013c,Cong2012} tightens the constraint and requires that the result trajectory should contain all of the query keywords. So, spatial distance is the main ranking measure.

\myparagraph{Search by Points with Keywords}
Several recent papers have explored the problem of spatial-textual
trajectory search in a variety of different scenarios.
Table~{\ref{tab:com}} reports the differences and similarities
between our work and prior work in terms of query and data models,
search semantics, metrics, and result output, where ``Eu" stands for ``Euclidean", ``Jac"
stands for ``Jaccard" and ``ED" stands for ``Edit Distance".
%Example 2 also shows the direct differences with {\em ETQ}.
From Table~\ref{tab:com}, we can see that the only work which
supports the same input and output as {{\pats}} is the work
of \citet{Zheng2013c}.
However, their work only supports conjunctive matching, so all of the
results must contain every query keyword, which simplifies
the more general keyword search problem.
\citet{Shang2012a} presented a similar search
semantic, but keywords are attached to the whole trajectory,
and not individual locations in the query or the data.

\iffalse

At first glance, our problem can be scoped as a spatial-textual
trajectory search~{\cite{Zheng2013c,
		Cong2012, Zheng2015, Shang2012a}}.
%,zheng2016popularity}}.
%In particular, \citet{Zheng2013Towards} note that solutions to the spatial-only trajectory search cannot be applied to trajectories which should include both textual and spatial measures in the search process. 
%
%Here, we consider two aspects:
%(1) How should the trajectory data and the query be modeled; and (2) What search semantics should be imposed on the textual and spatial components.
%, i.e., the similarity model. Here we discuss the most closely related work only, and will expand the discussion in Section~\ref{sec:literature}.
%Regarding the data modeling, as shown in Example~1, the trajectory data is usually modeled as a set of spatial locations (points) plus a set of keywords specifying user preference (if any).
%by all existing works and also this work.
However, our input query differs from past work.
{\citet{Shang2012a}} modeled queries as distinct
sets of locations and keywords.
Consequently, retrieved trajectories were close to target locations,
but contained no common keyword with each query point since the
keywords were not necessarily constrained to any of the locations.
In contrast, {\citet{Zheng2013c}} used Boolean queries, which
only retrieved exact matches.
Neither of these approaches satisfy the query we wish to ask.
For example, in the work of 
\citet{Shang2012a}, the
trajectory in Figure~\ref{fig:running} which contains ``coffee'' 
in the $4^{th}$ point 
that is faraway from the query point may be recognized as a quite similar 
trajectory as the $2^{nd}$ point is spatially close to the query point, and
for {\citet{Zheng2013c}}, a trajectory without the keyword
``coffee'' would not be a result even if all of the other keywords
are matched.
\fi

Other work~\cite{HanWZZL15,Cong2012,Zheng2015} is quite
different with our work from the perspective of input and search
semantics. 
Briefly, \citet{Cong2012} proposed a sub-trajectory
search method to find the minimum travel distance for a single query
point using a Boolean keyword match.
\citet{Zheng2015} proposed an approximate query solution over
trajectories with a set of keywords.

A special case is when the input only contains the keywords,
which is known as a keyword-only query.
Another special case is when the trajectory data and query only contains a single point, which is known as Top-$k$ Spatial Keyword Search (\tksk).

\myparagraph{Keyword-only Query}
The keyword-only query is also an important tool to explore geo-tagged data. 
For example, people might want to search nearby restaurants by keywords 
``\textit{tacos restaurant}" (in Google Maps) when they go to \textit{Los Angeles}. These are normally resolved in two ways: (1) a textual Boolean query (\textit{conjunctive search}), where the objects
that contain all query keywords are returned as results. However, a textual Boolean query is too strict when a query has multiple keywords.
(2) a Top-$k$ Keyword query (\textit{disjunctive search}) which returns the top-$k$ objects ranked by the similarities of objects w.r.t. the query. Here, we focus on the top-$k$ keyword query. Term-at-a-time (TAAT) and Document-at-a-time (DAAT) 
are two common search paradigms \cite{Broder2003} in the area of information 
retrieval. The inverted list of each term can be used to filter 
out objects that do not contain any keyword in the query. 
In terms of the similarity metrics, TF-IDF \cite{Salton1988}
and Language Model \cite{Song1999} are two widely adopted ones.


\myparagraph{Top-$k$ Spatial Keyword Search}
A Top-$k$ Spatial Keyword~(\tksk) search retrieves the $k$
objects with the highest ranking scores, measured as a combination of
distance to the query location, and relevance of the text
description to the query keywords,  e.g., \textit{``finding 3 restaurants which could serve lobster, pizza or steak and are also close to my hotel"}.

The solution can be broadly divided into two categories:
spatial-first~{\cite{Cong2009a,Li2011}} and
text-first~{\cite{Zhang2013, Rocha2011}}.
A spatial-first strategy augments the nodes of a spatial data
structure like an R-tree with a pseudo-document vector to store the
textual information in each node.
For example, the IR-tree~{\cite{Cong2009a,Li2011}} was
proposed to combine an R-tree with an inverted index.
An upper bound of spatial proximity is calculated from the MBR, and an upper bound of
textual relevance is derived from the pseudo-document for pruning.

A spatial-first strategy will scan a few leaf nodes which
contain many unrelated points that do not share any common keywords at
all, so an IR-tree can be inefficient, especially when $k$ is large~{\cite{Mackenzie}}.
For text-first methods \cite{Rocha2011}, the search
space is primarily organized by keywords, so only the points which
share common keywords with the query will be checked, and the
processing time does not increase as in the IR-tree, even
though $k$ is large.
Recently, {\citet{zhang2014processing}} proposed a novel
solution for top-$k$ spatial keyword query which recasts the
problem to the well-known top-$k$ aggregation problem.
\citet{Li2010} proposed \textit{Aggregate Textual Nearest Neighbor} 
(\atnn) search based on \ann~by adding keywords in the query. The similarity
is an aggregation of the spatial proximity to the query locations and 
textual similarity to the query keywords.

\sheng{
\myparagraph{Boolean Range and Top-$k$ Query}\citet{Hariharan2007} proposed the Boolean range query to finds all the objects that contain the query keywords and locate in a query range.
Boolean Top-$k$ query \cite{Cary2010,DeFelipe2008a} searched all the $k$ nearest objects with conjunctive Boolean constraints on textual content, i.e., contain all the query keywords.
\citet{HanWZZL15} investigated the Boolean range query over trajectories where three important aspects, i.e., spatio, temporal and textual, are all taken into consideration.

To answer each type of query, a special design indexing structure is proposed to find the objects that meet the constraint of the query.
However, most of the existing work can only support a single type of query.
\citet{Hoang-Vu2016} proposed a single and unified Spatio-Temporal Textual Index structure (ST2I) to answer the range and \tksk query with multiple constraint types. The primary motivation is to reduce the storage cost of abundant index and also guarantees high query performance, which is consistent with our motivation for the supporting multiple queries over points and trajectories with a single index, while their work only focused on point data, and cannot answer our trajectory search.
%\citet{Zheng} investigated the interactive spatial keyword search by generating candidate input for user with zero-knowledge.
}


%\begin{comment}
%As we can see, the input query specified in \cite{Zheng2013Towards}
%is the same as the input query for ETQ.
%In their work, trajectories were found which contain all of the
%activities in the query using a top-$k$ minimal matching distance.
%\citet{Cong2012Efficient} take only a single point $q$ with a set of
%activities, and searches for sub-trajectories which contain all of the
%activities using a top-$k$ minimum travelling distances from $q$.
%%Given a region as input, \citet{HanWZZL15} find all trajectories located inside the region which also contain all of the keywords, which is not a top-$k$ problem strictly speaking. 
%\citet{DBLP:conf/edbt/ShangDYXZK12} is the only work which supports disjunctive search, and considers both the textual and spatial similarity.
%The main difference between the approach of
%\citet{DBLP:conf/edbt/ShangDYXZK12} and other work is that the
%input is a set of points and a set of activities, where the
%activities are attached to whole trajectory and not points.
%\citet{ZhengYZXSZ15} solve the approximate search problem over semantic
%trajectories by finding the sub-trajectory which contains the most
%relevant activities with top-$k$ minimum travelling distance.
%So, many different spatial-textual trajectory search problems and
%solutions have been proposed in recent years, but none which exactly
%correspond to the ETQ problem.
%\end{comment}

%\begin{comment}
%%Past work calculates spatial and textual similarity separately before combining them to get the final result~, meaning 
%Each query point
%will find the spatially closest point first in {\cite{DBLP:conf/edbt/ShangDYXZK12}}.
%Consider the example in Figure~{\ref{fig:running}}.
%Here, $Q$ has an equal spatial distance to $T_1$ and $T_2$
%as the $1^{st}$, $2^{nd}$ and $3^{rd}$ point of $T_1$ and $T_2$ are
%the closest points to the $p_3$, $p_1$ and $p_2$ in $Q$.
%However, such two connected points do not have any common keywords, so $T_1$
%should be closer to $Q$ than $T_2$ when the $2^{nd}$, $3^{rd}$,
%$4^{th}$ points of $T_1$ and the $2^{rd}$, $4^{th}$ points of $T_2$
%are selected in our case.
%The other common approach {\cite{Zheng2013Towards, Cong2012Efficient}} is to impose a Boolean conjunctive match
%constraint on the keywords, which would return trajectories which are
%further away than $T_1$ or $T_2$ but never take these highly relevant
%trajectories.
%\end{comment}


\begin{comment}
\centering
\label{tab:distancemeasures-st}
\caption{An overview on existing spatial-textual trajectory similarity measure.}
\begin{tabular}{ccc}
\toprule
\multirow{2}{*}{Spatial-textual} & Conjunctive distance \cite{Zheng2013c,Cong2012,Zheng2015}  & $\mathcal{O}(n^2)$  \\
\cmidrule{2-3}          &           Disjunctive distance \cite{Shang2012a}           & $\mathcal{O}(n^2)$  \\ \bottomrule
\end{tabular}
\end{comment}

\subsection{Textual Indexing Structure}
\sheng{Along with the spatial index, the inverted index \cite{Zobel2006} for text part has been widely used for searching spatial-textual data}.
Composed of all the identifiers of objects that contain a particular keyword, the inverted list can be as simple as indicating the existence of this keyword to serve the Boolean part of the query, or as complex as incorporating the 
weight of the keywords to serve the similarity computation for a top-$k$ spatial-keyword query.
Most work~\cite{zhang2014processing,chen2013spatial} 
proposed to use the inverted lists on top of an existing tree-structured index (say R-tree) to deal with spatial-textual search, which is known as spatial-first. 
Text-first usually employs the inverted index as the top-level index and then arranges the postings in the list in a spatial structure. 
%Textual-first indexes have been shown to be faster than the spatial-first index as it can filter more points earlier in the processing.
%Moreover, 

%Set intersection between inverted lists is a common operator for conjunctive Boolean queries \cite{Culpepper2010}.

\sheng{Since each keyword will have a separate inverted list, the space of an inverted index for a corpus will lead to high cost.
For example, the Second Edition of the 20-volume Oxford English Dictionary contains full entries for \numb{171476} words in current use (and \numb{47156} obsolete words).\footnote{\url{https://wordcounter.io/blog/how-many-words-are-in-the-english-language/}}
Then inverted index compression is a common operation to reduce the storage cost of the inverted index.
The goal of inverted list compression is to store a collection of sorted integers with as few as possible bits (low compression ratio) and support query processing (less decompression time) as fast as possible \cite{Wang2017b}.
Inverted list compression approaches usually follow common wisdom of computing the deltas (a.k.a d-gaps) between two consecutive integers first and then compress the deltas using variable bytes, existing commonly used methods include PforDelta \cite{Zukowski2006}, VByte \cite{Cutting1990}, SIMDPforDelta \cite{Lemire2015}, etc.}
%Compressed inverted index 
%For sorted and unsorted lists, the compression method also varies.


\iffalse
\subsection{Research Gaps}
\sheng{
	There are two gaps in the research on spatial-textual trajectory search:
	\begin{itemize}
		\item 
		As we concluded in Table~\ref{tab:com}, a similarity measure which meets the requirement of ranked, disjunctive, and point-wise search semantics is crucial for \tkstt.
		However, such a similarity measure for top-$k$ spatial-textual trajectory search is still an unsolved research question. 
		
		\item Most existing work focus on single query with single indexing framework, and the only exception is the unified index for point data \cite{Hoang-Vu2016}.
		There is no such a unified index and search paradigm to support various top-$k$ queries over trajectories and POI data.
	\end{itemize}
}
\fi

==> 1-Survey-trajectory 2/response.tex <==

\newcounter{cN}

\newcommand{\weakcomments}[1]{
	\refstepcounter{cN} % incrment counter
	\noindent \hangindent=0em 
	\textbf{\textcolor{maroon}{\underline{Weak Point \thecN}:~}
		\emph{``#1"}	}
}
\newcommand{\comments}[1]{
	\refstepcounter{cN} % incrment counter
	\noindent \hangindent=0em 
	\textbf{\textcolor{red}{\underline{Weak Point \thecN}:~}
		\emph{``#1"}	}
}

\newcommand{\response}[1]{
	\\[0.25em] 
	\hangindent=0.3em \textbf{\textcolor{blue}{\underline{Response}:~}}
	#1
	\vspace{1em} 
}



\setcounter{section}{9}
\renewcommand\thesection{\Roman{section}}
\renewcommand\thesubsection{\thesection.\Roman{subsection}}
\setcounter{figure}{0}
\renewcommand{\thefigure}{\Alph{figure}}
\pagenumbering{roman}

\vspace{2em}
{\centering{\huge\textbf{Response Letter to Reviewer Comments}}\vspace{2em}}

%\twocolumn[]
First of all, we would like to thank the reviewers for the constructive comments that have helped us to improve
our paper titled \emph{``A Survey on Trajectory Data Management, Analytics, and Learning"}.
We have revised our paper accordingly and are re-submitting the
manuscript for further evaluation.
In this response letter, we outline how each concern from the reviewers was
addressed, and describe the changes that we have made to the paper.
To assist the assessment, we have highlighted in the revised manuscript all changes in {\textcolor{blue}{blue color}}, and have cross-referenced each change with a margin note in {\textcolor{red}{red color}}. We have also highlighted several important statements with {{colored underlines}} (blue, green, brown, and red), indicating that these statements have been presented in the original manuscript and might have been overlooked in the first round of review. We have also fixed several small typos and improved the overall presentation. Thank you again for your time and efforts in reviewing our revised manuscript.


%We have also highlighted several important claims with {\textcolor{green}{green-colored underlines}} that have been presented in the original manuscript, in order to indicate that we have mentioned the importance of data distribution and \uni while they might be overlooked in the first round of review. We also fixed several small typos to improve the overall presentation. Thank you for your time and efforts reviewing our revised manuscript.
\setcounter{cN}{0}

\section{Response to Reviewer 1}
\label{sec:r1}
Thanks Reviewer 1 for your endorsement of our work. 
To further improve the quality of this survey, we make several changes according to other reviewers' comments.
It is also worth saying that we noticed there were several new papers published in PVLDB recently (after our submission date), such as \cite{Koide2020} \cite{Wang2020c} \cite{Wang2021}. We added them into the section of similarity measures (Section~\ref{sec:distance}), spatial index (Section~\ref{sec:spatialindexing}), and deep learning (Section~\ref{sec:deep}), respectively.
 
%\bao{R1 mentioned the possibility of elaborating a bit more on the deep learning part. If you have added a bit more details on that, you can include some response on it.}

\setcounter{cN}{0}
\section{Response to Reviewer 2}
\label{sec:r2}
\comments{The trajectory data definition includes only the timestamp in a point and not the data. However, at the description, it is mentioned that each point includes extra data, so I suggest to include the data in the formal definition of a point.}
\response{Thank you. We have added the information about the extra data to the definition.}

\comments{The description of equation 6 needs more details. Actually, the definition is complete but it needs more details to help the reader fully understand the concept.}
\response{Thank you. We have added more descriptive information into the definition.}

\comments{In sections 4.1.2 and 4.1.3, there is a need for at least an introductory sentence. Also, definition 9 requires a more clear description. For instance, what exactly is the query (Q)? - Finally, the authors refer that "the RkNN query include resource allocation, decision support, and profile-based marketing", without any reference.}
\response{Thank you. We have added an introductory sentence in each section. The reference about the applications RkNN are also added. }

\comments{In section 4.2, the description of the Mapping Table is vague; it needs more details.}
\response{Thank you. We have referred Fig.~\ref{fig:R-tree-indexing} and shown an example to have a better description.}

\comments{For the part saying "Distributed Systems for Intensive Similarity Computations" it is more appropriate to replace it with “Map-Reduce for Intensive ....” since the works are based on the map-reduce model, not on distributed systems. Joins are computed using the map-reduce model which can potentially be applied on distributed systems.}
\response{Thanks for pointing it out. We have changed it to be ``MapReduce-based Distributed Systems for Intensive Similarity Computations'', to remove the potential ambiguity.}

%\vspace{-2em}
\setcounter{cN}{0}
\section{Response to Reviewer 3}
\label{sec:r3}
We notice that Reviewer 3 may overlook some important parts of our paper, hence we use four different colors to underline them to address weak points \setulcolor{blue}\ul{1}, \setulcolor{green}\ul{5}, \setulcolor{brown}\ul{6}, and \setulcolor{red}\ul{7}, respectively. 

\comments{The most serious concern I have is the contribution of this survey. As also indicated by the authors, there are several other surveys on trajectory data. It is not clear how the results of these surveys are exploited/upgraded/enhanced in this survey. Or whether this survey just covers more areas for completeness? For potential readers (at least for me), they probably will not feel too excited about this paper. Additionally, the paper does not provide a clear and concise view and motivation.}
\response{
Thanks for the concerns; we understand that a good survey should be novel for readers to overview the state-of-the-art. When we read existing trajectory surveys, we found they were dated as current techniques have advanced significantly in the last three
years, and had a specific focus area such as data mining (detailed comparisons can be found in Section~\ref{sec:new}).

Based on the above observations, we were motivated to write such a survey to provide our readers the latest and complete review.
Reviewer 3 can refer to Section~\ref{sec:new} for our main contributions that distinguish our survey from others. It might be worth highlighting that we do not just cover more areas; instead, we cover the most recent work in a novel way through a pipeline decomposition on trajectory data management, analytics, and learning.
For example, in Table~\ref{tab:applications}, readers can easily link the trajectory pre-processing, similarity measures with upper-level applications.

Compared with other surveys, this survey also broadens the research areas on trajectories, and summarize useful and new resources (e.g., new datasets and commercial systems) than existing trajectory surveys.
Specially, we introduced new cross-disciplinary research on trajectories from computer vision and self-driving.
Most importantly, we point out several open challenges for readers to explore, especially the trajectory applications on public health and self-driving.

Figure~\ref{fig:data-query} has provided a fair and concise overview.
%Please check the underlined part which describes the details.
For the motivation, we added a new paragraph at the beginning of Section~\ref{sec:new} and we hope it can better motivate this survey. %since we are not contributing a new research problem but writing a survey, we think it is more appropriate to use a direct way to deliver what we will cover, just like other trajectory surveys \cite{Zheng2015b,Parent2013a,Richly2018}
%With proper introduction and
%through the comparison with existing surveys and our contributions in Section~\ref{sec:overview}, the motivation of this survey is clear.
For ease of reading and checking, we used \textcolor{blue}{blue} color to highlight several parts that reflect the detailed descriptions of the above summaries. Thank you.

\iffalse
\setulcolor{blue}
\ul{We sincerely hope the reviewer can take another look at the blue outlined text at the introduction; detailed comments are welcomed in future rexvisions.}
\fi
}

\iffalse
\comments{The first part of this article proposes to include some important tutorial materials, such as background knowledge about the research topic, which can better introduce the reader to the topic.}
\response{Sorry, we do not find the points to be revised here.}
\fi

\comments{On page 2, 1(a) (cited from “Social GAN” [78]) is not suitable for expressing the example of traffic surveillance cameras the author wants to express in this article. It is recommended to make some modifications or replace a figure.}
\response{Thanks for this suggestion. We replace a new one from the grand central station dataset \cite{Zhou2012}.}

\comments{The authors label their figures and refer to them in the text with Figure. The authors are invited to use the same wording of the labels in their text.}
\response{Thanks for this suggestion. We have unified all the terms to Fig.}

\comments{ Page 17, line 26-27, revise the sentences :“but not applicable to to urban trajectory data”and “Next, we will will mainly focus on the similarity-based classification”.}
\response{Thanks for pointing it out. We have revised it.}

\comments{The article reviewed several aspects of trajectory data research, but the significance or background knowledge of each sub-topic was not clearly described. Before presenting the technical details of each subtopic, it was not well coherent and introduced.}
\response{To make our survey easy to follow, at the beginning of most sections or sub-sections, we gave short (due to space limit) but proper introductions. For example, in the applications of trajectory, we gave an overview and mentioned the corresponding significance. 
Please kindly note that the text body underlined in \textcolor{green}{green} color is to facilitate the reviewer in checking the associated significance and background (which was in our original submission as well). Thank you.
}
%\setulcolor{green}
%\ul{We sincerely hope the reviewer can take another look at the green outlined text and check the significance and background. We look forwards to seeing detailed concerns on which part does not have the proper background in future revisions, thanks.}


%In the begining of writing this survey, due to space limit, we cannot be too specific. Instead of writing survey by explorate every work, we choose to apply a summarize with an overview. That means we compares the work's problem. For the methodology, we have covered in the previous sections. Trajectory applications are different.

%This paper is an overview survey in my opinion, not a book, and there are too many papers on trajectories. Here I prefer to conclude them in terms of index and methodology using tables, rather than elaborating every paper with details; otherwise, even sixty pages are not enough. Moreover, as we can observe, trajectory research prefers problem novelty and real-world applications, rather than pure techniques part (this is a little different from IR, so DB people usually do not list "research question" in the paper, as our problem itself is new.). Trajectory indexing for this analytic part is very similarly based on the mature spatial index, and the methodology is always filtering and verification. I hope you can understand why I do not mention too much about the techniques, the core part has been covered in the flow charts and tables, and the key indexing techniques are also thoroughly discussed in the first five sections. Thanks very much! Please let me know if you have further concerns.

\comments{The function of the figures and tables should be used to support the author’s point of view. The figures and tables in this article occupy a large space and the content is also detailed, it is conceivable that the authors have spent much effort to do these takes. However, the authors do not have much explanation and analysis of these charts.}
\response{For every figure and table, we have given the proper information in the title and text for readers to interpret. We believe our figures and tables are easy to follow with descriptive texts and indications. We highlight them in \textcolor{brown}{brown}-colored underlines to facilitate the reviewer in walking through them. Thank you.
}	
	
\iffalse	
\setulcolor{brown}
\ul{We sincerely hope the reviewer can take another look at the brown underlines and let us know more details about which figure is not clear in the future revision if possible, thanks.}
\fi

\comments{The article is almost a list of related research on various sub-topics. After reading this survey paper, I don't feel that I have learned anything particularly interesting. It does not provide much new insight or some inspiration for potential readers of related research directions (at least for me).}
\response{
%We covered many sub-topics that are published recently. Firstly, we show a clear taxonomy in various aspects. The most existing part is that we list the datasets. We also form a github repo to list the most important resource.
\iffalse
Before presenting why our survey is not boring, we sincerely suggest that the reviewer read our response to weak point 1 about our novel contributions. If you have checked every part of those contributions, 
you will find that this survey is not a list of sub-topics. 
\fi
We made a thorough taxonomy and concluded at a high-level to avoid abundant descriptions of each recently published work, and we believe this effort is more informative than simply including a list of related research in a flat manner.
%
As a survey that aims to inspire readers to grasp the pain-points and opportunities easily, we provided new insights in every section. 
For example, in the introduction, we listed various datasets from other areas that were always overlooked. We also mentioned that trajectory data could be from various devices rather than just GPS. 
In the second section, we concluded open-source/commercial systems for the first time.
In the third section, we emphasized that the segment-based similarity measure is an emerging topic.
In the fourth section, we summarized the works which are mostly published in the last three years, where no survey has done that.
In the fifth section, we put much effort into the latest research on large-scale trajectory clustering and a new type of classification, trip-purpose classification, which has not been reviewed or discussed in previous survey yet.
In the sixth section, we illustrated four main emerging applications on trajectory data, and we decomposed the common pipeline of each application.
In the seventh section, we reviewed how learning has been applied in various trajectory data analytic stages.
In the eighth section, we pointed out several new applications of trajectories, especially the research on self-driving and public health, and some open problems on building benchmarks and public data repositories.
%
We also highlight the above in \textcolor{red}{red}-colored underlines in each section, to facilitate the reviewer in walking through those insights brought by our work. Thank you.

\iffalse
\setulcolor{red}
\ul{Lastly, we sincerely hope the reviewer can check the red underlines in each section to double-check our new insights. It will be great if the reviewer can give more details on which part is not novel in future revisions, thanks.}
}
\fi


==> 1-Survey-trajectory 2/storage.tex <==
\section{Management Systems and Pre-processing}
%show a table to conclude all the open research trajectory datasets and their main application scenarios, then
To have an intuitive understanding of trajectory data, we first discuss the trajectory representation and available storage systems for trajectory data.
%Then we describe the common techniques on the pre-processing: the cleaning, compression and map-matching.


%For the commuting trajectory, we can take Google map as example, people can set the commuting in the app, and 77\% of smartphone owners regularly use navigation apps.

%\sheng{Show a trajectory figure here}

\subsection{Trajectory Representation and Storage}
A set of coordinates denoted by two floats (e.g., {\small``-37.807302, 144.963242''}) are traditional
representations of trajectories for storage, search, and analytics.
Storing a trajectory as a set of points is the common method in both research and industry.
Table~\ref{tab:systems} shows several research systems for trajectory data and other commercial systems which can store trajectory data as a specific data structure that are currently available.
% while trajectories can have different lengths.
%For example, a trajectory with $n$ points can be stored as $2n$-dimensional vector easily.
%While not all the trajectories have the same length $n$, hence storing various dimensional trajectory data in a table is not scalable.
%To overcome this problem, converting the raw data by learning \cite{Yao2017,Li2018a} or hashing \cite{Sanchez2016} to a vector of the same length can simplify the storing, while it may lose precision for further analytics.
%This is a relatively simple conversion but is often inefficient
%when used for hashing, or training machine learning models.


\iffalse
Recently, storing raw trajectories as a path on a road network using 
\textit{map matching}~\cite{Lou2009} has been shown to be more
effective in terms of storage~\cite{Song2014} and retrieval
performance~\cite{Wangsheng2018}.
The road network is modeled as a directed graph, and each road is an
edge with a unique ID, and a trajectory can be represented as a
sequence of unsorted integers.
More attributes are attached with the trajectory, such as the timestamp, 
keywords in the activity trajectory \cite{Bao2012Location}.
\fi

In the academic field, several trajectory storage systems have been built to manage trajectory data \cite{Cudre-Mauroux2010,Wang2014e,Shang2018,Ding2018,Xie2016a} by storing a trajectory as a set of points.
Moreover, most trajectory management systems \cite{Cudre-Mauroux2010,Wang2014e,Xie2016a} only support trajectory
storage and simple queries such as a range query (finding trajectories in a rectangle).
More recently, distributed systems \cite{Shang2018,Ding2018} have been developed to store the large-scale of point-based trajectory datasets and can perform advanced queries such as $k$NN search over trajectories.

Existing commercial or open-source systems (e.g., a general database such as Oracle Spatial\footnote{\url{https://www.oracle.com/technetwork/database/options/spatialandgraph/overview/index.html}}, SQL Server\footnote{\url{https://docs.microsoft.com/en-us/sql/relational-databases/spatial/spatial-data-sql-server}}, and MySQL\footnote{\url{https://dev.mysql.com/doc/refman/5.7/en/gis-linestring-property-functions.html}},
or the geospatial database such as ArcGIS\footnote{\url{http://www.arcgis.com/index.html}}, Tile38\footnote{\url{https://github.com/tidwall/tile38}}, PostGIS\footnote{\url{https://postgis.net/}}, GeoMesa\footnote{\url{https://www.geomesa.org/}}, Magellan\footnote{\url{https://github.com/harsha2010/magellan}})
can also be extended for trajectory management.
\sheng{For example, {\em LineString} (Figure~\ref{fig:linstring}) defined in a data-interchange format-GeoJSON\footnote{\url{https://en.wikipedia.org/wiki/GeoJSON}} is a geographic data structure for an array of point coordinates, and trajectory can be stored as a {\em LineString}.}
However, the supported operators over LineString are very limited, e.g., returning the number of points, the starting point, the ending point, and the $i$-th point, etc.
The supported range query and \knn are all over points, and not supported for LineString to our best knowledge.

\begin{figure}[htp]
	\centering
	\includegraphics[height=4.5cm]{graph/linestring.pdf}
	\caption{An example of \textit{LineString} with four points in the GeoJSON format \cite{butler2016geojson}.}
	\label{fig:linstring}
\end{figure}

\begin{table}
	\centering
	\caption{An overview of existing/potential systems for trajectories.}
	\begin{tabular}{cccccc}
		\toprule
		\addlinespace[0pt]\rowcolor{gray!30}
		System          &    Data    &    Indexing     & Range  & $k$NN  &         Similarity Measure          \\
		\addlinespace[-1pt]\midrule
		TrajStore \cite{Cudre-Mauroux2010} & Trajectory &    Quad-tree    & \cmark & \xmark &          \xmark          \\
		SharkDB \cite{Wang2014e}                      & Trajectory & Frame structure & \cmark & \cmark &   Point-to-trajectory    \\
		UITraMan \cite{Ding2018}                      & Trajectory &     R-tree      & \cmark & \cmark &   Point-to-trajectory    \\
		DITA \cite{Shang2018}                       & Trajectory &     R-tree      & \cmark & \cmark & Trajectory-to-trajectory \\ \midrule
		Oracle                               & LineString &     R-tree      & \cmark & \cmark &      Point-to-point      \\
		PostGIS                              & LineString &     R-tree      & \cmark & \cmark &      Point-to-point      \\
		SQL Server                             & LineString &   Grid-index    & \cmark & \cmark &      Point-to-point      \\
		GeoMesa                              & LineString &  Z-order curve  & \cmark & \cmark &      Point-to-point      \\
		Tile38                               & LineString &     R-tree      & \cmark & \cmark &      Point-to-point      \\
		Magellan                              & LineString &     \xmark      & \cmark & \xmark &           \xmark           \\
		GeoSpark \cite{Yu2015}                       & LineString &     R-tree      & \cmark & \cmark &      Point-to-point      \\
		SpatialSpark  \cite{You2015a}                   & LineString &     R-tree      & \cmark & \xmark &           \xmark            \\ \bottomrule
	\end{tabular}
	\label{tab:systems}
\end{table}


%we can show the LineString
%Time series database (InfluxDB\footnote{\url{https://github.com/influxdata/influxdb}}) can store a trajectory as a sequence to maintain the timestamps; 
%however, it cannot support any spatial features (e.g., index) and does not support any trajectory-based queries.

\sheng{
SpatialSpark \cite{You2015a} and GeoSpark \cite{Yu2015} are two representative open-source systems from the research filed of spatial database, which also support the storage and query of LineString.
The range query and $k$NN are the supported queries for the point data, but not for trajectory.
It is promising that these spatial database systems can be extended with trajectory search operator \cite{Pandey2018a} by constructing specific indexing structures and search paradigm in the future, as trajectory is composed of points. In Section~\ref{sec:spatialindexing}, we will review the index structures built over point data.
%Next, we will briefly introduce some representative systems, including Hadoop-GIS \cite{Aji2013}, GeoSpark \cite{Yu2015}, and Simba \cite{Xie2016}.
}


%\bao{More studies of the systems and their supported queries. Draw a table to illustrate the difference.}
\subsection{Trajectory Pre-processing}
\myparagraph{Trajectory Cleaning}
Since trajectory data is usually collected by a GPS with a global average user range error (URE) of 7.8 m (25.6 ft), with 95\% probability, such points in the trajectory are \textit{noisy} \cite{Zheng2015b}. Moreover, the sampling rate of GPS varies in different applications. Two vehicles crossing the same path may have a different number of sampled points. These factors will lead to the value change of distance or similarity, and make it imprecise to analyze further.
Hence, when we get a raw trajectory dataset, the first step is to clean the data.

\textit{Segmenting} \cite{Buchin2011}, \textit{calibration} \cite{Su2013} and \textit{enriching} \cite{Alvares2007} are the three most common cleaning techniques on trajectory data.
Specifically, segmenting will cut a long trajectory into several short trajectories, e.g., analysis of every taxi trip makes more sense than analyzing the whole day taxi trajectory.
\citet{Buchin2011} addressed the problem of segmenting a trajectory based on spatiotemporal criteria.
\citet{AAlewijnse2014} proposed an algorithmic framework for criteria-based segmentation of trajectories that can efficiently process a large
class of criteria.

\citet{Su2013} proposed calibration method to transform a heterogeneous trajectory dataset to one with (almost) unified sampling strategies, in order to achieve a more precise similarity between two trajectories.
For the points with noise, calibration will detect them first and fix to make the trajectory consistent instead of filtering the noise directly.
\citet{Liu2012a} took advantage of road networks topology, geometry information, and trajectory historical information on large scale to conduct the calibration.

When a trajectory is a set of sparse points, \citet{Alvares2007} enriched with more points and semantic information for a complete analysis.
\citet{Yan2011} proposed a framework that enables annotating trajectories of heterogeneous trajectories for any kind of moving objects, with semantic data provided by multiple 3rd party sources.
In contrast, trajectory simplification \cite{Zhang2016e} will remove the redundant points when the sampling rate is high.

\myparagraph{Trajectory Compression}
Existing trajectory compression can be divided into two groups: simplification-based and road network-based.
Excluding the extra points is a common compressing method when the sampling rate is high, which is known as {\em trajectory simplification} \cite{Zhang2016e,Chen2009,Lange2009} and also used in trajectory cleaning.
Removing the points can lead to a more compact size, but it also reduces the quality of the trajectory.
Besides lowering the storage, an error ratio is defined to guarantee that the simplified trajectory is still similar to the original trajectory \cite{Long2013}.

Alternatively, a road network can be used to support compression \cite{Kellaris2013,Song2014,Han2017,Popa2015}, and avoid harming the quality to some extent.
Each trajectory will be projected to the road network as a sequence of road segments.
By encoding each road segment uniquely with a Huffman code \cite{cormen2009introduction}, the trajectory can be represented as a sequence of symbols, which reduces the storage a lot as compared with using latitude and longitude.
Further, string compression techniques \cite{Koide2017,Yang2017b} can be used for trajectory data, including compressing the temporal information.

\myparagraph{Map-matching}
{With a road network, map-matching \cite{Lou2009,Newson2009} projects a raw trajectory onto a real path, it will serve for the cleaning and compression purposes \cite{Kellaris2013}.
The road network dataset of whole world available from \textsc{OpenStreetMap}, and some regions such as \textit{California} \cite{Leskovec2009} and the whole USA.\footnote{\url{http://www.dis.uniroma1.it/challenge9/download.shtml}}}
The road network is always modeled as a weighted graph \cite{cormen2009introduction}, where the road segment is an edge, and the weights could represent the length of the road. Further, a path mapped from raw trajectory is a set of connected edges in the road network.
%When the road network is not available, using the trajectory data to construct the road network \cite{Ahmed2015} can be seen as an opposite direction of map-matching.}

Map-matching is challenging in terms of effectiveness and efficiency.
For efficiency, we need to find the nearest road segments for each point in the trajectory; then the candidate road segments are connected to generate possible paths. Overall, uncertainty is the primary challenge, which reflects on the selection of parameters and candidate paths, and shortest path search.
For effectiveness, mapping a trajectory to the path where the vehicle crossed exactly is the objective. The ground truth matters to evaluate the precision of map matching.
Usually, there are three ways to generate the ground truth: 1) using real vehicles equipped with GPS devices on the road \cite{Newson2009}; 2) labeling the mapped path by humans \cite{Lou2009}; 3) simulating the GPS sampling \cite{Jagadeesh2004} which needs less cost and labor compared with the former two methods.

\subsection{Research Gaps}
\sheng{
	The research gaps in trajectory management systems are three-fold:
	\begin{itemize}
		\item Existing systems are all built over point-based trajectory data.
		Point-based representations are easy to work with, but are not space
		efficient as a float number usually needs eight bytes to store.
		The efficiency of queries over trajectories also suffers from the point-based trajectory similarity measure and indexing, which we will introduce in next two sections.
	%	We also show that point-based index will occupy 
		
		\item The map matching based on the road network is useful for improving the quality of vehicle trajectories, especially for the search and compression. However, existing system still remains on the point-based storage without considering the new features of mapped trajectories.

		\item From the system perspective, supporting various common queries more than range and \knn queries over trajectories are essential, especially that the input for a \knn query can be a trajectory, while most existing systems do not support this.
	\end{itemize}
}


==> 1-Survey-trajectory 2/tableApplications.tex <==
\hspace{-4em}\begin{table}
	\centering
	\ra{0}
	\caption{A summary of trajectory applications, where ``P2P'' denotes the point-to-point distance, and ``P2T'' denotes the point-to-trajectory distance.}
	\vspace{-1em}
	\label{tab:applications}
	\scalebox{0.75}{
		\begin{tabular}{cccccccc}
			\toprule
			\addlinespace[0pt]\rowcolor{gray!30}
			\textbf{Type} &                             \textbf{Work} & \textbf{\makecell {Map\\matching}} & \textbf{Storage} & \textbf{Measure} & \textbf{\makecell{Representative \\ query}} & \textbf{Clustering} & \textbf{Indexing} \\
			             \addlinespace[0pt]\midrule               &              \makecell{Monitoring  \\ \cite{Wang2019,Wangsheng2018,Xie2017a}} &     \cmark     &     segment      &       -        &     \makecell{Range \\query }     &      \cmark      &      \cmark       \\ % \cmidrule{2-8}
			                       \makecell{Road \\Traffic}                        &                   \makecell{ Jam \& Flow\\ \cite{DAndrea2017,Zheng2014a,Jeung2008}} &     \cmark     &     segment      &      EBD      &     \xmark      &      \cmark      &      \cmark       \\  %\cmidrule{2-8}
			                                                      &                \makecell{Anomaly   \\\cite{Chen2012a,Wang2018f}} &     \xmark     &      point       &     EDR             &     \xmark            &                  \cmark&    \cmark               \\ \midrule
			                                                      &         \makecell{Network design  \\ \cite{Chen2014a,Liu2016,Pinelli2016}} &     \xmark     &   point               &    P2P              &   \makecell{Constrained\\ path search}              &  \cmark                &  \cmark                 \\  %\cmidrule{2-8}
			                     \makecell{Green \\Transport}                       &              \makecell{  Navigation \\\cite{Dai2016,Guo2018a}} &     \cmark     &      segment            &  \xmark                &   \makecell{Shortest \\path query}              &    \xmark              &         \cmark          \\  %\cmidrule{2-8}
			                                                      &              \makecell{ Carpooling \\ \cite{Hsieh2017,He2014}} &     \xmark     &            segment      &        P2P         & Join                &      \cmark            & \cmark                  \\ \midrule
			                                                      &          \makecell{  Trip search \\  \cite{Wang2018a,Wang2017}} &     \xmark     &        point          &    P2T             &    TkSTT             &        \cmark          &       \cmark            \\  %\cmidrule{2-8}
			                       \makecell{Tourism \\ Planning}                      &        \makecell{   Customized trip
			              \\ \cite{Wang2018b,Chen2011a}} &     \xmark     &         point         &         P2P         &        \makecell{ Frequent \\path }       &        \cmark          &             \cmark      \\ %\cmidrule{2-8}
			                                                      &             \makecell{Interest Discovery \\\cite{Palma2008,Wang2018b}} &     \xmark     &      point            &     \makecell{ P2P \\P2T}            &           \makecell{ Multiple \\queries }        &        \cmark          &    \cmark               \\ \midrule
			                                                      &              \makecell{Billboard \\\cite{Zhang2018c,Zhang2019a}} &     \xmark     &     point             &     P2T             &     Set cover        &       \xmark           &             \cmark      \\ %\cmidrule{2-8}
			                   \makecell{Site\\ Selection}                     &           \makecell{Charging station\\  \cite{Li2015c,Liu2017d}} &     \xmark     &     point             & \xmark                 &     \xmark            &      \xmark            &         \cmark          \\  %\cmidrule{2-8}
			                                                      &          \makecell{ Facility route\\  \cite{Bao2017a,Wang2018c,Li2018d}} &     \cmark     &  segment                &   P2T               &     \makecell{ Shortest \\path query}           &   \cmark               & \cmark                  \\ 
			                                                     % \midrule
			                                                     % &            Sport play    \cite{Wang2019b} &     \cmark     &    point              &    ED              &        \cmark         & \xmark                 &   \xmark                \\
			                      %Non-urban                       &            Map inference \cite{Ahmed2015} &     \cmark     &    segment              &    \cmark              &      \xmark           &   \cmark               &        \xmark           \\
			                                    %                  & {Public safety} \cite{Song2014b} &     \xmark     &     point             &     ED             &     \xmark            &   \cmark               &                  \xmark \\
			                                                       \bottomrule			                                          
		\end{tabular}}
		\vspace{-1em}
\end{table}


==> ack.tex <==
\section{Acknowledgments}

Identification of funding sources and other support, and thanks to
individuals and groups that assisted in the research and the
preparation of the work should be included in an acknowledgment
section, which is placed just before the reference section in your
document.

This section has a special environment:
\begin{verbatim}
  \begin{acks}
  ...
  \end{acks}
\end{verbatim}
so that the information contained therein can be more easily collected
during the article metadata extraction phase, and to ensure
consistency in the spelling of the section heading.

Authors should not prepare this section as a numbered or unnumbered {\verb|\section|}; please use the ``{\verb|acks|}'' environment.

==> deep-tab.tex <==
\begin{table}
	\ra{-0.5}
	\centering
	\caption{Recent work on deep trajectory learning.}
%	\vspace{-1em}
	\scalebox{0.82}{
	\hspace{-3em}	\begin{tabular}{ccccccccc}
		\toprule	\addlinespace[0pt]\rowcolor{gray!30}\rowcolor{gray!30}
		  \textbf{Work} &   \textbf{Tasks} & \textbf{Data sources}  & \textbf{\makecell{~~~Encoder/Input}} & \cellcolor{gray!30} \textbf{\makecell{Decoder/Output}} & \textbf{\makecell{Deep Model}} & \textbf{\makecell{More Feature}} & \textbf{\makecell{Loss Function}} \\ \addlinespace[-1pt] \midrule

		\cite{Wang2019i} & Data recovery  & Taxi  & LSTM  & BiLSTM &  seq2seq & \makecell{Spatial \\temporal\\ attention} & softmax \\
		\cite{Ouyang2018} &\makecell{Synthetic data \\generation} & Mobile GPS& \makecell{Matrix \\representation}&  \makecell{matrix \\representation} &GAN &\makecell{Semantic \\ duration}&WGAN-GP \\ 
%		\cite{Systems2017} &  \makecell{Mobility \\simulation}& Cellular data&IO-HMMs&  \makecell{Distribution\\ coefficients}&GAN-LSTM &\makecell{Activity \\Features}&\\
		\makecell{\cite{Liu2018}} &\makecell{Privacy \\protection}& APPs&Embedding& \makecell{Random\\ deviations}&CGAN&POI &minimax\\
		\makecell{\cite{Gupta2018} }&\makecell{Mobility \\prediction}& Video&LSTM&LSTM&GAN&Pooling&L2\\\midrule
		
		\cite{Li2018a} & \makecell{Similarity \\computation}&Taxi&\makecell{Token\\ embedding}&\makecell{Conditioned \\sequence}&RNN&\makecell{Sampling \\rate,\\noise}&\makecell{Spatial \\proximity\\ aware loss}\\
		\cite{Yao2017} &Clustering& vessels &LSTM &LSTM&Seq2Seq &\makecell{Moving \\behavior} &\\
		\makecell{ \cite{Yao2019} }&Metric learning&&\makecell{SAM-augmented \\LSTM}&-&RNN&\makecell{Attention \\on grids}&\makecell{weighted\\
		ranking loss}\\
		\cite{Gao2017b} &\makecell{Trajectory-User\\
		Linking}& segmentation&&&&\\
%		\cite{Wu2017a}&&\makecell{Trajectory \\modeling}& & & &RNN&- & \\
		\cite{Zhang2019d}  & \makecell{Similarity \\computation}&\makecell{Activity \\trajectory} &RNN&RNN&Seq2Seq&\makecell{Spatial\\temporal\\activity}&weighted loss \\
%		\cite{Boonchoo2019a} &&Embedding &&&&&&\\ 
		\midrule
		
%		\cite{Xuan2016} &&\makecell{Transportation\\ mode}&&LSTM&LSTM&\makecell{Shared\\memory \\LSTM}&&\\
		\cite{Liu2016c} &\makecell{Next \\location} &Check-in&&&ST-RNN& & \\
%		\cite{Jin2018} &&\makecell{Next \\ location\\ with time}&&\makecell{Multi-modal \\embedding} &&RNN & &\\
		\cite{Zhou2018a} &Next trajectory&Flickr &\makecell{variational\\ encoder}&LSTM &RNN &Attention & \\
		\cite{Wu2019} &\makecell{Query \\optimization}&Taxi&LSTM&LSTM&Seq2Seq&-&\makecell{minimum \\square error}\\
		\cite{Gao2019c} &Next POI &Check-in &\makecell{POI\\ embedding}&Classifier&CNN&\makecell{Variational\\ attention}&\makecell{empirical\\ risk }\\
		\cite{Lv2019} &Destination&Taxi&Image&&CNN&&\\
		\cite{Zhang2017e} &\makecell{Crowd \\prediction}&Taxi&Grid&-&ST-ResNet&\makecell{weather\\ holiday}&\makecell{Root Mean \\Square Error}\\
%		\cite{Jiang2019} &&\makecell{Online \\crowd}&Big events&Grid &LSTM&ConvLSTM&&\makecell{reconstruction \\error}\\
		\bottomrule
	\end{tabular}}
\label{tab:deep}
%\vspace{-1.5em}
\end{table}


==> deep.tex <==
\sheng{\section{Emerging trend on Deep Trajectory Learning}
\label{sec:deep}
In the last three years, deep learning \cite{Lecun2015} becomes a useful tool to solve several problems of trajectory analytics.
%We have also sporadically covered some work that utilizes deep learning in anomaly detection, clustering, and classification In previous sections.
Next, we will conclude three types of representative work systematically, Table~\ref{tab:deep} shows their solved problem, with the model used in each work and their loss functions.

\input{deep-tab}

\subsection{Trajectory Data Recovery and Generation}
Sharing raw trajectory data always faces concerns on privacy \cite{Guo2015b}, and some datasets choose to remove most information and just maintain the source and destination for each trajectory, such as the NYC taxi trip dataset. 
However, such cleaning makes it hard to conduct a precise analysis of real trends and demand from commuters.
%\citet{Systems2017} employed deep recurrent neural network architecture to generate human activity chains from cellular data, which provides transportation planners, policy-makers, and related stakeholders with detailed and timely travel demand models.
A novel Deep Hybrid Trajectory Recovery model \cite{Wang2019i} aims to recover low-sampled trajectory data between a source and a destination.
Different to trajectory data recovery from a source and a destination, trajectory synthetic data generation aims to learn an open trajectory based on a private dataset which is complete.
\citet{Ouyang2018} proposed a generative model for trajectory by considering the constraint of privacy in data sharing, and high-order geographic and semantic features of human mobility.
\citet{Liu2018} designed a framework which uses generative adversarial networks (GAN) \cite{Goodfellow2014} to protect privacy but still enable effective analytics over a synthetic dataset.
%\citet{Kulkarni2018} considered the semantic information when generating a synthetic trajectory using GAN.
\citet{Gupta2018} proposed to generate pedestrian trajectories with GAN, and the main difference is that it is for pedestrian walk trace under cameras.
Not only can the generative model work for data recovery and generation, but also for anomaly detection. \citet{Liu2020} predicted the probability of a new trajectory being an anomaly.% using a deep generative sequence model.
%\cite{Kulkarni2018} conducted an evaluation.
%trajectory privacy

\subsection{Trajectory Representation and Metric Learning}
Representation learning of trajectory aims to convert trajectories into vectors with a fixed dimension, and then most trajectory analytics can be done using existing mature analytics based on Euclidean distance.
The main objective of deep trajectory embedding is for classification \cite{Endo2016}, clustering \cite{Yao2017}, and fast trajectory similarity search \cite{Li2018a,Yao2019}.
\citet{Endo2016} proposed a method that automatically extracts additional features using a convolution neural network (CNN), for transportation mode classification problem, their method converts a raw trajectory data structure into an image data structure while maintaining effective spatiotemporal information.
%\citet{Gao2017b} embedding for human mobility prediction.
%
%\cite{Ouyang2018} proposed to use GAN to preserve privacy for trajectories.
%\citet{Wu2017a} proposed RNN-based models to model trajectory, for the tasks over road network-constrained trajectories.
The recurrent network is widely used in deep trajectory embedding inspired by the word2vec. \citet{Li2018a} transferred each spatial-only trajectory to a vector first based on a probability model, and proposed a new spatial proximity aware loss function and a cell representation learning approach that incorporate the spatial proximity into the deep learning model.
\citet{Zhang2019d} further learned the representation for activity trajectory similarity computation, and proposed a novel loss function based on the attention mechanism in natural language processing to distinguish these three kinds of information, and an encoder-decoder model is also used similar to \cite{Li2018a}.
%\cite{Taghizadeh2019}
%\citet{Boonchoo2019a} proposed embedding for the attribute-aware trajectories.
%\cite{Pandhre2018} 
%\subsection{Metric learning}
Metric learning aims to learn similarity scores with an existing measure \cite{Yao2019} when inputting two trajectories, and it is generic to accommodate any existing trajectory measure and fast to compute the similarity of a given trajectory pair in linear time. The basic idea is to samples a number of seed trajectories from the given database and then use their pair-wise similarities as guidance to approximate the similarity function with a neural metric learning framework.
%this is put as an explansion, temporal aware.
%\citet{Chen2019b} learned a deep embedding approach for clustering and profiling taxi trip purposes.

\subsection{Trajectory Prediction for Human Mobility Analytics}
As trajectory is a sequential set of points, predicting where to go next \cite{Monreale2009} has several applications, e.g., indicating future locations of taxi drivers to assign new passengers, and restaurant recommendation based on users' check-ins.
%A survey \cite{Wang2019g} presents an overview on trajectory prediction research using traditional methods, including Markov-based, time-series based, and compression-based.
%Generally, prediction based on historical trajectories can be divided into two types: 1) next-point prediction \cite{Xuan2016,Liu2016c}; 2) crowd flow prediction \cite{Zhang2017e,Jiang2019}.
%Predict the destination of taxi trips based on initial partial trajectories, in the ECML/PKDD competition.
%As prediction itself is a learning-based task, and 
%neural network gradually becomes a as it enables modeling complex patterns and prediction problems.
%\subsubsection{Next-point Prediction}
%Since individual next-point prediction has a common objective, improving prediction precision is the goal.
Temporal information is crucial to train an effective prediction model, and recurrent neural network (RNN) is widely used.
%\citet{Xuan2016} predict transport mode of the next movement.
\citet{Liu2016c} extended RNN and proposed a novel method called Spatial Temporal RNN (ST-RNN) for next-point prediction, which can model local temporal and spatial contexts in each layer with time-specific transition matrices for different time intervals and distance-specific transition matrices for different geographical distances.
%\cite{Lei2011,Besse2018a,Rossi2019} 
%\citet{Jin2018} proposed human mobility prediction model based on Attentional Recurrent Networks.
\citet{Zhou2018a} predicted the future trip that the user would travel rather than predicting a single point, which can also reconstruct users trajectory.
Their model everages two variational latent factors which are respectively the traditional latent variables and the variational hidden state attention, for learning trajectory-level context.
NEIST \cite{Wu2019} applies an RNN to predict future positions of moving objects based on observed trajectories, and further accelerate the spatial-temporal queries.

Instead of using RNN which cannot train long sequence, \citet{Gao2019c} firstly incorporated convolutional neural network (CNN) to capture long term and structural dependency among user check-ins, achieving comparable learning ability with the state-of-the-art RNN based methods, while significantly improving the learning efficiency.
\citet{Lv2019} proposed a novel prediction algorithm T-CONV, which models trajectories as two-dimensional images, and then feed them into a CNN architecture to extract multi-scale patterns for precise destination prediction.
%\cite{Alahi2016}
%\subsubsection{Crowd Prediction}
Since trajectory data in a wide range can also indicate the historical crowd flow from one area to another area, crowd flow prediction \cite{Zhang2017e}  aims to indicate the amount of people that will travel in a given region and time stamp.
Specifically, \citet{Zhang2017e} proposed a deep-learning-based approach, called ST-ResNet, to forecast the in-flow and outflow of crowds in each and every region of a city.}
%To meet the demand that crowd flow prediction needs to be done in real time for emergence response,
%\citet{Jiang2019} built an online system which can iteratively take citywide crowd dynamics from the current one hour as input and report the prediction results for the next one hour as output.

%Temporal information
%\input{appendix}

%\subsection{Remarks}
%Trajectory modeling in neural network is a start, here we briefly introduce two kinds of modeling method to fit into neural network.

==> query.tex <==

\section{Trajectory Similarity Measures}\label{sec:distance}
In this section, we will introduce the widely used trajectory similarity measures.
As shown in Figure~\ref{fig:distance-example},
two different kinds of similarity measures are computed between the query and trajectory separately. \sheng{The float number on each dotted line denotes the distance from a query point to a point in the trajectory.}
\begin{figure}[htp]
	\centering
	\includegraphics[height=2.1cm]{graph/distance-measure1.pdf}
	\caption{Two kinds of similarity measures: (a) a query is a set of points; (b) a query is a trajectory.}
	\label{fig:distance-example}
\end{figure}

\subsection{Points to Trajectory}
To measure the distance between a set of points $Q$ and a trajectory $T$ in the $k$ Best Connected Trajectories search problem (\kbct) \cite{Chen2010a,Qi2015,Tang2011},
each query point  {q} will find the nearest point  {p} in $T$, then all the distances from each query point to their nearest neighbor are aggregated to generate the final distance, i.e.,
\begin{equation}
d_{\svar{kBCT}}(Q,T) = \sum_{q\in Q}{\min_{p\in T} d(q, p)}
\end{equation}

Based on the above equation, $d_{\svar{kBCT}}(Q_1, T_1)=1+1.7+2.2=4.9$ in Figure~\ref{fig:distance-example}(a) is the aggregation of distance between every query point in $Q$ to its nearest neighbor point in $T$ (\sheng{three dotted lines}).
\sheng{When there is only one query point, it is a specific and simple case of \kbct and is also the only supported \knn in \cite{Ding2018,Wang2014e}.}
Since scanning every point in the trajectory returns the nearest point, then the complexity of this measure is quadratic.
Note that this measure only works when the query $Q$ is a set of points, and it does not obey the symmetry rule, i.e., $d(Q,T)\ne d(T,Q)$.
Instead of summing up the distance with the nearest neighbor, another well-known measure called the \textit{closest-pair distance (CPD)} \cite{Zheng2015b} which chooses the minimum distance as the final distance, i.e.,
\begin{equation}
d_{\svar{CPD}}(Q,T) = \min_{q\in Q}{\min_{p\in T} d(q, p)}
\end{equation}
\sheng{
Then $d_{\svar{CPD}}(Q_1, T_1)=1$. Compared with $d_{\svar{kBCT}}$, $d_{\svar{CPD}}$ will be more robust when there is an error point which is far to all the query points in the trajectory.}

\subsection{Trajectory to Trajectory}
Since the query above is a set of discrete points, the order among points in trajectory is not considered when computing the distance. 
However, when we compute the distance between trajectories, the order constraint should be met, i.e., the similarity measure for trajectory should obey the \textit{local time shifting} \cite{Chen2005a}. 

\begin{table}
	\ra{1}
	\centering
	\caption{An overview of existing trajectory-to-trajectory similarity measures.}
	\scalebox{0.9}{\begin{tabular}{cccccccc}
		\toprule\addlinespace[0pt]\rowcolor{gray!30}
		 &    &  & & & \multicolumn{3}{c}{\textbf{Robustness}} \\ \addlinespace[-1pt]\cmidrule{6-8}\addlinespace[-3pt]\rowcolor{gray!30}
		\multirow{-2}{*}{\textbf{Categorization}}      &                     	\multirow{-2}{*}{\textbf{Measures}}                     & \multirow{-2}{*}{\textbf{Complexity}} & \multirow{-2}{*}{\textbf{Metric}} & \multirow{-2}{*}{\textbf{\makecell{Parameter-\\free}}} &  \makecell{GPS \\Error} & \makecell{Sampling\\Rate} & \makecell{Point\\ Shift}   \\ \addlinespace[0pt]\midrule
		\multirow{2}{*}{Curve distance}          & Hausdorff  \cite{Nutanong2011} & $\mathcal{O}(n^2)$ & \xmark &\cmark&\xmark&\xmark &\xmark\\ 	\cmidrule{2-8}
		& Fr\'echet \cite{Eiter1994} & $\mathcal{O}(n^2)$  & \xmark&\cmark &\xmark&\xmark &\xmark \\\midrule				
		\multirow{2}{*}{Real distance}           &     {dtw} \cite{yi1998efficient}      & $\mathcal{O}(n^2)$ & \xmark&\cmark&\xmark&\xmark &\xmark\\ \cmidrule{2-8}
		&   {erp} \cite{Chen2004}      & $\mathcal{O}(n^2)$  & \cmark&\xmark &\xmark&\xmark &\xmark\\ \midrule
		\multirow{2}{*}{Edit distance}           &   {edr} \cite{Chen2005a}  & $\mathcal{O}(n^2)$  & \xmark &\xmark &\cmark&\xmark &\xmark\\ \cmidrule{2-8}
		&   {lcss} \cite{vlachos2002discovering}  & $\mathcal{O}(n^2)$  & \xmark&\xmark &\cmark&\xmark &\xmark  \\   \bottomrule
	\end{tabular}}
	\label{tab:distancemeasures}
\end{table}

%\bao{1) Flat description of each measure, 2) no example on the pros and cons of each class of measure. 3) need to distinguish them well in your table 2.2.}
Several similarity measures have been proposed for trajectory data
in recent years.
As shown in Table~\ref{tab:distancemeasures}, we broadly divide the widely used six similarity measures into three kinds: curve-based, real-distance, and edit-distance.
We will elaborate each measure with the formal definitions and Figure~\ref{fig:distance-example}(b).
As a trajectory can also be viewed as a \textit{geometric curve}, Hausdorff distance~\cite{Nutanong2011,Roh2011} measures
how far two subsets of a metric space are from each other by choosing the max-min distance, without considering the order constraint.

\begin{equation}
\label{equ:hau}
d_{\tvar{Hau}}(Q,T)=\max_{p\in T}{\min_{\ q\in Q}  {eucdis}}
\end{equation}

Fr\'echet distance~{\cite{Eiter1994,Agarwal2014}} extends the Hausdorff
distance to account for location and ordering of the points along the
curves, as shown in Equation~\ref{equ:fre}, where $p$ and $q$ are the head (first) point of $T$ and $Q$, respectively, and $T_h$ and $Q_h$ are the sub-trajectory excluding the head $p$ and $q$.
\sheng{
Taking Figure~\ref{fig:distance-example}(b) as an example, $d_{\tvar{Hau}}$ and $d_{\tvar{Fre}}$ will return the same value $3.1$, as the matching shown in the figure not only finds the nearest neighbor for each point, but also obeys the local time shifting (order constraint).
If any two points in $T_5$ swap the location, $d_{\tvar{Hau}}$ does not change, while $d_{\tvar{Fre}}$ will change as the order is broken.}

As a trajectory can be also viewed as a time series, many similarity
measures originally designed for time series search can be deployed in
trajectory top-$k$ search~{\cite{Zheng2015b}}, such as Dynamic
Time Warping (\dtw) \cite{yi1998efficient}, Longest Common
Subsequence (\lcss) \cite{vlachos2002discovering,Morse2007}, and Edit
Distance on Real sequence (\edr) \cite{Chen2005a} and Edit distance with Real Penalty {(\erp)}~\cite{Chen2004}.
\sheng{\dtw computes the distance based on the sum of minimum distances, instead of choosing the maximum in Fr\'echet distance.}
Equation \ref{equ:dtw} shows the formal definitions of \dtw.
Figure~\ref{fig:distance-example}(b) shows the distance computation using 
\dtw, where every point in $T_5$ and $Q_3$ is matched with each other and will contribute to minimizing the final aggregated distance without breaking the order constraint, i.e., $d_{\tvar{DTW}}(Q_3,T_5)=1.2+3+1+2.2+3.1=10.5$.
\sheng{Note that \dtw has a parameter sometimes when it considers the window constraint $r$ on the matching points' order, e.g., $|o(p)-o(q)|\le w$, where $o(p)$ denotes the order of $p$ in $T$. The window parameter $w$ is widely used in time series data. However, there is always no such constraint on trajectory data.}

\begin{equation}\small
\label{equ:fre}
d_{\tvar{Fre}}(Q,T)=\begin{cases}0,\ \text{if}\ Q=\emptyset\ and\ T=\emptyset\\
\infty,\ \text{if}\ Q=\emptyset\ or\ T=\emptyset\\
\max\{d(q, p), \min\{d_{\tvar{Fre}}(Q_h,T_h),\ d_{\tvar{Fre}}(Q, T_h), d_{\tvar{Fre}}(Q_h, T)\}\},\ \text{otherwise}
\end{cases}
\end{equation}

\begin{equation}\small
\label{equ:dtw}
d_{\tvar{DTW}}(Q,T)=\begin{cases}0,\ \text{if}\ Q=\emptyset\ and \ T=\emptyset\\
\infty,\ \text{if}\ Q=\emptyset\ or\ T=\emptyset\\
d(q, p)+\min\{d_{\tvar{DTW}}(Q_h,T_h),\ d_{ \tvar{DTW}}(Q, T_h),\ d_{\tvar{DTW}}(Q_h, T)\},\ \text{otherwise}
\end{cases}
\end{equation}

%
%, while no vehicle trajectory data is used.
%As a trajectory can also be viewed as a \textit{geometric curve},
%similarity measures between curves can also be used for trajectory
%similarity search~{\cite{Xie2017a}}.

Instead of computing the real distance, computing the edit distance (0 or 1) is more robust to the GPS error as two far points will lead to a big distance if using \dtw.
To judge whether two points are matched, edit-distance based measures need to set a range threshold $\tau$, as shown in Equation~\ref{equ:match}, where $||$ denotes $L1$ norm, and $p_x$ and $p_y$ denote the latitude and longitude of point $p$, respectively.
Then we can define \lcss and \edr as shown in Equation~\ref{equ:lcss} and \ref{equ:edr}.
The basic difference between \lcss and \edr is that \lcss is defined to measure how similar two trajectories are, while \edr is for measuring how different two trajectories are.
\sheng{
For example, if we set $\tau=0.5$ in Figure~\ref{fig:distance-example}(b), then there is no matched point, $d_{\scriptscriptstyle \tvar{LCSS}}(Q_3,T_5)=0$ and $d_{\scriptscriptstyle \tvar{EDR}}(Q_3,T_5)=4$; if we set $\tau=5$, then every point can be matched, and $d_{\scriptscriptstyle \tvar{LCSS}}(Q_3,T_5)=4$ and $d_{\scriptscriptstyle \tvar{EDR}}(Q_3,T_5)=0$. Hence, these two measures highly depends on the parameter $\tau$.}
\begin{equation}
\label{equ:match}
\var{match}(p, q)=\begin{cases}\var{true},\ \text{if}\ |p_x- q_x|\le\tau\ \text{and}\ |p_y-q_y|\le\tau\\
\var{false},\ \text{otherwise}
\end{cases}
\end{equation}

\begin{equation}\small
\label{equ:lcss}
d_{\scriptscriptstyle \tvar{LCSS}}(Q,T)=\begin{cases}0,\ \text{if}\ Q=\emptyset\ \text{or}\ T=\emptyset\\
1+d_{\scriptscriptstyle \tvar{LCSS}}(Q_h, T_h),\ \text{if}\ \var{match}(p,q)=\var{true}\\
\max\{d_{\scriptscriptstyle \tvar{LCSS}}(Q, T_h),\  d_{\scriptscriptstyle \tvar{LCSS}}(Q_h, T)\},\ \text{otherwise}
\end{cases}
\end{equation}

\begin{flalign}\small
\label{equ:edr}
d_{\scriptscriptstyle \tvar{EDR}}(Q,T)=\begin{cases}
|Q|,\ \text{if}\ T=\emptyset \\
|T|,\ \text{if}\ Q=\emptyset \\
\min\{d_{\scriptscriptstyle \tvar{EDR}}(Q_h,T_h), d_{\scriptscriptstyle \tvar{EDR}}(Q, T_h)+1,\ d_{\scriptscriptstyle \tvar{EDR}}(Q_h, T)+1\},\ \text{if}\ \var{match}(p,q)=\var{false} \\
\min\{1+d_{\scriptscriptstyle \tvar{EDR}}(Q_h,T_h), d_{\scriptscriptstyle \tvar{EDR}}(Q, T_h)+1,\ d_{\scriptscriptstyle \tvar{EDR}}(Q_h, T)+1\},\ \text{otherwise}
\end{cases}
\end{flalign}


As they do not obey the triangle inequality which is an essential requirement in the \textit{Metric} space pruning, all the existing measures are \textit{non-metric} except for {\erp}.
\citet{Chen2004} defined a metric trajectory similarity measure, as shown in Equation \ref{equ:erp}, where
point $g$ can be any constant point in the space, it is always set as the origin, i.e., $g=\{0,0\}$.
However, $g$ is also a parameter, the changes will also lead to the change of distance value similar to \lcss and \edr, and further affect the results of \knn search.
Hence, a parameter-free measure is essential for trajectory search.

\begin{flalign}\small
\label{equ:erp}
d_{\scriptscriptstyle \tvar{ERP}}(Q,T)=\begin{cases}\sum_{p\in T}d(g, p),\ \text{if}\ Q=\emptyset\\
\sum_{q\in Q}d(q, g),\ \text{if}\ T=\emptyset\\
\min\{d_{\scriptscriptstyle \tvar{ERP}}(Q_h,T_h)+d(q, p),d_{\scriptscriptstyle \tvar{ERP}}(Q, T_h)+d(g, p),d_{\scriptscriptstyle \tvar{ERP}}(Q_h, T)+d(q, g)\},\ \text{otherwise}
\end{cases}
\end{flalign}



%\sheng{The scenarios, there is not }
\subsection{Complexity and Robustness}
Table~\ref{tab:distancemeasures} compares characteristics of six similarity measures in four-fold: complexity, metric, parameter, and robustness.
\sheng{Since the parameter can be easily observed from their definitions, we will elaborate the other three characteristics next.}

\myparagraph{Complexity}These similarity measures were designed to make search more robust
against local time shifting.
However, existing similarity measures always try to find the best matching
point without breaking order constraints, thus requiring dynamic
programming solutions with a quadratic complexity ($\mathcal{O}(n^2)$).
%New measures such as {\small $\textsf{EDwP}$} \cite{ranu2015indexing} were proposed to reduce the complexity and maintain precision.
Learning an embedding for a trajectory \cite{Li2018a,Yao2017} to compute the Euclidean distance based on vectors with fixed length is promising as it achieves linear ($\mathcal{O}(n)$) computation, but requires long training time for the learning models.
%However, {\erp} has a complexity of $\mathcal{O}(n^2)$ despite being
%metric, and is therefore not useful for problems such as {\kpath} 
%in large collections.

%Effectiveness evaluation of these similarity measures over
%time series data~{\cite{UCRArchive}} was performed by
%{\citet{Wang2013b}}.
\myparagraph{Metric}\sheng{Being metric or not is crucial for a similarity measure, as obeying the triangle inequality is a fundamental feature for reducing distance computation. Here, we use an example to illustrate how to avoid distance computation for a metric similarity measure-Euclidean distance.
In Figure~\ref{fig:triangle}, a query point $q$ is searching the nearest neighbor, $p_1$ and $p_2$ are the two points to be scanned next, and we just computed $d(q,p_1)$. Before conducting distance computation with $p_2$, we can estimate the lower and upper bound of $d(q,p_2)$ based on $d(q,p_1)$ and $d(p_1, p_2)$, where $d(p_1, p_2)$ can be computed off-line for any query.
With the lower bound, we can compare it with $d(q, p^{'})$ where $p^{'}$ is the current founded nearest neighbor. If the lower bound is bigger, we can discard $p_2$ directly as it cannot beat $p^{'}$ to be the nearest neighbor.}
\begin{figure}[htp]
	\centering
	\includegraphics[height=2.5cm]{graph/metric.pdf}
	\caption{Using triangle inequality to estimate the bounds.}
	\label{fig:triangle}
\end{figure}

\myparagraph{Robustness}Besides the high complexity and metric,
most similarity measures are sensitive to noise, sampling rate, and point shift (points are shifted on the path where the trajectory lies). In other words, the existence of noise (due to GPS errors), more (less) sampled points or point shift on a trajectory will make it be judged as dissimilar to the original trajectory using the existing measures in Table~\ref{tab:distancemeasures}.
\sheng{\citet{Wang2013a} also conducted an effectiveness evaluation on the robustness of these six measures over a real-world trajectory dataset.
	
Here, we use an example in Figure~\ref{fig:robustness} to illustrate why they are not robust, where $T_1$ and $T_2$ are two similar vehicle trajectories in the road network as they crossed the same path. After sampling, we will use a set of points to denote them, the ideal sampling (b) will record the same number of points which are also pair-wise close. Nevertheless, in the real case, the sampling rate and time are various, e.g., the point shift (c) will sample the same number of points in the road, but not pair-wise close. The GPS error (d) will sample points that are not in the road, and the inconsistent sampling rate (d) will lead to a different number of points for two similar trajectories. Each of the above three factors will lead to a distance value bigger than that of the ideal sampling using existing similarity measure. 
However, a robust similarity measure should always return the same value if such cases occur, and we find that existing similarity measures are not robust to the point shift, error, and sampling.}


\subsection{Metric learning}
\cite{Yao2017,Li2018a} learns same length vector, and further use the Euclidean distance.



%We further show the complexity.

\begin{figure}
	\centering
	\includegraphics[height=4cm]{graph/robustness.pdf}
	\caption{A similarity measure is sensitive to the point shift, error, and sampling rate.}
	\label{fig:robustness}
\end{figure}


\subsection{Research Gaps}
\sheng{
	Even though the trajectory similarity measure is under-explored in the past two decades, there is still no such a robust measure with low complexity to our best knowledge. Specifically, the research gaps are two-fold:
	\begin{itemize}
		\item An effective similarity measure needs to be robust to the GPS error, point shift, and sampling rate, and should also be parameter-free. However, there is no such a measure as we concluded in Table~\ref{tab:distancemeasures}.
		%Moreover, evaluating the effectiveness toward robustness for the similarity search is another gap.
		
		\item The complexity of existing measures is quadratic, and most of them are non-metric. When we need to conduct \knn search over a vital amount of data, it is unscalable in two-fold: 1) point-wise computation is expensive; 2) distance computation pruning by triangle inequality cannot be applied.
	\end{itemize}
}

%\subsection{Beyond Pre-processing: Trajectory Search}
%Pre-processing over trajectories mainly serve for the effective analytics.
\section{Spatial-Only Trajectory Search}
%As one of the most important data discovery tools, query over the trajectory can help select the most relevant data instead of digesting all the dataset for a specific application.
%As we can see, existing work on trajectory pre-processing deal all the data with a same representation-points for the generality of point data management.
%However, for different trajectory data, the modeling method highly depends on the data type and applications.

%To explain the difference of these queries clearly, we will use an exemplar figure.

%Note that trajectory is composed by points, so we also cover the related work on point data search.
%In the next two sections, we will elaborate the queries over spatial-only and spatial-textual trajectory data, respectively.
\begin{table}
	\centering
	\ra{1}
	\caption{{An overview of existing queries over trajectory data.}} 
	\begin{comment}
	%IR: Information Retrieval \cite{Broder2003}, 
	$k$NN: $k$ 
	Nearest Neighbour \cite{Guttman1984},
	TkSK: Top-k Spatial Keyword Query~\cite{chen2013spatial}, 
	ANN: Aggregate Nearest Neighbour Query~\cite{Papadias2005},
	ATNN: Aggregate Textual Nearest Neighbour Query~\cite{Li2010,Yao2016},
	kBCT: k Best-Connected-Trajectory Query~\cite{Chen2010a}, 
	TkSTT: Top-$k$ Spatial-Textual Trajectory Query~\cite{Wang2017,Shang2012a}.
	\end{comment}
	\label{tab:methods}
	\scalebox{0.9}{\begin{tabular}{ccccccc}
			\toprule\addlinespace[0pt]\rowcolor{gray!30}
			\textbf{Data}&\textbf{Type}&\textbf{Query} & \textbf{Input} & \textbf{Output} & \textbf{Measure}&  \textbf{Index} \\\addlinespace[-2pt]
			\midrule
			&\multirow{2}{*}{Boolean}& Range \cite{SanduPopa2011,Krogh2016} & range & trajectories& N/A & R-tree \\
			\cmidrule{3-7}
			&& Path \cite{Krogh2016,Koide2015} & path & trajectories& N/A & R-tree \\
			\cmidrule{2-7}
			&\multirow{4}{*}{$k$NN}&\knn~\cite{Guttman1984,beckmann1990r,Sellis1987} & point & points & Euclidean & R-tree  \\
			\cmidrule{3-7}
			&&$k$NNT \cite{vlachos2002discovering,Chen2005a}& trajectory & trajectories& LCSS, DTW & R-tree \\
			\cmidrule{3-7}
			&&\kbct \cite{Chen2010a,Tang2011}& points & trajectories& Aggregate & R-tree \\
			\cmidrule{3-7}
			{\makecell{Spatial\\-only}}&&\ann \cite{Papadias2005,Yiu2005}& points & points & Aggregate & R-tree \\
			\cmidrule{2-7}
			& \multirow{2}{*}{\makecell{Reverse\\ $k$NN}} & \rknn \cite{Tao2004,Chan2008}& \makecell{point} & points& Euclidean & R-tree \\
			\cmidrule{3-7}
			& & R-PNN \cite{Shang2011}& \makecell{point} & trajectories & Euclidean & N/A \\
			\cmidrule{2-7}
			& \multirow{2}{*}{Clustering} & Density-based \cite{Lee2007}& \makecell{thresholds} & paths& N/A & N/A \\
			\cmidrule{3-7}
			& & Partition-based \cite{Chan2018}& \makecell{$k$} & trajectory& Hausdorff & N/A \\
			\midrule
			& &KS \cite{Broder2003,Ding2011a,Daoud2016} & keywords & points & TF-IDF & Inverted list \\
			\cmidrule{3-7}
			%IR \cite{Zobel2006} & keywords & points & TF-IDF & Inverted list \\
			%\hline
			\multirow{4}{*}{\makecell{Spatial\\-textual}}& \multirow{4}{*}{Top-$k$} &\tksk \cite{zhang2014processing,Li2011} & \begin{tabular}{c}point, \\ keywords\end{tabular} & points & Aggregate & IR-tree \\
			\cmidrule{3-7}
			& &\atnn \cite{Li2010,Yao2016}& \begin{tabular}{c}points, \\ keywords\end{tabular} & points & Aggregate& IR-tree\\
			\cmidrule{3-7}
			& &\tkstt \cite{Shang2012a,Zheng2013c}& \begin{tabular}{c}points, \\ keywords\end{tabular} & trajectories &  Aggregate & \begin{tabular}{c}Grid-index, \\ Inverted list\end{tabular} \\
			\bottomrule
			%$\dddot{Q}_{n}^m$
	\end{tabular}}
\end{table}

Figure~\ref{fig:queries} shows three exemplary queries $Q_1$, $Q_2$, $Q_3$ for spatial-only trajectories $T_1$ to $T_6$.
Given three points ($q_1$, $q_2$, $q_3$), $Q_1$ finds the best connected trajectory. Among all six trajectories, $T_1$ and $T_2$ are both possible final results. A similarity measure needs to be defined to distinguish which trajectory is closer to $Q_1$.
Given a range (red box), $Q_2$ finds all the trajectories crossing in it, then $T_3$ and $T_4$ will be returned, it is much simple than $Q_1$ as no similarity measure is needed.
Given a trajectory $Q_3$, it will search the most similar trajectories. Similar to $Q_1$, a similarity measure needs to be defined, while it is between two trajectories rather than points and trajectories.

\begin{figure}[h]
	\centering
	\includegraphics[height=5.5cm]{graph/spatial-only-queries.pdf}
	\caption{Three kinds of spatial-only trajectory queries.}
	\label{fig:queries}
\end{figure}

Table~\ref{tab:methods} concludes different kinds of common queries on trajectory data in terms of four aspects: input, output, similarity measure, and index. The column for ``Index" only lists the representative index structure, we will further elaborate in the following sections.
The queries range from basic trajectory search, top-$k$ trajectory similarity search (spatial-only and spatial-textual), reverse $k$ nearest neighbors search, and trajectory clustering.
Next, we will elaborate on each query, and introduce the common indexing structures used for accelerating the performance.
\subsection{Query Types}
\subsubsection{Basic Trajectory Search}
A basic trajectory search includes three main types of queries.
The first one is a {\em Range Query}
( {rq})~{\cite{SanduPopa2011,Krogh2016,Song2014,Roh2011}} that
finds all (sub-)trajectories located in a spatial region or a temporal region.
The range query has many applications in traffic monitoring, e.g., return all the vehicles in a road intersection.
The second is a {\em Path Query} ( {pq}) which retrieves the
trajectories that contain any edge of the given path query.
%, or more generally, any trajectory that contains an edge of the query can be a result.
The third is a {\em Strict Path Query}
( {spq})~{\cite{Krogh2016,Koide2015,SanduPopa2011,kim2008path}}
which finds all trajectories that strictly follow the entire path from
beginning to end. %\shane{detours? can we be more precise?}
Interestingly, the path query and strict path query
share many commonalities with disjunctive (OR) and conjunctive (AND)
Boolean queries~{\cite{Christopher2009}}. 
The main difference is that an SPQ is order-sensitive.

%Keywords can be a query constraint when the target is the activity trajectory, coupled with the range query, it can further shrink the searched results, e.g., finding all the Mexican restaurants in the CBD.

\subsubsection{$k$ Nearest Neighbors Query}
%Top-k trajectory search is a very broad area, so we first review the top-k spatial-only trajectory search.

\myparagraph{Search by Trajectory}
{Given a query trajectory $Q$, the $k$ Nearest Neighbor Trajectories Query aims to search the $k$ most similar/nearest trajectories to $Q$, based on a given trajectory similarity measure.
Such a query can be used to find the most similar trips for traffic flow analysis.}
For the special case when the trajectory is a single point, which is also known as \knn search (we use \textit{kNNT} to denote trajectory search), where the Euclidean distance between two points is utilized.
%However, the distance measure between two trajectories is more complex than points as trajectories can have different number of points.
%There are more than $10$ distance measures for trajectory data, and choosing the right distance measure for the dataset is essential.

\myparagraph{Search by Points}
There have also been various work
targeting search on spatial-only trajectory data using 
a set of points as the input query~\cite{Chen2010a,Tang2011,Qi2015,Yan2014,Qi2016}.
%Edit Distance on Real sequences (EDR)~{\cite{chen2005robust}}, Edit distance with Real Penalty (ERP)~{\cite{chen2004marriage}}, Longest Common Subsequences (LCSS)~{\cite{vlachos2002discovering}},
%and Dynamic Time Warping (DTW)~{\cite{yi1998efficient}}. 
%Despite various similarity metrics adopted for various purposes/scenarios, the commonality among these work is that the trajectory distance is computed as an aggregation of point-to-point distances.
\citet{Chen2010a} initially formulated the problem of
querying over a set of points with spatial-only trajectories.
They proposed an incremental expansion method which used an R-tree for
pruning and referred to the search algorithm as {\em Incremental K Nearest
	Neighbors (IKNN)}.

\citet{Tang2011} proposed a qualifier expectation measure
that ranks partial-matching candidate trajectories to accelerate
query processing for non-uniform trajectory distributions and/or
outlier query locations.
\citet{Qi2015,Qi2016} went on to combine {\em
	IKNN} and the qualifier expectation model to improve the efficiency,
and presented a range-based method to improve the efficiency
even further.
By extending a point-wise similarity measure, {\citet{Yan2014}}
assigned an {\em importance value} to each point based on a timestamp to distinguish between points where a user spends more
time within a trajectory.
Given a set of points, \citet{Papadias2005} searched $k$ Nearest 
Neighbor points in term of the aggregate distance of each neighbor to query points, 
and with an \textit{Aggregate Nearest Neighbor} (\ann) search.


\subsubsection{Reverse $k$ Nearest Neighbor Query}
\label{sec:rnns}
\myparagraph{Search over Trajectories}
Different from finding the most similar or nearest trajectories, the reverse $k$ nearest neighbors query will find the trajectory who will take the query as the nearest neighbor.
Formally, 
given a moving object dataset
$\mathcal{D}$ and a candidate point set $Q=\left( o_1,o_2,...,o_m \right)$ as a
query, \citet{Shang2011} aimed to find the optimal point from
$\mathcal{D}$ such that the number of moving objects that choose $o_i$ as the
nearest neighbor is maximized.
Specifically, they proposed a {\em Reverse Path Nearest Neighbor}
(R-PNN) search to find the nearest point {in $\mathcal{D}$ for the trajectory of a moving object, and returned the 
point in $\mathcal{D}$ that is the nearest point for the maximal number of 
	trajectories of moving objects.}
%Shang et al. introduced the concept of {\em influence-factor} to determine the
%optimal point.
%The influence-factor of $o$ is $f$ if $o$ is the nearest neighbor of
%$f$ trajectories for all candidate points in $O$.
%\revione{Given two sets of trajectories and a threshold $\theta$, \textit{trajectory similarity join} \cite{Shang2017} returns all pairs of trajectories from the two sets with similarity above $\theta$, which can be extended to answer our query when $k=1$, by checking whether the query trajectory lies in the result set of each trajectory. While it does not work with arbitrary $k$ as the result set may contain less than $k$ trajectories.}

\citet{Cheema2012} proposed a \textit{continuous
	reverse nearest neighbors} query to monitor a moving object and find
all static points that take the moving object as one of the $k$ nearest
neighbors.
Recently, \citet{Emrich2014} proposed a solution for
the problem of \rknn search with ``uncertain'' moving object
trajectories using a Markov model approach.
A moving object is treated as a result when it always takes the query
object as the nearest neighbor within a given time interval.
All of these approaches target a single point rather than a
commuter trajectory of multiple-points, which is the focus of our work.

\begin{figure}
	\centering
	\includegraphics[height=3.5cm]{graph/TPL.pdf}
	\caption{Half-space pruning used in {\rknn} for query point $q$.}
	\label{fig:tpl}
\end{figure}

\myparagraph{Search over Points}
Most existing {\rknn} search
work focuses on static point data, and often use pruning-refinement
frameworks to avoid scanning the entire dataset.
However, these approaches cannot easily be translated to route search
where both queries and collections consist of multi-point
trajectories.
%Given a set of candidates as a query, a maximizing {\rknn} query
%finds the optimal point with the maximum number of
%results~{\cite{Zhou2011}}.
Improving search performance has attracted much attention
in previous work.
The basic intuition behind filtering out a point $p$ is to find
another point which is closer to $p$ than the query point $q$
~{\cite{Tao2004,Chan2008,Cheema2011}}.

Here, we review the half space method and use a simple example to
show how pruning works.
Figure~\ref{fig:tpl} shows a query point $q$ and a data point $p$.
As we can see, a perpendicular bisector divides the whole space into
two sub-spaces, and all points inside the lower subspace prefer 
$p$ as the nearest neighbor, such as point $r$.
For the reverse nearest neighbor search, $r$ may be filtered 
from the candidate set of query $q$.
More specifically, $r$ can be filtered out if it can be pruned by at
least $k$ such points.


\iffalse
\subsection{Trajectory Planning}
\label{sec:bnp}

Trajectory query is not limited to searching from a trajectory dataset, but also searching the trajectory from a road network, which is known as the \textit{route planning}.
%Trajectory (route) planning is also an area in robot, our trajectory planning is conducted in road network by default.

\myparagraph{Traditional Transit Route Planning}Bus network design is
known to be a complex, non-linear, non-convex, 
NP-hard problem~{\cite{Chen2014a}}.
Based on existing bus networks, \citet{Shivraj1997}
proposed a heuristic method which uses a genetic algorithm to
minimize the cost of passengers and operators.
Population estimation and user surveys~{\cite{Xian2013}} around the
planned route are traditional ways to estimate the number of
passengers that may use the planned travel route, such as
\textit{Journey to Work}\footnote{\url{https://en.wikipedia.org/wiki/Journey_to_work}}
which is data collected as part of a census that describes aspects of
commuting behavior.
However, the data is usually out-of-date, and may not reflect current travel
patterns.

{\myparagraph{Data-driven Transit Network Planning}A general
	approach to \textit{transit network design} is to use {\em demand}
	data from passengers in addition to {\em supply} data from existing
	routes~{\cite{Guihaire2008}}.
	Supply and demand data is usually abstracted as origin-destination
	(OD) pairs, and can be used to identify the most profitable routes.
	With the proliferation of GPS devices on mobile phones and vehicles,
	demand data can be collected via multiple channels in real time, and
	several previous studies have exploited such data.}

By mining taxi data, \citet{Chen2014a} tried to
approximate night time bus route planning by first clustering all
points in taxi trajectories to determine ``hot spots'' which could be
bus stops, and then created bus routes based on the connectivity
between two stops.
Similarly, based on human mobility patterns extracted from taxi data
and smart card data, \citet{Liu2016} proposed a localized
transportation choice model, which predicts travel demand for
different bus routes by taking into account both bus and taxi routes.

{\citet{Toole2015162} used census records and
	mobile phone location information to estimate demand in
	transit routes.
	Historical traffic data~\cite{6878453}, smart cards~\cite{Zhang2017},
	sensors~\cite{Lv2014}, and cellular data~\cite{Pinelli2016} can
	provide more comprehensive demand data and be used to further improve
	data-driven transit network design.
	Most of these studies employ data mining methods, which scan the
	static and historical records for all the customers.
	In contrast, {\rknnt}-based approaches can efficiently maintain
	up-to-date results whenever there is an update on the trajectory
	data; moreover, \rknnt~query can be answered efficiently which is
	critical to real-time decision making.
	In other words, {\rknnt} augments the existing data-driven methods
	for transit network design.}

\myparagraph{Optimal Route Searching}Given a starting vertex and an
ending vertex, the classical problem is to find the
shortest path in a graph.
\textit{Best-first Search} (BFS) and \textit{Depth-first Search}
(DFS) are two commonly used algorithms for this problem.
An extension of this problem is {\em $k$ Shortest Path searching}
($k$SP) ~{\cite{Yen1971,Aljazzar2011}}, which aims to find the $k$
shortest paths from a start vertex $s$ to a target vertex $t$ in a
directed weighted graph $G$.
Yen's algorithm~{\cite{Yen1971}} is a derivative algorithm for
ranking the $k$ shortest paths between a pair of nodes.
The algorithm always searches the shortest paths in a tree containing
the $k$ shortest loop free paths.
The shortest one is obtained first, and the second shortest path is
explored based on the previous paths.
The {\em Constraint Shortest Path} (CSP) problem
{\cite{Lozano2013,Bolivar2014,Wang2016d}} applies resource
constraints on each edge, and solves the shortest path problem
based on these constraints.
An example constraint in this scenario is the time cost.
\fi


\subsection{Spatial Indexing Structures}
\label{sec:spatialindexing}
Trajectory indexing is proposed for efficient search; it organizes the trajectory data in advance, and can avoid scanning every trajectory until returning the result.
Existing trajectory indexing employs two components: indexing points, and mapping tables.
%R-tree \cite{Guttman1984} is one of the most popular index structures for efficient spatial searching.

\myparagraph{Indexing Points}
To achieve scalable efficiency, a space-efficient index
representation and processing framework are crucial, but existing
indexes for trajectory
search~\cite{Vlachos2003,Pfoser2000,ranu2015indexing} rely on an
R-tree~{\cite{Guttman1984}}, which stores all points from the raw
trajectories.
As shown in Figure~\ref{fig:R-tree-indexing}, trajectories are decomposed to points first, then R-tree is used to index all the points, and the mapping table links the point to its belonging trajectory.
It should be noted that trajectory datasets like \texttt{T-drive}~{\cite{Yuan2010}} can have millions of points, and an R-tree has to manage a massive number of maximum
bounding rectangles ( {mbr}), which is not space efficient in practice.
\sheng{
It often requires a prodigious amount of space in order to
accelerate search, and the pruning method originally devised for
point search is not effective for trajectory search as many of the
similarity measures are
non-metric\footnote{\url{https://en.wikipedia.org/wiki/Metric_(mathematics)}}.}
A simple Grid-index can be a more useful index structure in such
scenarios~{\cite{Zheng2013c}}.
%Z-curve and Hilbert curve further enable a simple accessing in Grid-index instead of traversing in a tree.

Rather than storing all the points, a moving object index can be built over the points.
\citet{Pfoser2000} proposed the TB-tree and STR-tree for trajectory data based on an R-tree.
\citet{G2010} built the R-tree in a special way to obtain coverage functions that are effective for trajectory pruning. Similar moving object index such as TPR-trees \cite{Tao2003,Saltenis2000b}, and MVR-trees \cite{Mokbel2003} have been further proposed based on R-tree.
Note that the moving object index cannot support trajectory search as the similarity measure is limited to the Euclidean distance between points.

\myparagraph{Mapping Table}
A mapping table is used to map points to trajectories \cite{Chen2010a,Zheng2013c}.
After searching for a point, the mapping table will help find the correct trajectory it belongs.
To save space, every point will have a unique identifier ranging from $[1, |\mathcal{D}.P|]$ and every trajectory will have a unique identifier ranging from $[1, |\mathcal{D}|]$, where $|\mathcal{D}.P|$ and $|\mathcal{D}|$ are the number of points and trajectories in the dataset $\mathcal{D}$.
This index is widely used in most trajectory search work on point-based indexes.
Moreover, a table can be built for mapping trajectory to points, i.e., a trajectory is then denoted as a list of point integers.
%A mapping table can be compressed when a point is mapped to multiple trajectories.

\myparagraph{Pruning Mechanism}
%In this section, we mainly investigate the index structure for trajectories, and the pruning methodology.
There are two kinds of index pruning: early termination and early abandoning.
Early termination is used for the threshold algorithm \cite{Fagin2003}.
Given an index, the algorithm gradually scans the sorted lists, and early termination can discard the objects directly based on the upper bound of unseen nodes.
For range query, most of the existing approaches use MBR-based pruning, as
MBR intersection with the query trajectory can be used to prune
out irrelevant trajectories~\cite{Keogh2002}.
By judging whether the minimum distance between the query and the node  {node} of the index is bigger than the distance to the current $k$-th result, 
or whether the node intersects with the query range, a batch of objects can be skipped directly.

For example, the nodes $N_7$ and $N_8$ in Figure~\ref{fig:R-tree-indexing}(a) do not intersect with $N_2$, and can be pruned directly, and we only need to check node $N_9$.
Bounded computations are another method used to accelerate search
\cite{Rakthanmanon2012,vlachos2002discovering}.
This is achieved by estimating the upper bound of the similarity
score and comparing it with the current top-$k$ result set to
determine if the exact distance must be computed.
This approach is often referred to as \textit{early
	abandoning}~\cite{Rakthanmanon2012}.


\begin{figure}
	\centering
	\includegraphics[height=5cm]{graph/spatial-indexing.pdf}
	\caption{Indexing spatial-only trajectories based on R-tree and mapping table.}
	\label{fig:R-tree-indexing}
\end{figure}

\iffalse
\subsection{Research Gaps}
\sheng{
	The research gaps in spatial-only trajectory queries are three-fold:
	\begin{itemize} 
		\item There is no work on reverse $k$ nearest neighbors search over trajectory (\rknnt) which has a promising application on transport capacity estimation as we described in Chapter~\ref{chap-introduction}, where the input data is the users' commuter trajectories and transport routes.
		
		\item There are various kinds of queries over trajectory, while no trajectory system which can support all the common spatial-only trajectory queries.
		
		\item Existing indexing structures are for point-based trajectory, which will suffer from the drawback of high cost from the tree-structured index. There is still no index and pruning algorithm for the mapped trajectory which we intend to manage.
	\end{itemize}
}
\fi

\section{Spatial-Textual Trajectory Search}
%In the top-$k$ trajectory search, defining the distance or similarity measure between the query and trajectory is the first step, and several distance measures have been proposed for various scenarios
Spatial-textual search further supports attaching keywords to a query and trajectory, and the relevant trajectories should not only be close to the query trajectory, but also contains keywords from the query, such as $T_1$ shares the keywords ``\textit{seafood}", ``\textit{coffee}'' and ``\textit{swimming}'' with $Q$, as shown in Figure~\ref{fig:running}. ((a): six trajectories
and the query $Q$; (b): Keywords with
a weight of $T_1$ in each point; (c) Point-wise
matching between $Q$ and $ T_1 $.)

\begin{figure}
	\begin{center}
		\includegraphics[width=0.8\textwidth]{graph/Running.pdf}
		\caption{An example of top-$k$ spatial-textual trajectory search.}
		\label{fig:running} 
	\end{center}
	\vspace{-1em}
\end{figure}



\begin{table*}[!ht]
	\ra{1}
	\centering
	\caption{Comparison between related work on spatial-textual
		trajectory search.}
	\label{tab:com}
	\scalebox{0.9}{\begin{tabular}{cccccccc}
			\toprule\addlinespace[0pt]\rowcolor{gray!30}
			& \multicolumn{2}{c}{\textbf{Input}} &   & \multicolumn{2}{c}{\textbf{Search Metric}} & \\ \addlinespace[-2pt]\cmidrule{2-3} \cmidrule{5-6}\addlinespace[-2pt]\rowcolor{gray!30}
			\multirow{-2}{*}{\textbf{Work}}& Query         & Data Model         &  \multirow{-2}{*}{\textbf{Search Semantic}}        & Spatial      & Textual    & \multirow{-2}{*}{\textbf{Output}} \\\addlinespace[-2pt] \midrule
			{\em \pats-based \tkstt}   &    \makecell{Points with\\keywords}           &         Trajectory    &         Disjunctive &     Eu        &       TF$\cdot$IDF     & \makecell{Top-$k$ \\Trajectories} \\ \midrule
			\citet{Zheng2013c}    &     \makecell{Points with\\keywords}          &     Trajectory       &    Conjunctive      &    Eu          &       N/A    & \makecell{Top-$k$ \\Trajectories}  \\ \midrule
			\citet{Shang2012a}   &        \makecell{Points,\\Keywords}         &      \makecell{Spatial-only \\Trajectory\\ and Keywords}      &    Disjunctive      &       Eu       &       Jac    &  \makecell{Top-$k$ \\Trajectories} \\ \midrule
			\citet{Cong2012}   &        \makecell{Point,\\ Keywords}         &     Trajectory      &       Conjunctive   &       Eu       &      N/A       & \makecell{Top-$k$ sub-\\Trajectories}\\ \midrule
			\citet{Zheng2015}    &        Keywords       &     Trajectory        &    Conjunctive      &      Eu        &      ED      &  \makecell{Top-$k$ sub-\\Trajectories}\\ \midrule
			\citet{HanWZZL15}   &    \makecell{Region,\\ Keywords}           &         Trajectory    &         Conjunctive &      N/A        &       N/A     & Trajectories \\ \bottomrule
	\end{tabular}}
\end{table*}


\subsection{Top-$k$ Spatial-Textual Trajectory Search}
\label{sec:literature-etq}
\myparagraph{Similarity Measures}
Different from spatial-only similarity measures, spatial-textual measures for activity trajectories depend on two parts: spatial and textual.
An aggregated similarity measure is a common solution for spatial-textual points \cite{Cong2009a,Yao2016,zhang2014processing}, i.e., the spatial distance can be normalized as proximity, then coupled with the relevance in the textual dimension with a weight to balance the importance.
Such a measure is also extended by \citet{Shang2012a}, where the spatial-distance is computed in a manner similar to the \textit{$k$ Best Connected Trajectories query} (\kbct).
The textual relevance is computed based on the intersection of all the keywords in the trajectory.
Such a measure is a disjunctive measure, as the textual relevance is computed as a part in the final score, which is more flexible in real applications.
Conversely, a conjunctive measure \cite{Zheng2013c,Cong2012} tightens the constraint and requires that the result trajectory should contain all of the query keywords. So, spatial distance is the main ranking measure.

\myparagraph{Search by Points with Keywords}
Several recent papers have explored the problem of spatial-textual
trajectory search in a variety of different scenarios.
Table~{\ref{tab:com}} reports the differences and similarities
between our work and prior work in terms of query and data models,
search semantics, metrics, and result output, where ``Eu" stands for ``Euclidean", ``Jac"
stands for ``Jaccard" and ``ED" stands for ``Edit Distance".
%Example 2 also shows the direct differences with {\em ETQ}.
From Table~\ref{tab:com}, we can see that the only work which
supports the same input and output as {{\pats}} is the work
of \citet{Zheng2013c}.
However, their work only supports conjunctive matching, so all of the
results must contain every query keyword, which simplifies
the more general keyword search problem.
\citet{Shang2012a} presented a similar search
semantic, but keywords are attached to the whole trajectory,
and not individual locations in the query or the data.

\iffalse

At first glance, our problem can be scoped as a spatial-textual
trajectory search~{\cite{Zheng2013c,
		Cong2012, Zheng2015, Shang2012a}}.
%,zheng2016popularity}}.
%In particular, \citet{Zheng2013Towards} note that solutions to the spatial-only trajectory search cannot be applied to trajectories which should include both textual and spatial measures in the search process. 
%
%Here, we consider two aspects:
%(1) How should the trajectory data and the query be modeled; and (2) What search semantics should be imposed on the textual and spatial components.
%, i.e., the similarity model. Here we discuss the most closely related work only, and will expand the discussion in Section~\ref{sec:literature}.
%Regarding the data modeling, as shown in Example~1, the trajectory data is usually modeled as a set of spatial locations (points) plus a set of keywords specifying user preference (if any).
%by all existing works and also this work.
However, our input query differs from past work.
{\citet{Shang2012a}} modeled queries as distinct
sets of locations and keywords.
Consequently, retrieved trajectories were close to target locations,
but contained no common keyword with each query point since the
keywords were not necessarily constrained to any of the locations.
In contrast, {\citet{Zheng2013c}} used Boolean queries, which
only retrieved exact matches.
Neither of these approaches satisfy the query we wish to ask.
For example, in the work of 
\citet{Shang2012a}, the
trajectory in Figure~\ref{fig:running} which contains ``coffee'' 
in the $4^{th}$ point 
that is faraway from the query point may be recognized as a quite similar 
trajectory as the $2^{nd}$ point is spatially close to the query point, and
for {\citet{Zheng2013c}}, a trajectory without the keyword
``coffee'' would not be a result even if all of the other keywords
are matched.
\fi

Other work~\cite{HanWZZL15,Cong2012,Zheng2015} is quite
different with our work from the perspective of input and search
semantics. 
Briefly, \citet{Cong2012} proposed a sub-trajectory
search method to find the minimum travel distance for a single query
point using a Boolean keyword match.
\citet{Zheng2015} proposed an approximate query solution over
trajectories with a set of keywords.

A special case is when the input only contains the keywords,
which is known as a keyword-only query.
Another special case is when the trajectory data and query only contains a single point, which is known as Top-$k$ Spatial Keyword Search (\tksk).

\myparagraph{Keyword-only Query}
The keyword-only query is also an important tool to explore geo-tagged data. 
For example, people might want to search nearby restaurants by keywords 
``\textit{tacos restaurant}" (in Google Maps) when they go to \textit{Los Angeles}. These are normally resolved in two ways: (1) a textual Boolean query (\textit{conjunctive search}), where the objects
that contain all query keywords are returned as results. However, a textual Boolean query is too strict when a query has multiple keywords.
(2) a Top-$k$ Keyword query (\textit{disjunctive search}) which returns the top-$k$ objects ranked by the similarities of objects w.r.t. the query. Here, we focus on the top-$k$ keyword query. Term-at-a-time (TAAT) and Document-at-a-time (DAAT) 
are two common search paradigms \cite{Broder2003} in the area of information 
retrieval. The inverted list of each term can be used to filter 
out objects that do not contain any keyword in the query. 
In terms of the similarity metrics, TF-IDF \cite{Salton1988}
and Language Model \cite{Song1999} are two widely adopted ones.


\myparagraph{Top-$k$ Spatial Keyword Search}
A Top-$k$ Spatial Keyword~(\tksk) search retrieves the $k$
objects with the highest ranking scores, measured as a combination of
distance to the query location, and relevance of the text
description to the query keywords,  e.g., \textit{``finding 3 restaurants which could serve lobster, pizza or steak and are also close to my hotel"}.

The solution can be broadly divided into two categories:
spatial-first~{\cite{Cong2009a,Li2011}} and
text-first~{\cite{Zhang2013, Rocha2011}}.
A spatial-first strategy augments the nodes of a spatial data
structure like an R-tree with a pseudo-document vector to store the
textual information in each node.
For example, the IR-tree~{\cite{Cong2009a,Li2011}} was
proposed to combine an R-tree with an inverted index.
An upper bound of spatial proximity is calculated from the MBR, and an upper bound of
textual relevance is derived from the pseudo-document for pruning.

A spatial-first strategy will scan a few leaf nodes which
contain many unrelated points that do not share any common keywords at
all, so an IR-tree can be inefficient, especially when $k$ is large~{\cite{Mackenzie}}.
For text-first methods \cite{Rocha2011}, the search
space is primarily organized by keywords, so only the points which
share common keywords with the query will be checked, and the
processing time does not increase as in the IR-tree, even
though $k$ is large.
Recently, {\citet{zhang2014processing}} proposed a novel
solution for top-$k$ spatial keyword query which recasts the
problem to the well-known top-$k$ aggregation problem.
\citet{Li2010} proposed \textit{Aggregate Textual Nearest Neighbor} 
(\atnn) search based on \ann~by adding keywords in the query. The similarity
is an aggregation of the spatial proximity to the query locations and 
textual similarity to the query keywords.

\sheng{
\myparagraph{Boolean Range and Top-$k$ Query}\citet{Hariharan2007} proposed the Boolean range query to finds all the objects that contain the query keywords and locate in a query range.
Boolean Top-$k$ query \cite{Cary2010,DeFelipe2008a} searched all the $k$ nearest objects with conjunctive Boolean constraints on textual content, i.e., contain all the query keywords.
\citet{HanWZZL15} investigated the Boolean range query over trajectories where three important aspects, i.e., spatio, temporal and textual, are all taken into consideration.

To answer each type of query, a special design indexing structure is proposed to find the objects that meet the constraint of the query.
However, most of the existing work can only support a single type of query.
\citet{Hoang-Vu2016} proposed a single and unified Spatio-Temporal Textual Index structure (ST2I) to answer the range and \tksk query with multiple constraint types. The primary motivation is to reduce the storage cost of abundant index and also guarantees high query performance, which is consistent with our motivation for the supporting multiple queries over points and trajectories with a single index, while their work only focused on point data, and cannot answer our trajectory search.
%\citet{Zheng} investigated the interactive spatial keyword search by generating candidate input for user with zero-knowledge.
}


%\begin{comment}
%As we can see, the input query specified in \cite{Zheng2013Towards}
%is the same as the input query for ETQ.
%In their work, trajectories were found which contain all of the
%activities in the query using a top-$k$ minimal matching distance.
%\citet{Cong2012Efficient} take only a single point $q$ with a set of
%activities, and searches for sub-trajectories which contain all of the
%activities using a top-$k$ minimum travelling distances from $q$.
%%Given a region as input, \citet{HanWZZL15} find all trajectories located inside the region which also contain all of the keywords, which is not a top-$k$ problem strictly speaking. 
%\citet{DBLP:conf/edbt/ShangDYXZK12} is the only work which supports disjunctive search, and considers both the textual and spatial similarity.
%The main difference between the approach of
%\citet{DBLP:conf/edbt/ShangDYXZK12} and other work is that the
%input is a set of points and a set of activities, where the
%activities are attached to whole trajectory and not points.
%\citet{ZhengYZXSZ15} solve the approximate search problem over semantic
%trajectories by finding the sub-trajectory which contains the most
%relevant activities with top-$k$ minimum travelling distance.
%So, many different spatial-textual trajectory search problems and
%solutions have been proposed in recent years, but none which exactly
%correspond to the ETQ problem.
%\end{comment}

%\begin{comment}
%%Past work calculates spatial and textual similarity separately before combining them to get the final result~, meaning 
%Each query point
%will find the spatially closest point first in {\cite{DBLP:conf/edbt/ShangDYXZK12}}.
%Consider the example in Figure~{\ref{fig:running}}.
%Here, $Q$ has an equal spatial distance to $T_1$ and $T_2$
%as the $1^{st}$, $2^{nd}$ and $3^{rd}$ point of $T_1$ and $T_2$ are
%the closest points to the $p_3$, $p_1$ and $p_2$ in $Q$.
%However, such two connected points do not have any common keywords, so $T_1$
%should be closer to $Q$ than $T_2$ when the $2^{nd}$, $3^{rd}$,
%$4^{th}$ points of $T_1$ and the $2^{rd}$, $4^{th}$ points of $T_2$
%are selected in our case.
%The other common approach {\cite{Zheng2013Towards, Cong2012Efficient}} is to impose a Boolean conjunctive match
%constraint on the keywords, which would return trajectories which are
%further away than $T_1$ or $T_2$ but never take these highly relevant
%trajectories.
%\end{comment}


\begin{comment}
\centering
\label{tab:distancemeasures-st}
\caption{An overview on existing spatial-textual trajectory similarity measure.}
\begin{tabular}{ccc}
\toprule
\multirow{2}{*}{Spatial-textual} & Conjunctive distance \cite{Zheng2013c,Cong2012,Zheng2015}  & $\mathcal{O}(n^2)$  \\
\cmidrule{2-3}          &           Disjunctive distance \cite{Shang2012a}           & $\mathcal{O}(n^2)$  \\ \bottomrule
\end{tabular}
\end{comment}

\subsection{Textual Indexing Structure}
\sheng{Along with the spatial index, the inverted index \cite{Zobel2006} for text part has been widely used for searching spatial-textual data}.
Composed of all the identifiers of objects that contain a particular keyword, the inverted list can be as simple as indicating the existence of this keyword to serve the Boolean part of the query, or as complex as incorporating the 
weight of the keywords to serve the similarity computation for a top-$k$ spatial-keyword query.
Most work~\cite{zhang2014processing,chen2013spatial} 
proposed to use the inverted lists on top of an existing tree-structured index (say R-tree) to deal with spatial-textual search, which is known as spatial-first. 
Text-first usually employs the inverted index as the top-level index and then arranges the postings in the list in a spatial structure. 
%Textual-first indexes have been shown to be faster than the spatial-first index as it can filter more points earlier in the processing.
%Moreover, 

%Set intersection between inverted lists is a common operator for conjunctive Boolean queries \cite{Culpepper2010}.

\sheng{Since each keyword will have a separate inverted list, the space of an inverted index for a corpus will lead to high cost.
For example, the Second Edition of the 20-volume Oxford English Dictionary contains full entries for \numb{171476} words in current use (and \numb{47156} obsolete words).\footnote{\url{https://wordcounter.io/blog/how-many-words-are-in-the-english-language/}}
Then inverted index compression is a common operation to reduce the storage cost of the inverted index.
The goal of inverted list compression is to store a collection of sorted integers with as few as possible bits (low compression ratio) and support query processing (less decompression time) as fast as possible \cite{Wang2017b}.
Inverted list compression approaches usually follow common wisdom of computing the deltas (a.k.a d-gaps) between two consecutive integers first and then compress the deltas using variable bytes, existing commonly used methods include PforDelta \cite{Zukowski2006}, VByte \cite{Cutting1990}, SIMDPforDelta \cite{Lemire2015}, etc.}
%Compressed inverted index 
%For sorted and unsorted lists, the compression method also varies.


\iffalse
\subsection{Research Gaps}
\sheng{
	There are two gaps in the research on spatial-textual trajectory search:
	\begin{itemize}
		\item 
		As we concluded in Table~\ref{tab:com}, a similarity measure which meets the requirement of ranked, disjunctive, and point-wise search semantics is crucial for \tkstt.
		However, such a similarity measure for top-$k$ spatial-textual trajectory search is still an unsolved research question. 
		
		\item Most existing work focus on single query with single indexing framework, and the only exception is the unified index for point data \cite{Hoang-Vu2016}.
		There is no such a unified index and search paradigm to support various top-$k$ queries over trajectories and POI data.
	\end{itemize}
}
\fi

==> response.tex <==

\newcounter{cN}

\newcommand{\weakcomments}[1]{
	\refstepcounter{cN} % incrment counter
	\noindent \hangindent=0em 
	\textbf{\textcolor{maroon}{\underline{Weak Point \thecN}:~}
		\emph{``#1"}	}
}
\newcommand{\comments}[1]{
	\refstepcounter{cN} % incrment counter
	\noindent \hangindent=0em 
	\textbf{\textcolor{red}{\underline{Weak Point \thecN}:~}
		\emph{``#1"}	}
}

\newcommand{\response}[1]{
	\\[0.25em] 
	\hangindent=0.3em \textbf{\textcolor{blue}{\underline{Response}:~}}
	#1
	\vspace{1em} 
}



\setcounter{section}{9}
\renewcommand\thesection{\Roman{section}}
\renewcommand\thesubsection{\thesection.\Roman{subsection}}
\setcounter{figure}{0}
\renewcommand{\thefigure}{\Alph{figure}}
\pagenumbering{roman}

\vspace{2em}
{\centering{\huge\textbf{Response Letter to Reviewer Comments}}\vspace{2em}}

%\twocolumn[]
First of all, we would like to thank the reviewers for the constructive comments that have helped us to improve
our paper titled \emph{``A Survey on Trajectory Data Management, Analytics, and Learning"}.
We have revised our paper accordingly and are re-submitting the
manuscript for further evaluation.
In this response letter, we outline how each concern from the reviewers was
addressed, and describe the changes that we have made to the paper.
To assist the assessment, we have highlighted in the revised manuscript all changes in {\textcolor{blue}{blue color}}, and have cross-referenced each change with a margin note in {\textcolor{red}{red color}}. We have also highlighted several important statements with {{colored underlines}} (blue, green, brown, and red), indicating that these statements have been presented in the original manuscript and might have been overlooked in the first round of review. We have also fixed several small typos and improved the overall presentation. Thank you again for your time and efforts in reviewing our revised manuscript.


%We have also highlighted several important claims with {\textcolor{green}{green-colored underlines}} that have been presented in the original manuscript, in order to indicate that we have mentioned the importance of data distribution and \uni while they might be overlooked in the first round of review. We also fixed several small typos to improve the overall presentation. Thank you for your time and efforts reviewing our revised manuscript.
\setcounter{cN}{0}

\section{Response to Reviewer 1}
\label{sec:r1}
Thanks Reviewer 1 for your endorsement of our work. 
To further improve the quality of this survey, we make several changes according to other reviewers' comments.
It is also worth saying that we noticed there were several new papers published in PVLDB recently (after our submission date), such as \cite{Koide2020} \cite{Wang2020c} \cite{Wang2021}. We added them into the section of similarity measures (Section~\ref{sec:distance}), spatial index (Section~\ref{sec:spatialindexing}), and deep learning (Section~\ref{sec:deep}), respectively.
 
%\bao{R1 mentioned the possibility of elaborating a bit more on the deep learning part. If you have added a bit more details on that, you can include some response on it.}

\setcounter{cN}{0}
\section{Response to Reviewer 2}
\label{sec:r2}
\comments{The trajectory data definition includes only the timestamp in a point and not the data. However, at the description, it is mentioned that each point includes extra data, so I suggest to include the data in the formal definition of a point.}
\response{Thank you. We have added the information about the extra data to the definition.}

\comments{The description of equation 6 needs more details. Actually, the definition is complete but it needs more details to help the reader fully understand the concept.}
\response{Thank you. We have added more descriptive information into the definition.}

\comments{In sections 4.1.2 and 4.1.3, there is a need for at least an introductory sentence. Also, definition 9 requires a more clear description. For instance, what exactly is the query (Q)? - Finally, the authors refer that "the RkNN query include resource allocation, decision support, and profile-based marketing", without any reference.}
\response{Thank you. We have added an introductory sentence in each section. The reference about the applications RkNN are also added. }

\comments{In section 4.2, the description of the Mapping Table is vague; it needs more details.}
\response{Thank you. We have referred Fig.~\ref{fig:R-tree-indexing} and shown an example to have a better description.}

\comments{For the part saying "Distributed Systems for Intensive Similarity Computations" it is more appropriate to replace it with “Map-Reduce for Intensive ....” since the works are based on the map-reduce model, not on distributed systems. Joins are computed using the map-reduce model which can potentially be applied on distributed systems.}
\response{Thanks for pointing it out. We have changed it to be ``MapReduce-based Distributed Systems for Intensive Similarity Computations'', to remove the potential ambiguity.}

%\vspace{-2em}
\setcounter{cN}{0}
\section{Response to Reviewer 3}
\label{sec:r3}
We notice that Reviewer 3 may overlook some important parts of our paper, hence we use four different colors to underline them to address weak points \setulcolor{blue}\ul{1}, \setulcolor{green}\ul{5}, \setulcolor{brown}\ul{6}, and \setulcolor{red}\ul{7}, respectively. 

\comments{The most serious concern I have is the contribution of this survey. As also indicated by the authors, there are several other surveys on trajectory data. It is not clear how the results of these surveys are exploited/upgraded/enhanced in this survey. Or whether this survey just covers more areas for completeness? For potential readers (at least for me), they probably will not feel too excited about this paper. Additionally, the paper does not provide a clear and concise view and motivation.}
\response{
Thanks for the concerns; we understand that a good survey should be novel for readers to overview the state-of-the-art. When we read existing trajectory surveys, we found they were dated as current techniques have advanced significantly in the last three
years, and had a specific focus area such as data mining (detailed comparisons can be found in Section~\ref{sec:new}).

Based on the above observations, we were motivated to write such a survey to provide our readers the latest and complete review.
Reviewer 3 can refer to Section~\ref{sec:new} for our main contributions that distinguish our survey from others. It might be worth highlighting that we do not just cover more areas; instead, we cover the most recent work in a novel way through a pipeline decomposition on trajectory data management, analytics, and learning.
For example, in Table~\ref{tab:applications}, readers can easily link the trajectory pre-processing, similarity measures with upper-level applications.

Compared with other surveys, this survey also broadens the research areas on trajectories, and summarize useful and new resources (e.g., new datasets and commercial systems) than existing trajectory surveys.
Specially, we introduced new cross-disciplinary research on trajectories from computer vision and self-driving.
Most importantly, we point out several open challenges for readers to explore, especially the trajectory applications on public health and self-driving.

Figure~\ref{fig:data-query} has provided a fair and concise overview.
%Please check the underlined part which describes the details.
For the motivation, we added a new paragraph at the beginning of Section~\ref{sec:new} and we hope it can better motivate this survey. %since we are not contributing a new research problem but writing a survey, we think it is more appropriate to use a direct way to deliver what we will cover, just like other trajectory surveys \cite{Zheng2015b,Parent2013a,Richly2018}
%With proper introduction and
%through the comparison with existing surveys and our contributions in Section~\ref{sec:overview}, the motivation of this survey is clear.
For ease of reading and checking, we used \textcolor{blue}{blue} color to highlight several parts that reflect the detailed descriptions of the above summaries. Thank you.

\iffalse
\setulcolor{blue}
\ul{We sincerely hope the reviewer can take another look at the blue outlined text at the introduction; detailed comments are welcomed in future rexvisions.}
\fi
}

\iffalse
\comments{The first part of this article proposes to include some important tutorial materials, such as background knowledge about the research topic, which can better introduce the reader to the topic.}
\response{Sorry, we do not find the points to be revised here.}
\fi

\comments{On page 2, 1(a) (cited from “Social GAN” [78]) is not suitable for expressing the example of traffic surveillance cameras the author wants to express in this article. It is recommended to make some modifications or replace a figure.}
\response{Thanks for this suggestion. We replace a new one from the grand central station dataset \cite{Zhou2012}.}

\comments{The authors label their figures and refer to them in the text with Figure. The authors are invited to use the same wording of the labels in their text.}
\response{Thanks for this suggestion. We have unified all the terms to Fig.}

\comments{ Page 17, line 26-27, revise the sentences :“but not applicable to to urban trajectory data”and “Next, we will will mainly focus on the similarity-based classification”.}
\response{Thanks for pointing it out. We have revised it.}

\comments{The article reviewed several aspects of trajectory data research, but the significance or background knowledge of each sub-topic was not clearly described. Before presenting the technical details of each subtopic, it was not well coherent and introduced.}
\response{To make our survey easy to follow, at the beginning of most sections or sub-sections, we gave short (due to space limit) but proper introductions. For example, in the applications of trajectory, we gave an overview and mentioned the corresponding significance. 
Please kindly note that the text body underlined in \textcolor{green}{green} color is to facilitate the reviewer in checking the associated significance and background (which was in our original submission as well). Thank you.
}
%\setulcolor{green}
%\ul{We sincerely hope the reviewer can take another look at the green outlined text and check the significance and background. We look forwards to seeing detailed concerns on which part does not have the proper background in future revisions, thanks.}


%In the begining of writing this survey, due to space limit, we cannot be too specific. Instead of writing survey by explorate every work, we choose to apply a summarize with an overview. That means we compares the work's problem. For the methodology, we have covered in the previous sections. Trajectory applications are different.

%This paper is an overview survey in my opinion, not a book, and there are too many papers on trajectories. Here I prefer to conclude them in terms of index and methodology using tables, rather than elaborating every paper with details; otherwise, even sixty pages are not enough. Moreover, as we can observe, trajectory research prefers problem novelty and real-world applications, rather than pure techniques part (this is a little different from IR, so DB people usually do not list "research question" in the paper, as our problem itself is new.). Trajectory indexing for this analytic part is very similarly based on the mature spatial index, and the methodology is always filtering and verification. I hope you can understand why I do not mention too much about the techniques, the core part has been covered in the flow charts and tables, and the key indexing techniques are also thoroughly discussed in the first five sections. Thanks very much! Please let me know if you have further concerns.

\comments{The function of the figures and tables should be used to support the author’s point of view. The figures and tables in this article occupy a large space and the content is also detailed, it is conceivable that the authors have spent much effort to do these takes. However, the authors do not have much explanation and analysis of these charts.}
\response{For every figure and table, we have given the proper information in the title and text for readers to interpret. We believe our figures and tables are easy to follow with descriptive texts and indications. We highlight them in \textcolor{brown}{brown}-colored underlines to facilitate the reviewer in walking through them. Thank you.
}	
	
\iffalse	
\setulcolor{brown}
\ul{We sincerely hope the reviewer can take another look at the brown underlines and let us know more details about which figure is not clear in the future revision if possible, thanks.}
\fi

\comments{The article is almost a list of related research on various sub-topics. After reading this survey paper, I don't feel that I have learned anything particularly interesting. It does not provide much new insight or some inspiration for potential readers of related research directions (at least for me).}
\response{
%We covered many sub-topics that are published recently. Firstly, we show a clear taxonomy in various aspects. The most existing part is that we list the datasets. We also form a github repo to list the most important resource.
\iffalse
Before presenting why our survey is not boring, we sincerely suggest that the reviewer read our response to weak point 1 about our novel contributions. If you have checked every part of those contributions, 
you will find that this survey is not a list of sub-topics. 
\fi
We made a thorough taxonomy and concluded at a high-level to avoid abundant descriptions of each recently published work, and we believe this effort is more informative than simply including a list of related research in a flat manner.
%
As a survey that aims to inspire readers to grasp the pain-points and opportunities easily, we provided new insights in every section. 
For example, in the introduction, we listed various datasets from other areas that were always overlooked. We also mentioned that trajectory data could be from various devices rather than just GPS. 
In the second section, we concluded open-source/commercial systems for the first time.
In the third section, we emphasized that the segment-based similarity measure is an emerging topic.
In the fourth section, we summarized the works which are mostly published in the last three years, where no survey has done that.
In the fifth section, we put much effort into the latest research on large-scale trajectory clustering and a new type of classification, trip-purpose classification, which has not been reviewed or discussed in previous survey yet.
In the sixth section, we illustrated four main emerging applications on trajectory data, and we decomposed the common pipeline of each application.
In the seventh section, we reviewed how learning has been applied in various trajectory data analytic stages.
In the eighth section, we pointed out several new applications of trajectories, especially the research on self-driving and public health, and some open problems on building benchmarks and public data repositories.
%
We also highlight the above in \textcolor{red}{red}-colored underlines in each section, to facilitate the reviewer in walking through those insights brought by our work. Thank you.

\iffalse
\setulcolor{red}
\ul{Lastly, we sincerely hope the reviewer can check the red underlines in each section to double-check our new insights. It will be great if the reviewer can give more details on which part is not novel in future revisions, thanks.}
}
\fi


==> storage.tex <==
\section{Management Systems and Pre-processing}
%show a table to conclude all the open research trajectory datasets and their main application scenarios, then
To have an intuitive understanding of trajectory data, we first discuss the trajectory representation and available storage systems for trajectory data.
%Then we describe the common techniques on the pre-processing: the cleaning, compression and map-matching.


%For the commuting trajectory, we can take Google map as example, people can set the commuting in the app, and 77\% of smartphone owners regularly use navigation apps.

%\sheng{Show a trajectory figure here}

\subsection{Trajectory Representation and Storage}
A set of coordinates denoted by two floats (e.g., {\small``-37.807302, 144.963242''}) are traditional
representations of trajectories for storage, search, and analytics.
Storing a trajectory as a set of points is the common method in both research and industry.
Table~\ref{tab:systems} shows several research systems for trajectory data and other commercial systems which can store trajectory data as a specific data structure that are currently available.
% while trajectories can have different lengths.
%For example, a trajectory with $n$ points can be stored as $2n$-dimensional vector easily.
%While not all the trajectories have the same length $n$, hence storing various dimensional trajectory data in a table is not scalable.
%To overcome this problem, converting the raw data by learning \cite{Yao2017,Li2018a} or hashing \cite{Sanchez2016} to a vector of the same length can simplify the storing, while it may lose precision for further analytics.
%This is a relatively simple conversion but is often inefficient
%when used for hashing, or training machine learning models.


\iffalse
Recently, storing raw trajectories as a path on a road network using 
\textit{map matching}~\cite{Lou2009} has been shown to be more
effective in terms of storage~\cite{Song2014} and retrieval
performance~\cite{Wangsheng2018}.
The road network is modeled as a directed graph, and each road is an
edge with a unique ID, and a trajectory can be represented as a
sequence of unsorted integers.
More attributes are attached with the trajectory, such as the timestamp, 
keywords in the activity trajectory \cite{Bao2012Location}.
\fi

In the academic field, several trajectory storage systems have been built to manage trajectory data \cite{Cudre-Mauroux2010,Wang2014e,Shang2018,Ding2018,Xie2016a} by storing a trajectory as a set of points.
Moreover, most trajectory management systems \cite{Cudre-Mauroux2010,Wang2014e,Xie2016a} only support trajectory
storage and simple queries such as a range query (finding trajectories in a rectangle).
More recently, distributed systems \cite{Shang2018,Ding2018} have been developed to store the large-scale of point-based trajectory datasets and can perform advanced queries such as $k$NN search over trajectories.

Existing commercial or open-source systems (e.g., a general database such as Oracle Spatial\footnote{\url{https://www.oracle.com/technetwork/database/options/spatialandgraph/overview/index.html}}, SQL Server\footnote{\url{https://docs.microsoft.com/en-us/sql/relational-databases/spatial/spatial-data-sql-server}}, and MySQL\footnote{\url{https://dev.mysql.com/doc/refman/5.7/en/gis-linestring-property-functions.html}},
or the geospatial database such as ArcGIS\footnote{\url{http://www.arcgis.com/index.html}}, Tile38\footnote{\url{https://github.com/tidwall/tile38}}, PostGIS\footnote{\url{https://postgis.net/}}, GeoMesa\footnote{\url{https://www.geomesa.org/}}, Magellan\footnote{\url{https://github.com/harsha2010/magellan}})
can also be extended for trajectory management.
\sheng{For example, {\em LineString} (Figure~\ref{fig:linstring}) defined in a data-interchange format-GeoJSON\footnote{\url{https://en.wikipedia.org/wiki/GeoJSON}} is a geographic data structure for an array of point coordinates, and trajectory can be stored as a {\em LineString}.}
However, the supported operators over LineString are very limited, e.g., returning the number of points, the starting point, the ending point, and the $i$-th point, etc.
The supported range query and \knn are all over points, and not supported for LineString to our best knowledge.

\begin{figure}[htp]
	\centering
	\includegraphics[height=4.5cm]{graph/linestring.pdf}
	\caption{An example of \textit{LineString} with four points in the GeoJSON format \cite{butler2016geojson}.}
	\label{fig:linstring}
\end{figure}

\begin{table}
	\centering
	\caption{An overview of existing/potential systems for trajectories.}
	\begin{tabular}{cccccc}
		\toprule
		\addlinespace[0pt]\rowcolor{gray!30}
		System          &    Data    &    Indexing     & Range  & $k$NN  &         Similarity Measure          \\
		\addlinespace[-1pt]\midrule
		TrajStore \cite{Cudre-Mauroux2010} & Trajectory &    Quad-tree    & \cmark & \xmark &          \xmark          \\
		SharkDB \cite{Wang2014e}                      & Trajectory & Frame structure & \cmark & \cmark &   Point-to-trajectory    \\
		UITraMan \cite{Ding2018}                      & Trajectory &     R-tree      & \cmark & \cmark &   Point-to-trajectory    \\
		DITA \cite{Shang2018}                       & Trajectory &     R-tree      & \cmark & \cmark & Trajectory-to-trajectory \\ \midrule
		Oracle                               & LineString &     R-tree      & \cmark & \cmark &      Point-to-point      \\
		PostGIS                              & LineString &     R-tree      & \cmark & \cmark &      Point-to-point      \\
		SQL Server                             & LineString &   Grid-index    & \cmark & \cmark &      Point-to-point      \\
		GeoMesa                              & LineString &  Z-order curve  & \cmark & \cmark &      Point-to-point      \\
		Tile38                               & LineString &     R-tree      & \cmark & \cmark &      Point-to-point      \\
		Magellan                              & LineString &     \xmark      & \cmark & \xmark &           \xmark           \\
		GeoSpark \cite{Yu2015}                       & LineString &     R-tree      & \cmark & \cmark &      Point-to-point      \\
		SpatialSpark  \cite{You2015a}                   & LineString &     R-tree      & \cmark & \xmark &           \xmark            \\ \bottomrule
	\end{tabular}
	\label{tab:systems}
\end{table}


%we can show the LineString
%Time series database (InfluxDB\footnote{\url{https://github.com/influxdata/influxdb}}) can store a trajectory as a sequence to maintain the timestamps; 
%however, it cannot support any spatial features (e.g., index) and does not support any trajectory-based queries.

\sheng{
SpatialSpark \cite{You2015a} and GeoSpark \cite{Yu2015} are two representative open-source systems from the research filed of spatial database, which also support the storage and query of LineString.
The range query and $k$NN are the supported queries for the point data, but not for trajectory.
It is promising that these spatial database systems can be extended with trajectory search operator \cite{Pandey2018a} by constructing specific indexing structures and search paradigm in the future, as trajectory is composed of points. In Section~\ref{sec:spatialindexing}, we will review the index structures built over point data.
%Next, we will briefly introduce some representative systems, including Hadoop-GIS \cite{Aji2013}, GeoSpark \cite{Yu2015}, and Simba \cite{Xie2016}.
}


%\bao{More studies of the systems and their supported queries. Draw a table to illustrate the difference.}
\subsection{Trajectory Pre-processing}
\myparagraph{Trajectory Cleaning}
Since trajectory data is usually collected by a GPS with a global average user range error (URE) of 7.8 m (25.6 ft), with 95\% probability, such points in the trajectory are \textit{noisy} \cite{Zheng2015b}. Moreover, the sampling rate of GPS varies in different applications. Two vehicles crossing the same path may have a different number of sampled points. These factors will lead to the value change of distance or similarity, and make it imprecise to analyze further.
Hence, when we get a raw trajectory dataset, the first step is to clean the data.

\textit{Segmenting} \cite{Buchin2011}, \textit{calibration} \cite{Su2013} and \textit{enriching} \cite{Alvares2007} are the three most common cleaning techniques on trajectory data.
Specifically, segmenting will cut a long trajectory into several short trajectories, e.g., analysis of every taxi trip makes more sense than analyzing the whole day taxi trajectory.
\citet{Buchin2011} addressed the problem of segmenting a trajectory based on spatiotemporal criteria.
\citet{AAlewijnse2014} proposed an algorithmic framework for criteria-based segmentation of trajectories that can efficiently process a large
class of criteria.

\citet{Su2013} proposed calibration method to transform a heterogeneous trajectory dataset to one with (almost) unified sampling strategies, in order to achieve a more precise similarity between two trajectories.
For the points with noise, calibration will detect them first and fix to make the trajectory consistent instead of filtering the noise directly.
\citet{Liu2012a} took advantage of road networks topology, geometry information, and trajectory historical information on large scale to conduct the calibration.

When a trajectory is a set of sparse points, \citet{Alvares2007} enriched with more points and semantic information for a complete analysis.
\citet{Yan2011} proposed a framework that enables annotating trajectories of heterogeneous trajectories for any kind of moving objects, with semantic data provided by multiple 3rd party sources.
In contrast, trajectory simplification \cite{Zhang2016e} will remove the redundant points when the sampling rate is high.

\myparagraph{Trajectory Compression}
Existing trajectory compression can be divided into two groups: simplification-based and road network-based.
Excluding the extra points is a common compressing method when the sampling rate is high, which is known as {\em trajectory simplification} \cite{Zhang2016e,Chen2009,Lange2009} and also used in trajectory cleaning.
Removing the points can lead to a more compact size, but it also reduces the quality of the trajectory.
Besides lowering the storage, an error ratio is defined to guarantee that the simplified trajectory is still similar to the original trajectory \cite{Long2013}.

Alternatively, a road network can be used to support compression \cite{Kellaris2013,Song2014,Han2017,Popa2015}, and avoid harming the quality to some extent.
Each trajectory will be projected to the road network as a sequence of road segments.
By encoding each road segment uniquely with a Huffman code \cite{cormen2009introduction}, the trajectory can be represented as a sequence of symbols, which reduces the storage a lot as compared with using latitude and longitude.
Further, string compression techniques \cite{Koide2017,Yang2017b} can be used for trajectory data, including compressing the temporal information.

\myparagraph{Map-matching}
{With a road network, map-matching \cite{Lou2009,Newson2009} projects a raw trajectory onto a real path, it will serve for the cleaning and compression purposes \cite{Kellaris2013}.
The road network dataset of whole world available from \textsc{OpenStreetMap}, and some regions such as \textit{California} \cite{Leskovec2009} and the whole USA.\footnote{\url{http://www.dis.uniroma1.it/challenge9/download.shtml}}}
The road network is always modeled as a weighted graph \cite{cormen2009introduction}, where the road segment is an edge, and the weights could represent the length of the road. Further, a path mapped from raw trajectory is a set of connected edges in the road network.
%When the road network is not available, using the trajectory data to construct the road network \cite{Ahmed2015} can be seen as an opposite direction of map-matching.}

Map-matching is challenging in terms of effectiveness and efficiency.
For efficiency, we need to find the nearest road segments for each point in the trajectory; then the candidate road segments are connected to generate possible paths. Overall, uncertainty is the primary challenge, which reflects on the selection of parameters and candidate paths, and shortest path search.
For effectiveness, mapping a trajectory to the path where the vehicle crossed exactly is the objective. The ground truth matters to evaluate the precision of map matching.
Usually, there are three ways to generate the ground truth: 1) using real vehicles equipped with GPS devices on the road \cite{Newson2009}; 2) labeling the mapped path by humans \cite{Lou2009}; 3) simulating the GPS sampling \cite{Jagadeesh2004} which needs less cost and labor compared with the former two methods.

\subsection{Research Gaps}
\sheng{
	The research gaps in trajectory management systems are three-fold:
	\begin{itemize}
		\item Existing systems are all built over point-based trajectory data.
		Point-based representations are easy to work with, but are not space
		efficient as a float number usually needs eight bytes to store.
		The efficiency of queries over trajectories also suffers from the point-based trajectory similarity measure and indexing, which we will introduce in next two sections.
	%	We also show that point-based index will occupy 
		
		\item The map matching based on the road network is useful for improving the quality of vehicle trajectories, especially for the search and compression. However, existing system still remains on the point-based storage without considering the new features of mapped trajectories.

		\item From the system perspective, supporting various common queries more than range and \knn queries over trajectories are essential, especially that the input for a \knn query can be a trajectory, while most existing systems do not support this.
	\end{itemize}
}

